Fresh-Variable Automata for Service Composition

To model Web services handling data from an infinite domain, or with multiple sessions, we introduce fresh-variable automata, a simple extension of finite-state automata in which some transitions are labeled with variables that can be refreshed in some specified states. We prove several closure properties for this class of automata and study their decision problems. We then introduce a notion of simulation that enables us to reduce the Web service composition problem to the construction of a simulation of a target service by the asynchronous product of existing services, and prove that this construction is computable.

==> about.tex <==
\section*{About}

\subsection{Removed sentences and paragraphs}

\begin{definition}
Let $A,B$ be two variable automata. 
The game $\mathcal{G}(A,B)$ is the alternating parity game 
$\model{\Pos,Mov,p^{\star},\exists,\forall,\lambda,\eta}$ 
 defined by :
\begin{itemize}
\item It's set of positions is  $\Pos=Q(A) \times Q(B)$, 
\item \Abelard moves $Mov^{{\forall}}$ are in $\Graph(\delta(A))$ and \Eloise moves $Mov^{{\exists}}$ 
 are in $\Graph(\delta(B))\times (\mathcal{X}\to \terms)$.
\item The starting position is $p^{\star}=(p_{0},q_{0})_{A,\rho(B)}$ with $\lambda(p^{\star})=\forall$. That is,
 \Abelard moves first and  chooses any  transition $(p_0,\alpha,p') \in \delta(A)$, i.e.:
\begin{align*}
(p_0,q_0)_{(A,B)} \overset{\alpha}{\rightarrow} (p',q_0)_{(A,B)}
\end{align*}
\item The \Eloise must  attempt to match this transition,  i.e., he must find 
$\beta \in Q_{B}$ and a substitution 
$\sigma$ such that $\sigma(\beta)=\alpha$ and  moves 
\begin{align*}
(p',q)_{(A,B)} \overset{\alpha,\sigma}{\rightarrow} (p',q')_{(A,\sigma(B))} 
\end{align*}
\item The two players continue moving alternatively,
that is, $\lambda(p^{\star})=\forall$, and 
if $\lambda(p)=P$ then $\lambda(p')=\neg P$ where $p'$ is a successor of $p$.
\end{itemize}

The winning conditions follow.
\begin{itemize}
    \item If the \Eloise is unable to find any valid transitions to 
match the \Abelard's move, then in this case the \Abelard wins.
    \item  If the game reaches states $(p,q)$ which are both 'dead' 
(i.e., there are no transitions from either state), then in this case the \Eloise wins
    \item Any infinite play is winning for the \Eloise.
   \item If the game reaches states $(p,q)$ which have already been visited, then 
 this is equivalent to an infinite play and it is  a win for the \Eloise.
\end{itemize}
\end{definition}


A strategy $\sigma$ is said to be  regular, and denoted by 
$\sigma^{f}$, if the game graphs induced by $\sigma$ is regular.

\begin{definition}(simulation.)
We say that $B$ simulates $A$ and write $A{\preceq} B$ iff there exists a winning strategy for  \Eloise 
in the game $\mathcal{G}(A,B)$.
\end{definition}

\begin{lemma}
Let $A$ be a \vaut{automata}, and $\rho_{\infty}$ an infinite unfolding, then
every variable in $\rho_{\infty}(A)$ occurs finitely often.
\end{lemma}

\begin{theorem}
The following diagram commutes:
\begin{equation*}
 \xygraph{ !{<0cm,0cm>;<2cm,0cm>:<0cm,1.5cm>} 
[]*+{(A,B)}="S1"
[d]*+{(A,B_{f})}="S2" 
[rru]*+{(A,B_{\infty})}="S3" 
[d]*+{\cdot}="S23"
[rru]*+{(A,\widehat{B}_{\infty})}="S4"
"S1":"S2"_{\model{id,\eta_{f}}} 
"S1":"S3"^{\model{id,\eta_{\infty}}}
"S2":"S23"_{\rho({\mathcal{G}(A,B_f)})} 
"S3":"S23"^{ \rho({\mathcal{G}(A,B_{\infty})})}
"S1":@/^1cm/"S4"^(0.5){\model{id,\hookrightarrow \circ \eta}}
"S3":"S4"^{\model{id,tr}}
"S4":@/^0.5cm/"S23"^{\rho^{f}(\mathcal{G}(A,\widehat{B}_{\infty}))}
}
\end{equation*}
\end{theorem}

%%The proof is achieved by means of  a series of lemmas.
%% \begin{lemma} 
%% \label{strategy:construction:lemma}
%% Let $A$ and $B$ be a  variable automata.
%% If there is a winning strategy for the \Eloise in the game 
%% $\mathcal{G}(A,\eta_{\infty}(B))$ then there exists an automata transformation $tr$ and 
%% a finite winning strategy $\rho^{f}$ for the \Eloise in the game $\mathcal{G}(A,tr(\eta_{\infty}(B)))$ 
%% such that $tr \circ \eta_{\infty}$ can be decomposed into an automata embedding $\hookrightarrow$
%% and an unfolding $\eta$.
%% \end{lemma}
\begin{proof}
We show that out of  any (infinite) winning strategy $\rho_{\infty}$ for the 
\Eloise in the game $\mathcal{G}(A,B_{\infty})$ we can construct a winning strategy $\rho^f$ for 
\Eloise in another game $\mathcal{G}(A,\widehat{B}_{\infty})$ where $\widehat{B}_{\infty}$
can be obtained from $B$ by a composition of  \vaut{automata} embedding and an unfolding such 
that ${\mathcal{G}(A,\widehat{B}_{\infty})}_{|\rho^{f}}$ is regular.
 We need the following Fact.
\begin{fact}
\label{infinite:path:redundant:fact}
  For every infinite play $\pi$ (simple path without loops) in $\mathcal{G}(A,B_{\infty})$
 that follows $\rho_{\infty}$, 
  there exists $p \in Q(A)$, $q \in Q(B)$, $a\in \Sigma_A$, $j \in \mathbb{N}$,
 and an infinite sequence of positions  $(p,q_j^{i_1}),(p,q_j^{i_2}), \ldots$ in $\pi$ such that,
for all $i_m$,  $M^{-}(p,q_j^{i_m})=a$, $\lambda((p,q_j^{i_m}))=\exists$, and $q_j^{i_m} \in \EuScript{B}_{v}(B)$.
\end{fact}
\begin{proof}
On the one hand, the number of states of $A$ is finite. 
On the other hand, since $\pi$ is an infinite path without loops, 
then there exists a state $q \in Q(B)$ and indexes $i,m$ such that $q_i^{m}$ 
occurs infinitely often in $\pi$. Therefore, there exists an infinite sequence 
$(p_1,q_i^{m}),(p_2,q_i^{m+1}),\ldots$ in $\pi$, where $\set{p_i, |i\ge 1} \subseteq Q(A)$.
From which we can extract an infinite sequence $(p_j,q_i^{m_1}),(p_j,q_i^{m_2}),\ldots$, since 
the set $\set{p_i, |i\ge 1}$ is finite.
 This ends the proof of the Fact.
\end{proof}


Let $\gamma_{a,p}$ 
be such a  play  in $\pi$:
\begin{align*}
\gamma_{a,p}= (p',q_j^{i'_2},\exists)\stackrel{\sigma',\beta'}{\to} (p',q_j^{i_2},\forall)  \stackrel{a}{\to} (p,q_j^{i_2},\exists)  
\stackrel{\sigma,\beta}{\to} ...
\end{align*}
 
and $\mathcal{G}$    is modified as follows 

\begin{align}
\label{redundant:path:formula}
\mathcal{G}'=(\mathcal{G} \setminus succ^{\star}(\gamma))
              \cup 
             \big\{(p',q_j^{i'_2},\exists)\stackrel{\sigma',\beta'}{\to} (p',q_j^{i_1},\forall)  \stackrel{a}{\to} (p,q_j^{i_1},\exists)  \big\}
\end{align}


and the strategy $\rho'$ in $\mathcal{G}'$ is modified accordingly: 
\begin{align*}
\rho' =  \rho_{\infty} \setminus (\rho_{\infty}|\gamma) \cup \set{(p',q_j^{i_2},\forall)  \stackrel{a}{\to} (p,q_j^{i_1},\exists)}
\end{align*}

\begin{fact}
The strategy $\rho'$ is winning for the \Eloise in $\mathcal{G}'$. 
\end{fact}
\begin{proof}
Immediate.
\end{proof}


\begin{fact}
There exists a \vaut{automata} $B'$ such that 
$B'$ is an unfolding of $B$ and 
$\mathcal{G}'=\mathcal{G}(A,B')$.
\end{fact}

\begin{fact}
Correction of the above construction.
\end{fact}

By iterating the construction \ref{rho:construction} for every $a \in \Sigma_A$ that satisfies the 
above condition we get the desired result.
\end{proof}

\section{An algorithm for deciding \vaut{automata} simulation}



\begin{lemma}
The following folds.
\begin{itemize}
\item For any unraveling $\eta$ we have that $A\preceq_{W} \eta(A)$ 
\item For any unraveling $\eta_A$ and $\eta_{A}$ we have that
 $\eta_{A}(A) \preceq_{W} \eta_{B}(B)$.
\end{itemize}
\end{lemma}


\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto] 
   \node[state,initial] (q_0)   {$q_0$}; 
   \node[state] (q_1) [above right=of q_0] {$q_1$}; 
   \node[state] (q_2) [below right=of q_0] {$q_2$}; 
   \node[state,accepting](q_3) [below right=of q_1] {$q_3$};
    \path[->] 
    (q_0) edge  node {$x$} (q_1)
          edge  node [swap] {1} (q_2)
    (q_1) edge  node  {1} (q_3)
          edge [loop above] node {0} ()
    (q_2) edge  node [swap] {0} (q_3) 
          edge [loop below] node {1} ();
\end{tikzpicture}



\begin{fact}
There is exists an infinite subpath of $\pi$ of the form 
\begin{align*}
\EloiseM{t_1<\mu X. u_1}{a_1}\EloiseM{t_2<\mu X.u_2}{a_2}\cdots
\end{align*}
where 
\[
\begin{cases}
  t_i \subseteq t & i \ge 1\\
  \mu X. u_1 \subf u &  \\
  \mu X. u_i \subf \mu X. u_{i+1} & i \ge 1
\end{cases}
\]
\end{fact}
\begin{proof} (Of the Fact)
  Since the set of the subterms of $t$ is finite and the path $\pi$ is infinite and simple,
  then there is an infinite application of the rule \texttt{E}-$\mu_f$.  
  That is, there exists an infinite derivation 
  \begin{align*}
    u \leadsto^{\star} \mu X. u_1 \leadsto u_1[X:= fresh(\mu X. u_1)]    
  \end{align*} 
\end{proof}





  \begin{align*}
    \AxiomC{$\AbelardM{\mu X. (a;b;X) <  \mu X.(x;X)}$}
    \RightLabel{\texttt{E-Comp}, with $\sigma=x_1 \mapsto b$}
    \UnaryInfC{$\EloiseM{\mu X. (a;b;X) < x_1; \mu X.(x;X)}{b}$}
    \RightLabel{\texttt{E-}$\mu$, with $\delta=x_1 \mapsto x$}
    \UnaryInfC{$\EloiseM{\mu X. (a;b;X) < \mu X.(x_1;X)}{b}$}
    \RightLabel{\texttt{A-Comp}}
    \UnaryInfC{$\AbelardM{b; \mu X. (a;b;X) < \mu X.(x_1;X)}$}
    \RightLabel{\texttt{E-Comp}, with $\sigma=x\mapsto b$}
    \UnaryInfC{$\EloiseM{b; \mu X. (a;b;X) < x;\mu X.(x_1;X)}{a}$}
    \RightLabel{\texttt{E}-$\mu$, with $\delta=x\mapsto x_1$}
    \UnaryInfC{$\EloiseM{b; \mu X. (a;b;X) < \mu X.(x;X)}{a}$}
    \RightLabel{\texttt{A-Comp}}
    \UnaryInfC{$\AbelardM{a;b; \mu X. (a;b;X) < \mu X.(x;X)}$}
    \RightLabel{\texttt{A}-$\mu$}
  \UnaryInfC{$\AbelardM{ \mu X. (a;b;X) < \mu X.(x;X)}$}
  \DisplayProof
  \end{align*}




The formal definition of the unfolding of variable automata follows.
\begin{definition}(Unfolding)
Let $r$ be the rewriting rule 
\begin{align*}
r : \;\; \mu X. t \leadsto t (X/ fresh(\mu X.(t)))
\end{align*}
where $fresh(u)$ replaces all  the $\mathcal{X}$-variables 
in $u$ by fresh ones. Indeed, the occurrences of the same  variable 
are replaced by the same fresh variable. An unfolding is 
a function $\mu\mathcal{T} \to \mu\mathcal{T}$  such that $\mu(t)=u$ iff 
$(u,t) \in r^{\star}$, where $r^{\star}$ is the reflexive, transitive closure of the 
reduction relation defined by the rewriting system that consists  of the rule $r$.
\end{definition}


\newpage
\subsection{Examples}
Let $t_A=\mu X. (a;b;z;X)$ and $t_B=\mu X. (x;y;a;a;X)$. The related \vaut{automata} are depicted 
in Figure \ref{}.

 

\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto, initial text=] 
   \coordinate (A) at (120:-3cm);
   \coordinate (B) at (120:-10cm);
   \coordinate (C) at (120:-15cm);
   \coordinate (D) at (120:-18.5cm);

   \node [above] at (A) {The \vaut{automata} $A$};
   \node [above,right,right] at (A) {The \vaut{automata} $B$};
   \node [above] at (B) {The \vaut{automata} $\rho^{\infty}(A)$};
   \node [above,left] at (C) {The \vaut{automata} $\rho^{\infty}(B)$};
   \node [above,left,left] at (D) {The \vaut{automata} $A \cap B$};

   \node[state,initial,accepting] (p_0)   {$p_0$}; 
   \node[state] (p_1) [above right=of p_0] {$p_1$}; 
   \node[state,accepting](p_2) [below right=of p_1] {$p_2$};
    \path[->] 
    (p_0) edge  node {$a$} (p_1)
    (p_1) edge  node  {$b$} (p_2)
    (p_2) edge  node {$z$} (p_0);

  \begin{scope}[xshift=6cm]
   \node[state,initial,accepting] (q_0)   {$q_0$}; 
   \node[state] (q_1) [above right=of q_0] {$q_1$}; 
   \node[state] (q_2) [below right=of q_1] {$q_2$}; 
   \node[state,accepting](q_3) [below right=of q_0] {$q_3$};
    \path[->] 
    (q_0) edge  node  {$x$} (q_1)
    (q_1) edge  node  {$y$} (q_2)
    (q_3) edge  node  {$a$} (q_0) 
    (q_2) edge  node  {$a$} (q_3) ;
\end{scope}
\begin{scope}[yshift=-5cm]
   \node[state,initial,accepting] (p_0)   {$p_0$}; 
   \node[state] (p_1) [right=of p_0] {$p_1$}; 
   \node[state,accepting] (p_2) [right=of p_1] {$p_2$}; 
   \node[state,accepting](p_{01}) [right=of p_2] {$p_0^1$};
   \node[state](p_{11}) [right=of p_{01}] {$p_1^1$};
   \node[state,accepting](p_{21}) [right=of p_{11}] {$p_2^1$};
   \node[state,accepting](p_{03}) [right=of p_{21}] {$p_0^3$};
   \node[state](p_{13}) [below=of p_{03}] {$p_1^3$};
   \node[state,accepting](p_{23}) [left=of p_{13}] {$p_2^3$};
    \path[->] 
    (p_0) edge  node  {$a$} (p_1)
    (p_1) edge  node  {$b$} (p_2)
    (p_2) edge  node  {$z$} (p_{01}) 
    (p_{01}) edge  node  {$a$} (p_{11}) 
    (p_{11}) edge  node  {$b$} (p_{21})
    (p_{21}) edge  node  {$z_1$} (p_{03}) 
    (p_{03}) edge  node  {$a$} (p_{13})
    (p_{13}) edge  node  {\textcolor{red}{$b$}} (p_{23}) ;
\end{scope}
  \begin{scope}[yshift=-11cm]
   \node[state,initial,accepting] (q_0)   {$q_0$}; 
   \node[state] (q_1) [right=of q_0] {$q_1$}; 
   \node[state] (q_2) [right=of q_1] {$q_2$}; 
   \node[state,accepting](q_3) [right=of q_2] {$q_3$};
   \node[state,accepting](q_{01}) [right=of q_3] {$q_0^1$};
   \node[state](q_{11}) [right=of q_{01}] {$q_1^1$};
   \node[state](q_{21}) [right=of q_{11}] {$q_2^1$};
   \node[state,accepting](q_{31}) [below=of q_{21}] {$q_3^1$};
   \node[state,accepting](q_{02}) [left=of q_{31}] {$q_0^2$};
    \path[->] 
    (q_0) edge  node  {$x$} (q_1)
    (q_1) edge  node  {$y$} (q_2)
    (q_2) edge  node  {$a$} (q_3) 
    (q_3) edge  node  {$a$} (q_{01}) 
    (q_{01}) edge  node  {$x_1$} (q_{11})
    (q_{11}) edge  node  {$y_1$} (q_{21}) 
    (q_{21}) edge  node  {$a$} (q_{31})
    (q_{31}) edge  node  {\textcolor{red}{$a$}} (q_{02});
\end{scope}

\begin{scope}[yshift=-15cm]
   \node[state,initial,accepting] (p_0)   {$Q_0$}; 
   \node[state] (p_1) [right=of p_0] {$Q_1$}; 
   \node[state] (p_2) [right=of p_1] {$Q_2$}; 
   \node[state,accepting](p_{01}) [right=of p_2] {$Q_3$};
    \path[->] 
    (p_0) edge  node  {$a$} (p_1)
    (p_1) edge  node  {$b$} (p_2)
    (p_2) edge  node  {$a$} (p_{01}) ;
   \end{scope}
\end{tikzpicture}

\newpage
Besides, we need the following fact
\begin{fact}
If $\psi_{A}(A)$ is  simulated by $\psi_B(B)$, where $\psi_{A},\psi_{B}$ are 
unfolding, then for any other unfolding $\psi'_{A}$, 
$\psi'_{A}(A)$ is  simulated by $\psi_B(B)$ as well.
\end{fact}

The first claim holds by the fact that \Eloise uses the copy-cut strategy in the game 
$\mycal{G}(t,\dual{t})$. 
That is, by  coping the moves of \Abelard from $t$ to $\dual{t}$, 
by  choosing $\sigma$ to be the identity, and the fresh assignment 
on $\dual{t}$ equal to the one on $t$, i.e. from any position of the form 
 $\AbelardM{X<X}$, the following derivations are possible:
\begin{align*}
\AbelardM{X<X} \uberTo{Skip}\EloiseMM{X<X}\uberTo{\texttt{E-L}_{\mu}} \AbelardM{\eta(S_X)<X}
\uberTo{(\texttt{A-}\lor)^{\star}, \texttt{A-Comp}} \EloiseM{t'<X}{a} \uberTo{\texttt{E-R}_{\mu}} \EloiseM{t'<\eta(S_X)}{a}
\end{align*}


We will construct a regular winning strategy  
$\rho_r$ and proof that it is winning for \Eloise.
 Let 
$\Pi_X^{1}=\EloiseMM{X<u_1}\EloiseMM{X<u_2}\EloiseMM{X<u_3}\ldots$
and  $\Pi_Y^{2}=\EloiseM{t_1<Y}{\alpha_1}\EloiseM{t_2<Y}{\alpha_2}
\EloiseM{t_3<Y}{\alpha_3}\ldots$. 
For every $X,Y$, 
we have that $\eta_1 \cap \eta_2=\emptyset$ and $\eta_{n+2}=\eta_{n}$, for all $n\ge 2$.



\begin{figure}[h*]
\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=2cm, bend angle=50,
   on grid,auto, initial text=, >=stealth] 
   \node[state,initial,accepting] (p_0)   {$p_0$}; 
   \node[state] (p_1) [below =of p_0] {$p_1$}; 
   \node[state,accepting](p_2) [below =of p_1] {$p_2$};
   \node[state,accepting](p_3) [below =of p_2] {$p_3$};
    \path[->] 
    (p_0) edge  node {$?x$} (p_1)
    (p_1) edge  node  {$!f(x,y)$} (p_2)
    (p_2) edge  node [above left] {$?h(y)$}  (p_3)
    (p_2) edge [bend left] node {$?g(x)$} (p_1)
    (p_3) edge [bend left] node [above left] {$!k(y,y)$} (p_0);

  \begin{scope}[xshift=7.8cm, yshift=0cm,node distance=2.1cm]
   \node[state,initial,accepting] (q_0)   {$q_0$}; 
   \node[state] (q_1) [below =of q_0] {$q_1$}; 
   \node[state] (q_2) [below =of q_1] {$q_2$}; 
   \node[state] (q_{11}) [below left=of q_2] {$q_1^1$}; 
   \node[state] (q_{21}) [below left=of q_{11}] {$q_{2}^1$}; 
   \node[state] (q_{12}) [below left=of q_{21}] {$q_{1}^2$}; 
   \node[state] (q_{22}) [below left=of q_{12}] {$q_{2}^2$}; 

   \node[state] (q_{31}) [below right=of q_{21}] {$q_3^1$}; 
   \node[state] (q_{01}) [below =of q_{31}] {$q_{0}^1$}; 

   \node[state] (q_3) [below right =of q_2] {$q_3$}; 

   \node[state] (q_{03}) [below =of q_3] {$q_{0}^3$};
   \node[state] (q_{13}) [below =of q_{03}] {$q_{1}^3$};

    \path[->] 
    (q_0) edge  node  {$?x$} (q_1) 
    (q_1) edge  node  {$!f(x,y)$} (q_2) 
    (q_2) edge  node  {$?h(y)$} (q_3) 
    (q_2) edge  node [above left] {$?g(x)$} (q_{11}) 

    (q_{11}) edge  node  {$!f(x',y')$} (q_{21}) 
    (q_{21}) edge  node  {$?g(x')$} (q_{12}) 
    (q_{12}) edge  node  [above right] {$!f(x'',y'')$} (q_{22}) 

    (q_{21}) edge  node  {$?h(y')$} (q_{31}) 
    (q_{31}) edge  node  {$!k(y',y')$} (q_{01}) 

    (q_3) edge  node  {$!k(y,y)$} (q_{03}) 
    (q_{03}) edge  node  {$?x$} (q_{13}) 
;
\end{scope}
\end{tikzpicture}
\end{center}
\caption{A \vaut{automata} and its unfolding. }
\label{vautomata:fig:x}
\end{figure}

\section{Possible extensions}
Consider that, inside cycles,  \emph{some} of the variables are fresh.
The following example shows the difficulty of deciding the simulation.
Let $t$ be the \vaut{automaton} defined by $X:=a!;X$ and $u$ defined by 
$Y:=\overline{y}?; z?;Y$, depicted in Figure \ref{sim:ex:vautomata:inifinite}. 
We mention that 
the variable $\overline{y}$ is fresh, but $z$ is not. The problem, 
is the infinite  applications of substitutions as shown bellow.



  \begin{align*}
    \AxiomC{$\AbelardM{X < \red{\sigma_n(\cdots(\sigma_1(Y)))}}$}
    \UnaryInfC{\vdots}
    \UnaryInfC{$\AbelardM{X < \red{\sigma_2(\sigma_1(Y))}}$}
    \RightLabel{\texttt{E-Comp}, with $\sigma_2= \overline{y}_2 \mapsto a$}
    \UnaryInfC{$\EloiseM{X < \overline{y}_2?;a?;\sigma_1(Y)}{a!}$}
    \RightLabel{=}
    \UnaryInfC{$\EloiseM{X < \sigma_1(\overline{y}_2?;z?;Y)}{a!}$}
    \RightLabel{\texttt{E-}$\mu$, with $\eta_2= \overline{y} \mapsto \overline{y}_2$}
    \UnaryInfC{$\EloiseM{X <  \red{\sigma_1(Y)}}{a!}$}
    \RightLabel{\texttt{A-Comp}}
    \UnaryInfC{$\AbelardM{a!; X < \red{\sigma_1(Y)}}$}
    \RightLabel{\texttt{A-}$\mu$}
    \UnaryInfC{$\AbelardM{X<\sigma_1(Y)}$}
    \RightLabel{\texttt{E-Comp}, with $\sigma_1=\overline{y}_1 \mapsto a, z\mapsto a$}
    \UnaryInfC{$\EloiseM{X < \overline{y}_1?;z?; Y}{a!}$}
    \RightLabel{\texttt{E}-$\mu$, with $\eta_1= \overline{y}\mapsto \overline{y}_1$}
    \UnaryInfC{$\EloiseM{X < Y}{a!}$}
    \RightLabel{\texttt{A-Comp}}
    \UnaryInfC{$\AbelardM{a!; X < Y}$}
    \RightLabel{\texttt{A}-$\mu$}
  \UnaryInfC{$\AbelardM{ X < Y}$}
  \DisplayProof
  \end{align*}


\begin{figure}[h*]
\begin{center}
\begin{tikzpicture}[shorten >=1pt, node distance=2cm,on grid,auto, initial text=, 
    bend angle=30] 
   \node[state,initial,accepting] (q_0)   {$q_0$}; 
    \path[->] 
    (q_0) edge  [loop above] node  {$a!$} ();

\begin{scope}[xshift=6cm]
   \node[state,initial,accepting] (p_0)   {$p_0$}; 
   \node[state,accepting](p_1) [right=of p_0] {$p_1$};

    \path[->] 
    (p_0) edge [bend left] node  {$\overline{y}?$} (p_1)
    (p_1) edge [bend left]  node  {$z?$} (p_0);
\end{scope}
\end{tikzpicture}
\end{center}
\caption{}
\label{sim:ex:vautomata:inifinite}
\end{figure}







 For this purpose, it is sufficient to show that,  
if $\match{\hat{\alpha}}{\hat{\beta}}$  appears in $\widehat{\mycal{G}}$, 
then its related matching problem in $\mycal{G}$ is   $\match{\alpha}{\beta}$ 
such that 
\begin{align*}
&\hat{\beta}=\beta \tand \\
& \textrm{there exist }  \hat{\theta}, \theta \tst \hat{\theta}(\hat{\alpha})=\theta(\alpha) \tand \hat{\theta} \sim \theta
\end{align*}

Therefore, the matching problem $\match{\hat{\alpha}}{\hat{\beta}}$ has a solution
iff $\match{{\alpha}}{{\beta}}$ has one.


\mycomment{Unnesessary}{
\begin{lemma}
\label{equiv:sim:lem:2}
Let $A$ and $B$ be two \vaut{automata}. 
  \Eloise has a  winning strategy 
 in the game $\mathcal{G}(A,B)$
iff she  has a  winning strategy 
 in the game $\widehat{\mathcal{G}}(A,B)$.
\end{lemma}
\begin{proof}
The direction "$\Leftarrow$" is straightforward since the game 
$\widehat{\mycal{G}}$  is a particular case of $\mycal{G}$.
 For the direction "$\Rightarrow$", we prove that out of a winning strategy 
of \Eloise in $\mycal{G}(A,B)$ we construct a winning strategy for 
\Eloise in  $\widehat{\mycal{G}}(A,B)$. 
 \Eloise just copies the moves from   $\mycal{G}(A,B)$
to $\widehat{\mycal{G}}(A,B)$   
until finding a pattern in $\mycal{G}(A,B)$ 
 of the form 
\begin{align} 
\label{Moves:pattern:G}
\EloiseM{t_1<X}{a_1} \uberTo{\mycal{G}} \EloiseM{t_1<\eta(X)}{a_1} \uberTo{\mycal{G}}^{\star}  
 \EloiseM{t_2<X}{a_2}  \uberTo{\mycal{G}} \underbrace{\EloiseM{t_2<\eta(X)}{a_2}}_{p_{G}} \uberTo{\mycal{G}}^{\star}  
\end{align}
The corresponding moves of \Eloise in $\widehat{\mycal{G}}(A,B)$  
are exactly the same as \ref{Moves:pattern:G} apart that the last move is 
\begin{align*} 
 \EloiseM{t_2<X}{a_2} \uberTo{\widehat{\mycal{G}}}  \underbrace{\EloiseM{t_2<\eta' (X)}{a_2}}_{p_{\widehat{G}}}
\end{align*}
where $\eta'$ is a fresh assignment. Now from the position 
$\EloiseM{t_2<\eta_2(X)}{a_2}$
\Eloise has to copy the moves of the form   
$ \EloiseM{t < \beta;u}{\alpha?} \uberTo{{\mycal{G}}}
  \AbelardM{\sigma(t) <u}$
to  
$ \EloiseM{t < \beta;u}{\alpha?} \uberTo{\widehat{\mycal{G}}}
  \AbelardM{\sigma'(t) <u}$
and 
$ \EloiseM{t < \beta;u}{\alpha!} \uberTo{{\mycal{G}}}
  \AbelardM{t <\sigma(u)}$
to  
$ \EloiseM{t < \beta;u}{\alpha!} \uberTo{\widehat{\mycal{G}}}
  \AbelardM{t <\sigma'(u)}$,
where $\sigma'=\sigma \circ \eta \circ \eta'^{-1}$. It remains to show that 
the  strategy constructed in such a way is winning for \Eloise in $\widehat{\mycal{G}}$.
 For this purpose, it is sufficient to show that,  
if $t'<u' \in \pi_1$ and $t''<u'' \in \pi_2$ are related, 
then $t'=t''$ and $u'=\eta \circ \eta'^{-1}(u'')$, where $\pi_1$ (resp. $\pi_2$) 
is any path starting from the position $p_{G}$ (resp. $p_{\widehat{G}}$). The 
latter property holds by construction.
\end{proof}
Summing up, the two previous lemmas we get the following conclusion.  
\begin{theorem}
\label{equiv:sim:th}
Let $A$ and $B$ be two \vaut{automata}. 
 There is a simulation of $A$ by $B$ (in the sense of Definition \ref{sim:def}) 
iff \Eloise has a  winning strategy 
 in the game $\mathcal{G}(A,B)$.
\end{theorem}
}




\begin{definition}[Tree, Tree with back-edges]
A pointed digraph $\langle V,E,v_{0} \rangle$ of root $v_0$, is a
\emph{tree} if for each $v \in V$ there exists a unique path from
$v_{0}$ to $v$.  A \emph{tree with back-edges} is a tuple ${\mycal {T}} =
\langle V,T,v_{0},B \rangle$ such that $\langle V,T,v_{0} \rangle$ is
a tree, and $B \subseteq V \times V$ is a second set of edges such
that if $(x,y) \in B$ then $y$ is an ancestor of $x$ in the tree
$\langle V,T,v_{0} \rangle$. We shall refer to edges in $T$ as tree
edges and to edges in $B$ as back-edges. We say that $r \in V$ is a
\emph{return} of the tree with back-edges ${\mycal T}$ if there exists
$x \in V$ such that $(x,r) \in B$. If $v \in T$ and  $r$ is a
return on the tree path from $v_{0}$ to $v$, then we say that $r$ is
\emph{active in $v$} if there is a descendant $x$ of $v$ such that
$(x,r)\in B$.
\label{tree:def}
\end{definition}

We shall say that a pointed directed graph $\langle V,E,v_{0}\rangle$
is a tree with back-edges if there is a partition of $E$ into two
disjoint subsets $T,B$ such that $\langle V,T,v_{0},B\rangle$ is a
tree with back-edges. The reader can verify that a pointed directed
graph $\langle V,E,v_{0}\rangle$ is a tree with back-edges if and only
if for every vertex $v \in V$ there exists a unique simple path from
the root $v_{0}$ to $v$.

Throughout this paper we only consider the class of \emph{well-founded} \vaut{automata}.
 A  \vaut{automata} is well-founded if it enjoys the two following properties: 
\begin{enumerate}
\item  Its underlying rooted graph 
is a tree with back-edges, see Definition \ref{tree:def}, and
\observe{This makes the proofs easier, we can probably   relax this condition}
\item  the co-domain 
of $\kappa$  is the set of back-vertices. Intuitively, if $\kappa(x)=q$, 
for a variable $x \in \mycal{X}$ and a back-vertex $q$, then 
the variable $x$ will be replaced by a fresh one only after passing through $q$.     
\end{enumerate}


\section{Complexity analysis of \vaut{automata} simulation}

\observe{The complexity depends on the size of the game graph that depends on an 
 upper bound of  $|\xi_1  \circ \cdots \circ \xi_i (X^j)|$.}

\begin{lemma}
\label{size:simul:game:lemma}
If $A$ and $B$ are two \vaut{automata}, and   $\rho_{f}$  is a minimal  
 winning strategy for 
the \Eloise  in $\mathcal{G}(A,B)$ then, 
\begin{align*}
 |\mathcal{G}(A,B)_{\rho_f}| = O(Q(A)^{2}\times Q(B)^{2})
\end{align*}
\end{lemma}
\begin{proof}
Let $\Gamma(A,B)$ be the bubble game over $A\times B$.
 First we prove that 
\begin{align*} 
|\mathcal{G}(A,B)_{\rho_f}|=O(\Gamma(A,B))=O(Q(A)^2 \times Q(B)^{2})
\end{align*}
Firstly we argue that  the second equality holds. On the one hand, 
the number of positions of $\Gamma(A,B)$ is $Q(A)\times A(B)$. 
Therefore the size of $\Gamma(A,B)$ is $O(Q(A)^2 \times Q(B)^{2})$

Secondly, to  prove the first equality 
we define a sort of  synchronization mechanism between $\mathcal{G}(A,B)_{\rho_f}$ and 
$\Gamma(A,B)$. The idea is that the bubbles on $\Gamma(A,B)$ correspond to 
some positions in $\mathcal{G}(A,B)_{\rho_f}$, besides, an arrow in 
$\Gamma(A,B)$ corresponds to a finite path in $\mathcal{G}(A,B)_{\rho_f}$.
\end{proof}

\begin{proposition}
If $A$ and $B$ are two \vaut{automata} such that $\mathcal{X}(A)=\emptyset$
 then deciding whether $B$ simulates $A$ can be done in $O(Q(A)^2 \times Q(B)^{2})$
time.
\end{proposition}
\begin{proof}
On the one hand it follows from Lemma  \ref{size:simul:game:lemma}
that the seize of the game $G(A,B)_{\rho_f}$ is $O(Q(A)^2 \times Q(B)^{2})$. 
On the other hand, this game  is reachability one  and therefore can be
 solved in linear time.
\end{proof}


\begin{lemma}
\label{bounded:constants:config:lemma}
Let $A$,$B$ be two \vaut{automata} over $\mycal{T}(\Sigma_0,\mathcal{X})$,
where $\Sigma_0$ is a countable (possibly infinite) set of constant symbols.
The number of constants appearing in  every position (or configuration?) of the 
game $\mycal{G}(A,B)$ is bounded by $|\Sigma_0(A)|+|\Sigma_0(B)|+|m_{!,?}(A,B)| + |m_{?,!}(A,B)|$.
%% Beside, the number of constants appearing in a position of the form $\EloiseM{(t<?y;u)}{!x}$
%%  is bounded by $|\Sigma_0(A)|+|\Sigma_0(B)|+|m_{!,?}(A,B)| + |m_{?,!}(A,B)|-1$, where $x,y$ are variables.
\red{Define $\sharp(c)$ (resp. $\sharp(h)$) as the number of  constants in the current configuration 
  (resp. number of "channels" until the current configuration). 
  and prove (the stronger) statement $\sharp(c) \le \sharp(h)$).}
\end{lemma}
\begin{proof}
The proof is by induction on $n$ the length of derivations. 
We consider a path $p_1 \uberTo{\frac{!}{?}a_1} p_2 \uberTo{\frac{!}{?}a_2} \cdots \uberTo{\frac{!}{?}a_{n-1}} p_n$ in $A$
and a path $q_1 \uberTo{\frac{!}{?}b_1} q_2 \uberTo{\frac{!}{?}b_2} \cdots \uberTo{\frac{!}{?}b_{n-1}} q_n$ in $B$. If $n=1$,  
then the claim holds trivially, since $\sharp_{(p_2,q_2)}(c)=1$ and $\sharp_{(p_2,q_2)}(h)=1$.
If $n > 1$, then let $p_n \uberTo{!a_n} p_{n+1}$ and  $q_n \uberTo{?b_n} q_{n+1}$, the case of  $?a_n$ and $!b_n$ is similar.
We distinguish two cases depending on the nature of $a_n$.
\begin{itemize}
\item $a_n$ is a constant. If $a_n$ is already in the configuration $(p_{n},q_n)$ then 
    $\sharp_{(p_{n+1},p_{n+1})}(c) \le \sharp_{(q_{n+1},q_{n+1})}(h)-1$. 
   Otherwise,     $\sharp_{(p_{n+1},p_{n+})}(c)+1 = \sharp_{(p_{n+1},p_{n+1})}(c) \le \sharp_{(q_{n+1},q_{n+1})}(h) =\sharp_{(q_{n},q_{n})}(h)+1$. 
\item $a_n$ is a variable. If $b_n$ is a constant then,
     since $b_n$ is already in the configuration, then 
$\sharp_{ (p_n, q_n)  }(c) = \sharp_{(p_{n+1},p_{n+1})}(c) \le \sharp_{(q_{n+1},q_{n+1})}(h)-1 =\sharp_{(q_{n},q_{n})}(h)$. 
If $b_n$ is a variable then we distinguish two cases:
  \begin{itemize}
  \item If $(!a_n,?b_n)$ did not already occur  (\red{To formalize}), then  
 on the one hand, either $\sharp_{(p_n,p_n)}(c) = \sharp_{(p_{n+1},p_{n+1})}(c)$ or 
$\sharp_{(p_n,p_n)}(c)+1 = \sharp_{(p_{n+1},p_{n+1})}(c)$ and, on the other hand, 
 $ \sharp_{(q_{n},q_{n})}(h)+1 = \sharp_{(q_{n+1},q_{n+1})}(h)$. Therefore,  
  $ \sharp_{(p_{n+1},q_{n+1})}(c) \le  \sharp_{(p_{n+1},q_{n+1})}(h)$.
  \item If $(!a_n,?b_n)$ did already  occur, that is, there is a configuration 
  $(p_i,q_i) \uberTo{\gamma(!a_n),\gamma(?b_n)} (\gamma(p_{i+1}),\gamma(q_{i+1}))$, $i<n$,  
  then $\sharp_{(p_{n},q_{n})}(h) = \sharp_{(p_{n+1},q_{n+1})}(h)$. We let 
    $(p_n,q_n) \uberTo{\sigma(!a_n),\sigma(?b_n)} (\sigma(p_{n+1}),\sigma(q_{n+1}))$
  
  We distinguish two cases. 
  If   $\sigma(a_n)$ is in the current configuration, then  
   $\sharp_{(p_{n},q_{n})}(c) = \sharp_{(p_{n+1},q_{n+1})}(c)$   and we are done. 
  Otherwise, 
   \end{itemize}
\end{itemize}  
\end{proof}


To this goal, \Eloise in $\mycal{G}(A,B)$ needs a (bounded) memory to store 
the history of the correspondence between the constants chosen 
in $\overline{\mycal{G}}(A,B)$ and those chosen in $\mycal{G}(A,B)$. That is, to 
each position of \Eloise in $\mycal{G}(A,B)$ we associate a  memory $M$ that is a finite set  
of pairs $\set{(a_0,b_0),\ldots}$ where $a_i \in C_0$ and $b_i \in \Sigma_0$. 
The memory is initialized  to the empty set. 



\subsection{Properties of  behavior  expressions with  substitutions}
We first state some properties of the behavior expressions (with  substitutions) 
that  appear  in the simulation game.

\begin{lemma}
\label{theta:var:cor}
Let $A,B$ be two \vaut{automata}.   
Let $\wp$ be the  expression  $[\theta_1 \circ \sigma^i \circ \theta_2](e)$,
 where  $\theta_1, \theta_2$ are  compositions of fresh renamings and substitutions,
$e$ is a behavior expression, and $\sigma^i$ is a substitution.  
If  the expression $\wp$   occurs in the simulation game $\mycal{G}^{}(A,B)$,
 that is, $\wp \in  L_{\mycal{G}^{}(A,B)} \cup R_{\mycal{G}^{}(A,B)}$, then 
there exists a fresh renaming $\rho^i \in \theta_2$ such that 
$dom(\sigma^i) \subseteq codom(\rho^i)$.
\end{lemma}
\begin{proof}
On the one hand, the rules \texttt{E-L}$_{\mu}$ and \texttt{E-R}$_{\mu}$ ensure that any occurrence
of a fixed-point variable $X_i$ is unfolded to $[\rho^i](S_i)$ for a fresh renaming $\rho$, where 
$S_i$  is the corresponding expression to $X_i$. 
On the other hand, all the substitutions are closed, see the rules \ttt{E!-comp} and  \ttt{E?-comp}.
\end{proof}



\begin{lemma}
\label{bounded:motif:lemma:1}
Let $A,B$ be two \vaut{automata}.   
Let $\wp$ be the  expression  $[\theta_3 \circ \rho^i_q \circ \theta_2 \circ \rho^i_p \circ \theta_1] (X_j)$,
 where  $i\neq j$, each $\theta_k, k=1,2,3$ is a composition of fresh renamings and ground substitutions and 
$\rho^i_p,\rho^i_q$ are fresh renamings such that $dom(\rho^i_p)=dom(\rho^i_q)=\kappa^-(X_i)$.
Then, $\wp$   never  occurs in the simulation game $\mycal{G}^{}(A,B)$,
 that is, $\wp \notin L_{\mycal{G}^{}(A,B)} \cup R_{\mycal{G}^{}(A,B)}$.
\end{lemma}
\begin{proof}
 We only discuss the case when $\wp \in L_{\mycal{G}^{}(A,B)}$. The case when 
$\wp \in R_{\mycal{G}^{}(A,B)}$ can be handled  similarly.
 Towards a contradiction, assume that the pattern $\wp$
 occurs.
 Therefore, there must be a series of derivations of the form:
\begin{align*}
 \EloiseMM{[\theta](X_i)< u} & \uberTo{}   \AbelardM{[\rho^{i}_p \circ \theta] (S_i)<u}   \\ 
& \uberTo{\star} \EloiseMM{[\theta_2 \circ \rho^i_p \circ \theta_1] (X_i) < u'}  \\ 
& \uberTo{}  \AbelardM{[\rho^i_q \circ \theta_2  \circ \rho^i_p \circ \theta_1] (S_i) < u''} \\ 
& \uberTo{\star}  \wp
\end{align*}
This is a contradiction since the rule  (\ref{Simplify-rho})   would have simplified 
the expression $[\theta_2 \circ \rho^i_p \circ \theta_1] (X_i)$ to 
$[\theta_2  \circ \theta_1](X_i)$. 
\end{proof}

In what follows, if $C,e$ are  expressions
  we shall write  $C\set{e}$ to mean  that $e$  is a subexpression of $C$.  
\begin{lemma}
\label{bounded:motif:lemma:2}
Let $A,B$ be two \vaut{automata}.   
Let $\wp$ be the  pattern $[\theta_3 \circ \sigma_2 \circ \theta_2 \circ \sigma_1 \circ \theta_1] (X_j)$,
 where  each $\theta_k, k=1,2,3$ is a composition of fresh renamings and substitutions and 
$\sigma_1,\sigma_2$ are substitutions.  
 If the  pattern  $\wp$
    occurs in a position of the simulation game $\mycal{G}^{}(A,B)$
(i.e.  $\wp \in L_{\mycal{G}^{}(A,B)} \cup R_{\mycal{G}^{}(A,B)}$), then 
 $dom(\sigma_1) \cap dom(\sigma_2) = \emptyset$.
\end{lemma}
\begin{proof}
From Lemma \ref{theta:var:cor} it follows that there are fresh renamings 
$\rho^p_1 \in \theta_1$ and  $ \rho^q_2  \in \theta_1 \cup \theta_2 $ 
such that, on the one hand, $dom(\rho^p_1) = \kappa^-(X_p)$ and $dom(\sigma_1) \subseteq codom(\rho^p_1)$, 
 and, on the other hand, $dom(\rho^q_2) = \kappa^-(X_q)$ and $dom(\sigma_2) \subseteq  codom(\rho^q_2)$.
 If $p \neq q$ then by the definition of the game $\mycal{G}$, see Definition \ref{}, 
we have that $codom(\rho^p_1)\cap codom(\rho^q_2)=\emptyset$, and we are done. 
  If  $p=q$ then we distinguish two cases. 
The first case is when  $p=q=j$. This case can not happen since the rule
 \ref{Simplify-sigma} could  have reduced 
$[\theta_3 \circ \sigma_2 \circ \theta_2 \circ \sigma_1 \circ \theta_1] (X_j)$ to 
$[\theta_3  \circ \theta_2 \circ \theta_1] (X_j)$. 
The second  case is when  $p \neq j$.  
 We only discuss  when $\wp \in L_{\mycal{G}^{}(A,B)}$, 
 the case when $\wp \in R_{\mycal{G}^{}(A,B)}$ can be handled   similarly.
There   exists   
 a derivation of the form: 
\begin{align}
\AbelardM{\alpha;C\set{[\theta_1](X_j)}<u} &  \uberTo{}  
\EloiseM{C\set{[\theta_1] (X_j)}<u}{\alpha}  \notag \\ 
&\uberTo{\star}  \EloiseM{C\set{[\theta_1] (X_j)}<\beta;w}{\alpha}   \notag  \\
&\uberTo{}  \AbelardM{\sigma_1 (C\set{[\theta_1] (X_j)})<w},  \quad \textrm{ where } \sigma_1=\match{\alpha}{\beta} \notag \\
&\uberTo{}  \AbelardM{C'\set{[\sigma_1 \circ \theta_1] (X_j)}<w},  \quad  \textrm{ where } C'= \sigma_1 (C) \notag  \\
&\uberTo{\star}  \AbelardM{\alpha''; C''\set{[\theta_2 \circ \sigma_1 \circ \theta_1] (X_j)}<w''}  \label{Passing-via-Xi} \\
&\uberTo{}  \EloiseM{ C''\set{[\theta_2 \circ \sigma_1 \circ \theta_1] (X_j)}<w''}{\alpha''} \notag  \\
&\uberTo{}  \EloiseM{ C''\set{[\theta_2 \circ \sigma_1 \circ \theta_1] (X_j)}<\beta''; m''}{\alpha''} \notag  \\
&\uberTo{}  \AbelardM{ \sigma_2 (C''\set{[\theta_2 \circ \sigma_1 \circ \theta_1] (X_j)})<m''},   \quad \textrm{ where } \sigma_2=\match{\alpha''}{\beta''} \notag  \\
&\uberTo{\star}  \AbelardM{ C''\set{[\sigma_2 \circ \theta_2 \circ \sigma_1 \circ \theta_1] (X_j)})<m''}=\wp \label{last:derivation:Passing-via-Xi}
\end{align}
Notice that the series of derivations \ref{Passing-via-Xi} does not pass through  $X_p$, otherwise 
the substitution $\sigma_1$ would be deleted after the application of the simplification  rule (\ref{Simplify-sigma}).   
Hence the variables instantiated by the substitution $\sigma_1$ never appear again in the remaining derivations 
up to the final expression of the derivation \ref{last:derivation:Passing-via-Xi}, 
and in particular we have that 
$dom(\sigma_1)  \cap \var{\alpha''}=\emptyset$, therefore
$dom(\sigma_1)  \cap dom(\sigma_2)=\emptyset$. 
\end{proof}



%% Summing up the two previous lemmas we get:
%% \begin{corollary}
%% Let $\hat{\beta}=\hat{\theta}(t)$ and $\beta=\theta(t)$ for some term $t$.
%%  We  show that for every variable  $x$ of $t$ we 
%% have that \emph{(i).} $\hat{\theta}(x)$ is a variable iff $\theta(x)$ is a variable, and \emph{(ii).} 
%% if   $\hat{\theta}(x)$ is a constant then $\hat{\theta}(x)={\theta}(x)$. 
%% \end{corollary}

\subsection{The construction of monotonic strategies }
\label{contruct:monotonic:sec}

In this section we show that if \Eloise has a winning strategy  
in the simulation game, then she has a \emph{monotonic} winning strategy, 
Lemma \ref{posi:monotonic:strat:lemma}.
The definition of monotonicity follows. 

\begin{definition}
\label{monotonic:strat:def}
In a simulation game $\mycal{G}(t,u)$, 
a strategy is  \emph{monotonic} if
 every fresh renamings $\rho$ chosen by \Eloise 
 is  the identity.
\end{definition}

In order to prove the Lemma \ref{posi:monotonic:strat:lemma}, we need the following definition.

\begin{definition}
\label{congruence:def}
We define the notion of \congmatch{matching}   of renamings,
terms, expressions  and positions.  

\begin{enumerate}[{(}I{).}]
\item Let $\hat{\theta}=\hat{\xi}_1\circ \cdots \circ \hat{\xi}_n$
and  $\theta=\xi_1\circ \cdots \circ \xi_n$, for $n\ge 0$, where every $\hat{\xi}_i,\xi_i$ is either a substitution 
or a fresh renaming. We say that $\hat{\theta}$ \congmatch{matches}
$\theta$ and write   $\hat{\theta} \mycong \theta$ iff for every $i=1,\cdots, n$,
 one of the two  following cases holds: 
\begin{enumerate}[{(}i{).}]
\item  $\hat{\xi}_i=\rho^{k}_p$, for some $k$ and some $p\ge 1$,  and   $\xi_i=\rho^{k}_1$,  or
\item  $\hat{\xi}_i=\sigma^{k}$, for some $k$,  where there exists $p>i$ s.t. 
       $\hat{\xi}_p=\rho^k_p$ and  $dom(\sigma^k) \subseteq codom(\rho^k_p)$ and   $p \ge 1$, 
      and  in this case $\xi_i=\sembrack{\sigma^{k} \circ \rho_{p}^k \circ (\rho_1^k)^{-1}}$. 
\end{enumerate}


\item A term $\hat{u}$ \congmatch{matches} a term $u$ iff there exist a term $t$ and $\hat{\theta}$ and $\theta$
 such that $\hat{\theta}(t)=\hat{u}$ and ${\theta}({t})={u}$.

\item We say that an  expression $\hat{e}$ \congmatch{matches} an expression $e$ and write $\hat{e} \mycong e$
%% iff  
%% \begin{align*}
%% \begin{cases}
%%  \hat{t}; \hat{e}_1  \mycong t; e_1  & \tif \hat{t} \mycong t \tand \hat{e}_1 \mycong e_1 \\
%%  \hat{e}_1 \lor  \hat{e}_2 \mycong e_1 \lor  e_2 &\tif \hat{e}_1 \mycong e_1 \tand \hat{e}_2 \mycong e_2 \\
%%  [\hat{\theta}](X) \mycong [\theta](X) & \tif \hat{\theta} \mycong \theta
%% \end{cases}
%% \end{align*}
%% \red{Can be replaced with }
iff there exists $\hat{\theta}$ and $\theta$ and an expression 
$e_0$ such that $\hat{\theta} \mycong \theta$, 
$NF_{\mathcal{S}}(\hat{[\theta]}(e_0))=\hat{e}$ and $NF_{\mathcal{S}}([\theta](e_0))=e$. 

\item  We say that a  position $\hat{\wp}$ matches $\wp$  and write 
$\hat{\wp} \mycong \wp$ iff one of the two following cases hold:
\begin{enumerate}[{(}i{).}]
\item if $\hat{\wp}=\EloiseM{\hat{t} < \hat{u}}{\hat{\alpha}}$ and ${\wp}=\EloiseM{{t} < {u}}{ {\alpha}}$, then
$\hat{t} \mycong t$, $\hat{u}\mycong u $, and 
$\hat{\alpha} \mycong \alpha$. 

\item if $\hat{\wp}=\AbelardM{\hat{t} < \hat{u}}$ and ${\wp}=\AbelardM{{t} < {u}}$, then
$\hat{t} \mycong t$ and  $\hat{u}\mycong u $.
\end{enumerate}
\end{enumerate}
\end{definition}

%% The following Lemma shows that the \congmatch{matching} is compatible with 
%% the simplification rules of  the system $\mathcal{S}$.
%% \begin{lemma}
%% \label{invariance:S:lemm}
%% Let $e$ be a "behavior" expression, 
%%  and let $\hat{\theta}$ and $\theta$ be composition of substitutions and fresh renamings.
%% If $\hat{\theta} \mycong \theta$  
%% then  $NF_{\mathcal{S}}(\hat{\theta}(e)) \mycong NF_{\mathcal{S}}(\theta(e))$. 
%% \end{lemma}

%% \begin{proof}
%% The proof is by induction on the structure of $e$.
%% If  $e$ is a term or of the form $e_1 \lor e_2$ or of the 
%% form $t;e'$  then  the result is obvious. If $e$ is of the form 
%%  $\gamma(X)$ where $\gamma$ is a composition of substitutions and fresh renamings and $X_i$ is a fixed-point variable then 
%% the proof is by a simple induction on $n$, the number of applications of the rule \ref{Simplify}, 
%% since it is the only rule that can be applied among the rules of the system $\mathcal{S}$. 
%% If $n=0$, then the result holds since $\hat{\theta}\circ \gamma \mycong \theta \circ \gamma$.
%% If $n>1$, then  
%%   $\hat{\theta}= \hat{\theta}_1 \circ \hat{\xi}_i \circ \hat{\theta_2}$ and  
%% $\theta= {\theta}_1 \circ \theta' \circ \theta_2$ such that 
%% $\hat{\theta}_j \mycong \theta_j, j=1,2$ and $\xi_i \mycong \theta'$. 
%% Since both $dom(\xi_i) \subseteq \kappa^{-1}(X_i)$ and $dom(\theta') \subseteq \kappa^{-1}(X_i)$
%% then by applying the rule \ref{Simplify} once we get 
%% $\hat{\theta}_1 \circ \hat{\xi}_i \circ \hat{\theta_2}(X_i) \uberTo{} \hat{\theta}_1 \circ \hat{\theta_2}(X_i)$
%% and 
%% $ \theta_1 \circ \theta' \circ \theta_2(X_i) \uberTo{} \theta_1 \circ \theta_2(X_i)$.
%% %%  It is sufficient to consider $t$ a leaf, that is, either a variable,
%% %% a constant, or a fixed-point variable. Let $\hat{\theta}=\hat{\xi}_1\circ \cdots \circ \hat{\xi}_n$
%% %% and  $\theta=\xi_1\circ \cdots \circ \xi_n$.  The case when $t$ is a constant is obvious. 
%% %% If  $t$ is  a fixed-point variable $X_i$ then the simplification rule 
%% %% \ref{Simplify} is applied many times and  the claimed property holds by a simple induction 
%% %% on the number of applications of the  rule \ref{Simplify}.   
%% \end{proof}

Before proving the main proposition of this section, we need first to prove a technical Lemma.
\begin{lemma}
\label{subs:cong:lemma}
Let $\alpha, \hat{\beta}, \beta$ be terms in $\mterms$ such that
$\hat{\beta}\mycong \beta$ and $\alpha$ is ground. If $\hat{\sigma}$ (resp. $\sigma$) 
is the solution of the matching problem  $\match{\hat{\beta}}{\alpha}$ (resp. $\match{\beta}{\alpha}$),
then  $\hat{\sigma} \mycong \sigma$.
\end{lemma}
 \begin{proof}
Let $\hat{\beta}=\hat{\theta}(t)$ and $\beta=\theta(t)$ for some term $t$.
 We  show that for every variable  $x$ of $t$ we 
have that \emph{(i).} $\hat{\theta}(x)$ is a variable iff $\theta(x)$ is a variable, and \emph{(ii).} 
if   $\hat{\theta}(x)$ is a constant then $\hat{\theta}(x)={\theta}(x)$. 

Let $\hat{\theta}=\hat{\theta}_1 \circ \hat{\theta}_2$ and $\theta=\sigma_1\circ \cdots \circ \sigma_2$. 
 There exists  $\hat{\rho}^i \in \hat{\theta}_2$ s.t. $x\in dom(\hat{\rho}^i)$
and according to Lemma \ref{theta:var:cor} 
there is at most a substitution $\hat{\sigma}_x \in \theta_1$ s.t. 
 $dom(\hat{\sigma}_x) \subseteq codom(\hat{\rho}^i)$, therefore 
$\ttt{eval}([\hat{\theta}](x))= \ttt{eval}([\hat{\sigma}_x \circ \hat{\rho}^i](x))$. 
On the other hand, since $\hat{\theta}\mycong \theta$, then by definition 
there exists $\sigma_i \in \theta$ s.t. $\sigma_i= \sembrack{\hat{\sigma}_x \circ \hat{\rho}^i}$.
Hence
$\ttt{eval}([\theta](x))=\ttt{eval}([\sigma_i](x))= \ttt{eval}([\hat{\sigma}_x \circ \hat{\rho}^i](x))= 
\ttt{eval}([\hat{\theta}](x))$.

%This ends the proof of the Claim.
 \end{proof}

\begin{proposition}
\label{posi:monotonic:strat:lemma}
\Eloise has a winning strategy in $\widehat{\mathcal{G}}(t,u)$ iff 
she has  a monotonic  winning strategy in $\mycal{G}(t,u)$.
\end{proposition}


\begin{proof}
For the  direction ''$\Leftarrow$'',  
  we prove that out of a  monotonic  winning strategy 
of \Eloise in  $\mycal{G}(t,u)$ we construct a winning strategy for 
\Eloise in $\widehat{\mycal{G}}(t,u)$.  For this purpose, it is sufficient 
 to show that each move of \Abelard in  
$\widehat{\mycal{G}}(t,u)$ can be  mapped to an   \Abelard move in $\mycal{G}(t,u)$, 
and   \Eloise response in $\mycal{G}(t,u)$ can be  mapped also to 
an  \Eloise move in $\widehat{\mycal{G}}(t,u)$ such that the following invariant holds:
\begin{align}
\label{invariant-sim}
\tag{Inv}
\textrm{If }  \hat{\wp} \in \Pos(\widehat{\mycal{G}}(t,u))  \tand \wp \in  \Pos(\mycal{G}(t,u))
  \textrm{ are "related",   then } \hat{\wp} \mycong \wp.
\end{align}
This is known as the  back and forth meta-simulation between  $\widehat{\mycal{G}}(t,u)$ 
and  ${\mycal{G}}(t,u)$. The proof is by induction on the number  of alternations  between 
$\widehat{\mycal{G}}(t,u)$  and  ${\mycal{G}}(t,u)$.
The first alternation trivially holds  since the two  starting positions of 
$\widehat{\mycal{G}}(t,u)$ and $\mycal{G}(t,u)$ are equal.
Assume that we are at the alternation  $n$ of the meta-simulation and  
let $\hat{\wp}_n$  be a position in  $\widehat{\mycal{G}}(t,u)$ and 
 $\wp_n$  its related   position in  ${\mycal{G}}(t,u)$.

We consider two possibilities: when both $\hat{\wp}_n$ and 
 $\wp_n$  are  \Abelard positions, and when they are \Eloise positions. 
 Consider  the first  possibility and an  \Abelard move $\hat{\wp}_n \uberTo{} \hat{\wp}_{n+1}$ in 
  $\widehat{\mycal{G}}(t,u)$. 
 We distinguish many cases according to the 
structure of $\hat{\wp}_n$.

\begin{proofbycases}
\begin{caseinproof}
The cases when   
$\hat{\wp}_{n}=\AbelardM{\hat{t}_1 \lor \hat{t}_2 <\hat{u}}$  and 
$\hat{\wp}_{n}=\AbelardM{[\hat{\theta}](X)< u }$ are straightforward, since 
the rules \texttt{A-}$\lor$ and \texttt{A-Skip} are applied, respectively. Hence
the move in  $\mycal{G}(t,u)$ is the same as the move 
  $\hat{\wp}_n \uberTo{} \hat{\wp}_{n+1}$ and the invariant \ref{invariant-sim} is maintained.
\end{caseinproof}

\begin{caseinproof}
If  $\hat{\wp}_{n}=\AbelardM{\hat{\alpha};\hat{t}<\hat{u}}$ and  
$\AbelardM{\hat{\alpha};\hat{t}<\hat{u}} \uberTo{} \EloiseM{\hat{t}<\hat{u}}{\hat{\alpha}}$
is a move in $\widehat{\mycal{G}}(t,u)$, then in this case, since  the invariant 
(\ref{invariant-sim})  holds then    ${\wp}_{n}=\AbelardM{{\alpha};{t}<{u}}$
and  $\hat{\alpha};\hat{t} \mycong \alpha;{t}$ and $\hat{u} \mycong u$.
 \Abelard move in $\mycal{G}(t,u)$ is 
$\AbelardM{{\alpha};{t}<{u}} \uberTo{} \EloiseM{{t}<{u}}{{\alpha}}$  and it remains 
to show that $\hat{t}\mycong t, \hat{u}\mycong u$ and $\hat{\alpha} \mycong \alpha$. 
Since $\hat{\alpha};\hat{t} \mycong \alpha;{t}$ then there exists $\hat{\theta}$
and $\theta$ and a term $t'$ such that $\hat{\theta} \mycong \theta$ and 
$NF_{\Eu{S}}([\hat{\theta}](t')) =  \hat{\alpha}; \hat{t}$ and  
$NF_{\Eu{S}}([{\theta}](t')) =  \alpha; t$. Therefore, 
$t'$ is of the form $\alpha_0; t_0$ where $\alpha_0$ is a term and 
$t_0$ is an expression. Hence,  
$NF_{\Eu{S}}([\hat{\theta}](t')) = NF_{\Eu{S}}([\hat{\theta}](\alpha_0 ; t_0))= 
 NF_{\Eu{S}}([\hat{\theta}](\alpha_0)) ; NF_{\Eu{S}}([\hat{\theta}](t_0)) =  \hat{\alpha}; \hat{t}$. 
And similarly,  
$NF_{\Eu{S}}([{\theta}](t')) = NF_{\Eu{S}}([{\theta}](\alpha_0 ; t_0))= 
 NF_{\Eu{S}}([{\theta}](\alpha_0)) ; NF_{\Eu{S}}([{\theta}](t_0)) =  {\alpha}; {t}$.
Therefore, $\hat{\alpha}\mycong \alpha$ and $\hat{t} \mycong t$.
\end{caseinproof}
\end{proofbycases}


Secondly, we  consider  the second   possibility;  when 
 both $\hat{\wp}_n$ and 
 $\wp_n$  are  \Eloise positions,
and an  \Eloise move ${\wp}_n \uberTo{} {\wp}_{n+1}$ in 
  ${\mycal{G}}(t,u)$ that has to be mapped to an \Eloise move in   $\widehat{\mycal{G}}(t,u)$. 
 We distinguish many cases according to the 
structure of $\wp_n$.

\begin{proofbycases}
\begin{caseinproof}
The case when $\wp_{n}=\EloiseM{t<u_1 \lor u_2}{\alpha}$ is straightforward. 
\end{caseinproof}


\begin{caseinproof}
If ${\wp}_{n}=\EloiseMM{ [{\theta}](X_i) <{u}}$, then in this case we have  a move in $\mycal{G}(t,u)$ 
that results from the  derivations 
\begin{align*}
\AbelardM{ [\theta](X_i) <{u}} \uberTo{\texttt{E-L}_{\mu}} \AbelardM{ [\rho_1^{i} \circ {\theta}](S_i) <{u}} 
 \uberTo{\Eu{S}^*} \AbelardM{ NF_{\mathcal{S}}([\rho_1^{i} \circ {\theta}](S_i)  <{u}}=\wp_{n+1}
\end{align*} 
 and its  related derivations in  $\widehat{\mycal{G}}(t,u)$  are
\begin{align*}
\AbelardM{ [\hat{\theta}](X_i) <\hat{u}} \uberTo{\texttt{E-L}_{\mu}} \AbelardM{ [\rho_p^{i} \circ \hat{\theta}](S_i) <\hat{u}}
\uberTo{}    \AbelardM{NF_{\mathcal{S}}([\rho_p^i \circ \hat{\theta}](S_i)) <\hat{u}}=\hat{\wp}_{n+1}
\end{align*} 

From the induction hypothesis we have that $\hat{\theta}\mycong \theta$ and  $\hat{u} \mycong u$.
Therefore,  we get $\rho_p^{i} \circ \hat{\theta} \mycong \rho_1^{i} \circ {\theta}$ by the item \emph{(I.i)} of 
the Definition \ref{congruence:def}. It follows that $\hat{\wp}_{n+1} \mycong \wp$. 


%% And it remains to show that 
%% $NF_{\mathcal{S}}([\rho_p^i \circ \hat{\theta}](S_i)) \mycong NF_{\mathcal{S}}([\rho_1^{i} \circ {\theta}](S_i))$, but
%% this follows from Lemma \ref{invariance:S:lemm}. 
\end{caseinproof}



\begin{caseinproof}
The case  when ${\wp}_{n}=\EloiseM{ {t} < [{\theta}](X_i)}{a}$ is  the same as  the previous 
one apart that  the rule \ttt{E-R}$_{\mu}$ is applied instead of  \ttt{E-L}$_{\mu}$ .
\end{caseinproof}

\begin{caseinproof}
If ${\wp}_{n}=\EloiseM{ {t} <{\beta};{u}}{! {\alpha}}$, then in this case we have the  move  $\wp_{n}\uberTo{} \wp_{n+1}$ in 
 $\mycal{G}(t,u)$ that results from the derivations:
\begin{align*}
\wp_{n}=\EloiseM{({t} <{\beta};{u})}{! {\alpha}} \uberTo{\ttt{E!}} \AbelardM{[\gamma](t)<{[\sigma]}({u})} \uberTo{\Eu{S}^*} \AbelardM{NF_{\Eu{S}}([\gamma]{t})<{NF_{\Eu{S}}([\sigma]({u}))}}=\wp_{n+1}, \;\;
\textrm{ where } \sigma = \match{\beta}{\gamma(\alpha)}
\end{align*}
 and their  related derivations in  $\widehat{\mycal{G}}(t,u)$  are
\begin{align*}
 \hat{\wp}_{n}=\EloiseM{(\hat{t} <\hat{\beta};\hat{u})}{! \hat{\alpha}} \uberTo{\ttt{E!}} 
    \AbelardM{[\hat{\gamma}](\hat{t})<[\hat{\sigma}](\hat{u})}
\uberTo{\Eu{S}^*} \AbelardM{NF_{\Eu{S}}[\hat{\gamma}](\hat{t})<{NF_{\Eu{S}}([\hat{\sigma}]({\hat{u}}))}}=\hat{\wp}_{n+1}, \\ 
\textrm{ where } \hat{\gamma}=\gamma \circ \hat{\xi} \tand \hat{\sigma}= \match{\hat{\beta}}{\hat{\gamma}(\hat{\alpha})}
\end{align*}
Notice that $\hat{\gamma}$ is chosen as   $\gamma \circ \hat{\xi}$ where there exists $t_0$ and $\hat{\xi}$
and ${\xi}$ such that $\hat{\xi}(t_0)=\hat{t}$ and $\xi(t_0)=t$, since 
it follows from induction hypothesis that $\hat{t}\mycong t$. 
On the one hand, from the induction hypothesis  
we have that   $\hat{u} \mycong u$, $\hat{\beta}\mycong \beta$, 
and $\hat{\alpha} = \alpha$. 
On the other hand,  it follows from Lemma \ref{subs:cong:lemma} that
 $\hat{\sigma} \mycong \sigma$.
It remains to show that $NF_{\mathcal{S}}([\hat{\sigma}](\hat{u})) \mycong NF_{\mathcal{S}}([\sigma](u))$.
That is, we need to show that there exist an expression $g_0$ and $\hat{\theta}$ and $\theta$ such that 
 $\hat{\theta}\mycong \theta$ and 
\begin{align}
\label{aim:eq:NF}
\begin{cases}
 NF_{\mathcal{S}}([\hat{\theta}](g_0))  = NF_{\mathcal{S}}([\hat{\sigma}](\hat{u}))   \\
 NF_{\mathcal{S}}([\theta](g_0))  = NF_{\mathcal{S}}([\sigma](u))
\end{cases}
\end{align}
But, since $\hat{u} \mycong u$ then  
there exist an expression $u_0$ and $\hat{\theta}_u$ and $\theta_u$ such that 
 $\hat{\theta}_u  \mycong \theta_u$  and
\begin{align*}
\begin{cases}
 NF_{\mathcal{S}}([\hat{\theta}_{u}](u_0))  = \hat{u}  \\
 NF_{\mathcal{S}}([\theta_u](u_0))  =u
\end{cases}
\end{align*}
By replacing $\hat{u}$ and $u$ by their respective values,  the equations \ref{aim:eq:NF} become

\begin{align}
\label{aim:eq:NF:2}
\begin{cases}
 NF_{\mathcal{S}}([\hat{\theta}](g_0))  = NF_{\mathcal{S}}([\hat{\sigma}]( NF_{\mathcal{S}}([\hat{\theta}_{u}](u_0))))   \\
 NF_{\mathcal{S}}([\theta](g_0))  = NF_{\mathcal{S}}([\sigma](NF_{\mathcal{S}}([\theta_u](u_0))))
\end{cases}
\end{align}
In  order to prove the equations (\ref{aim:eq:NF:2}) it is sufficient to show that 
\begin{align}
\label{aim:eq:NF:3}
\begin{cases}
 NF_{\mathcal{S}}([\hat{\sigma}]( NF_{\mathcal{S}}([\hat{\theta}_{u}](u_0)))) =    NF_{\mathcal{S}}([\hat{\sigma} \circ \hat{\theta}_{u}](u_0)) \\
 NF_{\mathcal{S}}([\sigma](NF_{\mathcal{S}}([\theta_u](u_0))))  = NF_{\mathcal{S}}([\sigma \circ \theta_u](u_0))
\end{cases}
\end{align}
under the hypothesis  $\hat{\theta}_{u} \mycong \theta_u$ and $\hat{\sigma} \mycong \sigma$,
that is, by taking $\hat{\theta}=\hat{\sigma}\circ \hat{\theta}_u$, ${\theta}={\sigma}\circ {\theta}_u$, 
and $g_0=u_0$. 
But the equalities (\ref{aim:eq:NF:3}) hold since \emph{(i.)} if there is $\hat{\sigma}_u \in \hat{\theta}_u $ then 
$dom(\hat{\sigma})\cap dom(\hat{\sigma}_u)=\emptyset$,  and 
\emph{(ii.)} if there is ${\sigma}_u \in {\theta}_u $ then 
$dom({\sigma})\cap dom({\sigma}_u)=\emptyset$,
\end{caseinproof}

\begin{caseinproof}
If ${\wp}_{n}=\EloiseM{ {t} <{\beta};{u}}{? {\alpha}}$, then this case is similar to the previous one.
\end{caseinproof}
\end{proofbycases} 
The proof of the direction ''$\Rightarrow$''   is dual  w.r.t. the proof of 
  ''$\Leftarrow$'' This ends the proof of the Proposition.
\end{proof}




\begin{definition}
Let $\widehat{\mathcal{G}}$ be exactly the game  $\mathcal{G}$
apart that  all  fresh  renamings are
pairwise disjoint,  that is, for every fresh renamings $\rho^i_p$ and $\rho^j_q$
appearing in the positions of $\widehat{\mathcal{G}}$  we have that 
\[ codom(\rho^i_p) \cap codom(\rho^j_q)=\emptyset
\]
\end{definition}


\begin{lemma}
\label{equiv:sim:lem:1}
Let $A$ and $B$ be two \vaut{automata}. 
 There is a simulation of $A$ by $B$ (in the sense of Definition \ref{sim:def}) 
iff \Eloise has a  winning strategy 
 in the game $\widehat{\mathcal{G}}(A,B)$.
\end{lemma}
\begin{proof}
For the direction "$\Rightarrow$"  it is sufficient to notice that 
 the game theoretic definition is just a   formulation of the 
simulation given in Definition \ref{sim:def}. To be more precise, 
the choice of the fresh renaming in the simulation game $\widehat{\mathcal{G}}$ 
by \Eloise is exactly the   fresh renaming of the unfolding of the fixed-point variables.

For the  direction "$\Leftarrow$", the proof tree is infinite 
and it corresponds to playing the simulation game on the (infinite) unfolding 
of $A$ and $B$, i.e. the game $\widehat{\mathcal{G}}(\psi_{A}(A),\psi_{B}(B))$. 
 \end{proof}



\ucomment{Notice that $\bar{\gamma}$ is chosen as   $\gamma \circ \bar{\xi}$ where there exists $t_0$ and $\bar{\xi}$
and ${\xi}$ such that $\bar{\xi}(t_0)=\bar{t}$ and $\xi(t_0)=t$, since 
it follows from induction hypothesis that $\bar{t}\synch t$. 
On the one hand, from the induction hypothesis  
we have that   $\bar{u} \synch u$, $\bar{\beta}\synch \beta$, 
and $\bar{\alpha} = \alpha$. 
On the other hand,  it follows from Lemma \ref{subs:cong:lemma} that
 $\bar{\sigma} \synch \sigma$.
It remains to show that $NF_{\mathcal{S}}([\bar{\sigma}](\bar{u})) \synch NF_{\mathcal{S}}([\sigma](u))$.
That is, we need to show that there exist an expression $g_0$ and $\bar{\theta}$ and $\theta$ such that 
 $\bar{\theta}\synch \theta$ and 
\begin{align}
\label{aim:eq:NF}
\begin{cases}
 NF_{\mathcal{S}}([\bar{\theta}](g_0))  = NF_{\mathcal{S}}([\bar{\sigma}](\bar{u}))   \\
 NF_{\mathcal{S}}([\theta](g_0))  = NF_{\mathcal{S}}([\sigma](u))
\end{cases}
\end{align}
But, since $\bar{u} \synch u$ then  
there exist an expression $u_0$ and $\bar{\theta}_u$ and $\theta_u$ such that 
 $\bar{\theta}_u  \synch \theta_u$  and
\begin{align*}
\begin{cases}
 NF_{\mathcal{S}}([\bar{\theta}_{u}](u_0))  = \bar{u}  \\
 NF_{\mathcal{S}}([\theta_u](u_0))  =u
\end{cases}
\end{align*}
By replacing $\bar{u}$ and $u$ by their respective values,  the equations \ref{aim:eq:NF} become

\begin{align}
\label{aim:eq:NF:2}
\begin{cases}
 NF_{\mathcal{S}}([\bar{\theta}](g_0))  = NF_{\mathcal{S}}([\bar{\sigma}]( NF_{\mathcal{S}}([\bar{\theta}_{u}](u_0))))   \\
 NF_{\mathcal{S}}([\theta](g_0))  = NF_{\mathcal{S}}([\sigma](NF_{\mathcal{S}}([\theta_u](u_0))))
\end{cases}
\end{align}
In  order to prove the equations (\ref{aim:eq:NF:2}) it is sufficient to show that 
\begin{align}
\label{aim:eq:NF:3}
\begin{cases}
 NF_{\mathcal{S}}([\bar{\sigma}]( NF_{\mathcal{S}}([\bar{\theta}_{u}](u_0)))) =    NF_{\mathcal{S}}([\bar{\sigma} \circ \bar{\theta}_{u}](u_0)) \\
 NF_{\mathcal{S}}([\sigma](NF_{\mathcal{S}}([\theta_u](u_0))))  = NF_{\mathcal{S}}([\sigma \circ \theta_u](u_0))
\end{cases}
\end{align}
under the hypothesis  $\bar{\theta}_{u} \synch \theta_u$ and $\bar{\sigma} \synch \sigma$,
that is, by taking $\bar{\theta}=\bar{\sigma}\circ \bar{\theta}_u$, ${\theta}={\sigma}\circ {\theta}_u$, 
and $g_0=u_0$. 
But the equalities (\ref{aim:eq:NF:3}) hold since \emph{(i.)} if there is $\bar{\sigma}_u \in \bar{\theta}_u $ then 
$dom(\bar{\sigma})\cap dom(\bar{\sigma}_u)=\emptyset$,  and 
\emph{(ii.)} if there is ${\sigma}_u \in {\theta}_u $ then 
$dom({\sigma})\cap dom({\sigma}_u)=\emptyset$,
\end{caseinproof}

\begin{caseinproof}
If ${\wp}_{n}=\EloiseM{ {t} <{\beta};{u}}{? {\alpha}}$, then this case is similar to the previous one.
\end{caseinproof}
}


\ucomment{
We now consider the constraint that every  send term is  smaller  
than the received terms. 
Given a \vaut{automata} $C$, we  let  $\mycal{T}(C)$ 
be its  set of actions.
Let $\mathbb{S}(C)=\set{t, | !t \in \mycal{T}(C)}$
 (resp. $\mathbb{R}(C)=\set{t, | ?t \in \mycal{T}(C)}$)
 be the set of sent (resp. received) actions of the \vaut{automaton} $C$. 
\begin{definition}
We say that the \vaut{automaton} $C$ has the subterm property iff
 for all $t \in \mathbb{S}(C)$ such that $t$ is not a variable nor 
a constant, we have that $t\in \mathbb{R}(C)$
\end{definition}
\begin{proposition}
\label{finite:game:subterm:prop}
Let $A$ and $B$ be two \vaut{automata}. If both  $A$ and $B$ have 
the subterm property then
the game graph $\mycal{G}(A,B)_{\rho_f}$  induced by the monotonic strategy $\rho_{f}$ 
is finite.  
\end{proposition}
}


\mycomment{}{TWO  (EQUIVALENT?) DEFINITIONS, THE SECOND ONE CORRESPONDS TO THE \vaut{AUTOMATA}}
\begin{definition}
\label{vaut:2:def}
A \vaut{automaton} is a tuple $\model{S,q_0,r, \delta}$ where 
\begin{itemize}
\item $S$ is a finite set of states,
\item $q_0$ is an initial state, 
\item $r \in \mathbb{N}$,  is the number of registers,
\item $\Delta:S  \times 2^{[r]} \times ([r]\times \Sigma) \times S$ is the transition relation.
\end{itemize}
\end{definition}


\begin{definition}
\label{vaut:2:def}
A \vaut{automaton} is a tuple $\model{S,q_0,r,\rho, \delta}$ where 
\begin{itemize}
\item $S$ is a finite set of states,
\item $q_0$ is an initial state, 
\item $r \in \mathbb{N}$,  is the number of registers,
%% \item $u=w_1w_2\ldots w_r \in (\Sigma\cup \set{\sharp})^r$ is an assignment
%%    of registers. 
\item $\rho: S \rTo 2^{[r]}$ is called the reinitialization function, 
 % It is meaning is, 
\item $\Delta:S  \times ([r]\times \Sigma) \times S$ is the transition relation.
\end{itemize}
\end{definition}

\begin{definition}
\label{coherence:def}
 Let $C \subseteq \Sigma_0$ be a  finite set of constant symbols. 
 We define the coherence relation $\synch_{C}$ with respect 
 to $C$ between substitutions, behavior expressions, and game positions as follows.   
\begin{itemize}
\item If $\bar{\sigma}$ and $\sigma$ are two ground substitutions with $codom(\sigma) \cup codom(\bar{\sigma}) \subseteq \Sigma_0$,
 then    $\bar{\sigma} \synch_{_{C}} \sigma$ 
iff the three following conditions hold:
\begin{enumerate}
\item $dom(\bar{\sigma}) = dom(\sigma)$,
\item If $\bar{\sigma}(x) \in C$ then  $\bar{\sigma}(x)=\sigma(x) $, and  
     if  $\sigma(x) \in C$, then $\bar{\sigma}(x)=\sigma(x) $, for any variable $x \in dom(\sigma)$, and 
   \item for any variables $x,y \in  dom(\sigma)$,  $\bar{\sigma}(x)=\bar{\sigma}(y)$ iff $\sigma(x)=\sigma(y)$.
\end{enumerate} 
\item If $\bar{t}$ and $t$ are behavior expressions with substitutions, then
   $\bar{t}$ $\synch_{C} t$  iff there exist
    two substitutions $\bar{\sigma},\sigma$ and a behavior expression
    $t_0$ such that $\bar{\sigma} \synch_{C} \sigma$ and $NF_{\Eu{S}}([\bar{\sigma}](t_0))=\bar{t}$ and 
  $NF_{\Eu{S}}([\sigma](t_0))=t$.  
\item Let $t=NF_{\Eu{S}}([\sigma_t](t_0))$, $\bar{t}=NF_{\Eu{S}}([\bar{\sigma}_t](t_0))$, 
    $u=NF_{\Eu{S}}([\sigma_u](u_0))$, and  $u=NF_{\Eu{S}}([\bar{\sigma}_u](u_0))$ be behavior expressions  such that 
    $dom(\sigma_{t}) \cap dom(\sigma_{u})=\emptyset$ and 
   $dom(\bar{\sigma}_{t}) \cap dom(\bar{\sigma}_{u})=\emptyset$. 
   Then, 
   \begin{itemize} 
   \item  $\AbelardM{\bar{t}< \bar{u}} \synch_{C} \AbelardM{t<u}$ iff $\bar{t}\synch_{C} t$ and $\bar{u} \synch_{C} u$, and 
     $(\sigma_t \uplus \sigma_u )(x)= (\sigma_t \uplus \sigma_u )(y)$ iff  
     $(\bar{\sigma}_t \uplus \bar{\sigma}_u )(x)= (\bar{\sigma}_t \uplus \bar{\sigma}_u )(y)$.
   \item  $\EloiseM{\bar{t}< \bar{u}}{\bar{\alpha}} \synch_{C} \EloiseM{t<u}{\alpha}$ iff 
   $\AbelardM{(\bar{\alpha}; \bar{t})< \bar{u}} \synch_{C} \AbelardM{(\alpha;t)<u}$. 
   \end{itemize} 
\end{itemize}
\end{definition}



\begin{proposition}
\label{sigma:finite:prop}
Let $A,B$ be FVAs such that all the actions of $A,B$ are either constants or variables.
That is, the actions are taken from $\overline{\mycal{T}}(\Sigma_0,\mycal{X})$, where 
$\Sigma_0$ is an enumerable infinite set of constant symbols. 
 Then \Eloise has a 
 winning strategy in $\mathcal{G}(A,B)$ iff she 
has a $\sigma$-{finite}  winning strategy in $\mathcal{G}(A,B)$.
\end{proposition}
\begin{proof}
We can assume without loss of generality that $var(A)\cap var(B)=\emptyset$.
We let 
\begin{align*}
C_0= \Sigma_0(A) \cup \Sigma_0(B) \cup c_{var(A) \times  var(B)} \cup c_{var(B) \times var(A)}
\end{align*}
We assume  that $(c_{var(A)\times var(B)} \cup c_{var(A) \times var(B)}) \cap \Sigma_0=\emptyset$.
Let  $\overline{\mycal{G}}(A,B)$ be the game  played  as the game $\mycal{G}(A,B)$ 
apart that \Eloise (in the rule \ttt{E!-comp}) and 
 \Abelard  (in the rule \ttt{E?}) must instantiate the variables from $C_0$.
 We shall  show that
\Eloise has a  winning strategy in ${\mycal{G}}(A,B)$ iff she has 
a  winning strategy in $\overline{\mycal{G}}(A,B)$. 
For the direction "$\Rightarrow$"  we show that out of a  winning strategy 
of \Eloise   in ${\mycal{G}}(A,B)$ we construct a  winning strategy 
for her in $\overline{\mycal{G}}(A,B)$.
  For this purpose, we shall  show that each move of \Abelard in  
$\overline{\mycal{G}}(A,B)$ can be  mapped to an   \Abelard move in $\mycal{G}(A,B)$, 
and   \Eloise response in $\mycal{G}(A,B)$ can be actually  mapped  to 
an  \Eloise move in $\overline{\mycal{G}}(A,B)$.
This mapping defines a relation \footnote{More precisely, if $(\bar{\wp},\wp) \in \mycal{R}$, 
 and the move $\bar{\wp}\uberTo{\overline{\mycal{G}}}\bar{\wp}'$ is mapped to $\wp \uberTo{\mycal{G}} \wp'$, 
  or  $\wp \uberTo{\mycal{G}} \wp'$ is mapped to $\bar{\wp}\uberTo{\overline{\mycal{G}}}\bar{\wp}'$, 
 then $(\bar{\wp}',\wp') \in \mycal{R}$} 
$\mycal{R} \subseteq \Pos_{E}(\overline{\mycal{G}}(A,B) \times \Pos_{E}(\mycal{G}(A,B)) \cup 
  \Pos_{A}(\overline{\mycal{G}}(A,B) \times \Pos_{A}(\mycal{G}(A,B))$. 
 Furthermore, we impose that the following invariant holds:
\begin{align}
\label{invariant-sim}
\tag{Inv-$\synch$}
\textrm{If }  (\bar{\wp}, \wp) \in  \mycal{R}  
  \textrm{ then } \bar{\wp} \synch \wp.
\end{align}
The $\synch$-coherence is always with respect to $\Sigma_{0}(A)\cup \Sigma_{0}(B)$,
and we shall simply write  ``$\synch$" instead of ``$\synch_{\Sigma_{0}(A)\cup \Sigma_{0}(B)}$". 
  The proof is by induction on the number  of the  moves  
 made in $\overline{\mycal{G}}(A,B)$  plus the number of moves made in  ${\mycal{G}}(A,B)$.
The base case trivially holds  since the two  starting positions of 
$\overline{\mycal{G}}(A,B)$ and $\mycal{G}(A,B)$ are equal.  They are of the form 
$\AbelardM{X_0<Y_0}$ and  the rule \ttt{A-L}$\mu$ is applied.
For the induction case let $(\bar{\wp}_n,\wp_n) \in \mycal{R}$.  
We consider two possibilities: when both $\bar{\wp}_n$ and 
 $\wp_n$  are  \Abelard positions  and when they are \Eloise positions. 
 Consider  the first  possibility and an  \Abelard move $\bar{\wp}_n \uberTo{} \bar{\wp}_{n+1}$ in 
  $\overline{\mycal{G}}(A,B)$. 
 We distinguish many cases according to the 
structure of $\bar{\wp}_n$.

\begin{proofbycases}
\begin{caseinproof}
The cases when   
$\bar{\wp}_{n}=\AbelardM{\bar{t}_1 \lor \bar{t}_2 <\bar{u}}$, 
$\bar{\wp}_{n}=\AbelardM{[\bar{\sigma}](X)< u }$, and 
$\bar{\wp}_{n}=\AbelardM{[\bar{\sigma}](\nu y. \bar{t} )< u }$
 are straightforward, since the related positions are of the form 
${\wp}_{n}=\AbelardM{{t}_1 \lor {t}_2 <{u}}$, 
${\wp}_{n}=\AbelardM{[{\sigma}](X)< u }$, and 
${\wp}_{n}=\AbelardM{[{\sigma}](\nu y. {t} )< u }$, respectively, 
the rules \texttt{A-}$\lor$,  and \texttt{A-L}$_\mu$ and \texttt{A-L}$_\nu$  are applied respectively. 
Hence the move in  $\mycal{G}(A,B)$ is the same as the move 
  $\bar{\wp}_n \uberTo{} \bar{\wp}_{n+1}$ and the invariant \ref{invariant-sim} is maintained.
\end{caseinproof}



\begin{caseinproof}
If  $\bar{\wp}_{n}=\AbelardM{?\bar{a};\bar{t}<\bar{u}}$, and 
 \begin{align*}
  \AbelardM{(?\bar{a};\bar{t})<\bar{u}} \uberTo{\ttt{A?-Comp}} \EloiseM{\bar{t}<\bar{u}}{?\bar{a}} 
 \end{align*}
is a move in $\overline{\mycal{G}}(A,B)$ then,  
 since  $\bar{\wp}_n \synch \wp_n$  then    ${\wp}_{n}=\AbelardM{(?a;{t})<{u}}$
where  $(?\bar{a};\bar{t}) \synch (?a;{t})$ and $\bar{u} \synch u$.
 \Abelard   move in $\mycal{G}(A,B)$ is 
 \begin{align*}
  \AbelardM{(?{a};{t})<{u}} \uberTo{\ttt{A?-Comp}} \EloiseM{{t}<{u}}{?{a}}, 
 \end{align*}
 and invariant (\ref{invariant-sim}) is trivially maintained.
\end{caseinproof}

%\mycomment{The first critical case}{}
\begin{caseinproof}
If  $\bar{\wp}_{n}=\AbelardM{(!\bar{a};\bar{t})<\bar{u}}$, 
 then the only relevant situation is when $\bar{a}$ is a variable $x$; the case 
 when $\bar{a}$ is a constant  is similar to the previous case. Hence,  
 \begin{align*}
  \AbelardM{(!x;\bar{t})<\bar{u}} \uberTo{\ttt{A!-Comp}} \EloiseM{[\bar{\gamma}](\bar{t})<\bar{u}}{[\bar{\gamma}](!x)} 
\uberTo{\Eu{S}^*} \EloiseM{NF_{\Eu{S}}([\bar{\gamma}](\bar{t}))<{u}}{[\gamma](!x)}   
 \end{align*}
is a move in $\overline{\mycal{G}}(A,B)$ and since $\bar{\wp_{n}} \synch \wp_n$ 
  by (\ref{invariant-sim})  then    ${\wp}_{n}=\AbelardM{!{a};{t}<{u}}$
where   $(!x;\bar{t}) \synch (!a;{t})$ and $\bar{u} \synch u$. It follows  from the Remark  \ref{synch:req}
 that $x \synch a$ and $\bar{t} \synch t$ and therefore $x=a$.
The corresponding \Abelard move in $\mycal{G}(A,B)$ results from the following derivations: 
\begin{align*} 
 \wp_n=\AbelardM{{(!x;{t})<{u}}} \uberTo{\ttt{A!-Comp}} \EloiseM{[\gamma](t)<{u}}{[\gamma](!x)}  \uberTo{\Eu{S}^*} \EloiseM{NF_{\Eu{S}}([\gamma](t))<{u}}{[\gamma](!x)}=\wp_{n+1}
\end{align*}  
And  \Abelard choice of $\gamma$
depends on the nature of $\bar{\gamma}(x)$.
\begin{itemize}
\item  If $\bar{\gamma}(x)\in \Sigma_{0}(t) \cup \Sigma_{0}(u)$ then in this case
   we let $\gamma:=\bar{\gamma}$,  and hence  the invariant \ref{invariant-sim} is trivially  maintained.
\item  If $\bar{\gamma}(x)  \in  (\cons{\bar{t}} \cup \cons{\bar{u}}) \setminus (\Sigma_{0}(A) \cup \Sigma_{0}(B))$. 
 Since $\bar{t}\synch t$ and $\bar{u}\synch u$, then  there exist $t_0,u_0,\sigma_t, \sigma_u, \bar{\sigma}_t,\bar{\sigma}_u$
such that $\bar{\sigma}_u \synch \sigma_u$ and $\bar{\sigma}_u \synch \sigma_u$ and 
\begin{align*}  
\begin{cases}
\bar{t}=NF_{\Eu{S}}([\bar{\sigma}_t](t_0)) \\
{t}=NF_{\Eu{S}}([{\sigma}_t](t_0)) 
\end{cases}
\; \tand \;
\begin{cases}
\bar{u}=NF_{\Eu{S}}([\bar{\sigma}_u](u_0)) \\
{u}=NF_{\Eu{S}}([{\sigma}_u](u_0)) 
\end{cases}
\end{align*}
Since the constant $\bar{\gamma}(x)$ figures  in the current position, then there is a variable $y$ such that
 $\big(y \mapsto \bar{\gamma}(x)\big) \in \bar{\sigma}_t \uplus \bar{\sigma}_u$. From the definition of  $\synch$ over the 
set of positions Def. \ref{coherence:def} item 3, 
it follows that there is a variable $y$ and a constant $y_0$ such that  $\big(y \mapsto y_0 \big) \in {\sigma}_t \uplus {\sigma}_u$.
Thus we let $\gamma:=\set{x \mapsto y_0}$ and the invariant is maintained.  
\item  Otherwise, i.e. $\bar{\gamma}(x)$ is a new constant that does not appear in the current position,
      then we take $\gamma(x)$ as a new constant as well.
Finally, notice   that the invariant \ref{invariant-sim} is maintained.  
%% One the one hand,  there exist $t_0,\bar{\sigma}, \sigma_0$ such that  $\bar{t}=NF_{\Eu{S}}([\bar{\sigma}_0](t_0))$, 
%%   ${t}=NF_{\Eu{S}}([{\sigma}_0](t_0))$ and $\bar{\sigma}_0 \synch \sigma_0$.
%%  On the other hand, 
%%   $x\notin \bar{\sigma}_0 \cup \sigma_0$,  therefore  $\bar{\gamma} \circ \bar{\sigma}_0 \synch \gamma \circ \sigma_0$.  
\end{itemize}
\end{caseinproof}
\end{proofbycases}


Secondly, we  consider  the second   possibility:  when 
 both $\bar{\wp}_n$ and 
 $\wp_n$  are  \Eloise positions.
We consider an  \Eloise move ${\wp}_n \uberTo{} {\wp}_{n+1}$ in 
  ${\mycal{G}}(A,B)$ that has to be mapped to an \Eloise move in   $\overline{\mycal{G}}(A,B)$. 
 We distinguish many cases according to the 
structure of $\wp_n$.

\begin{proofbycases}
\begin{caseinproof}
The cases when   
${\wp}_{n}=\EloiseM{u < u_1 \lor u_2}{\alpha}$, 
${\wp}_{n}=\EloiseM{t<[{\sigma}](X)}{\alpha}$, and 
${\wp}_{n}=\EloiseM{t<[{\sigma}](\nu y. {u} )}{\alpha}$
 are straightforward, since 
the rules \texttt{E-}$\lor$,  and \texttt{E-R}$_\mu$ and \texttt{E-R}$_\nu$  are applied respectively. Hence
the move in  $\bar{\mycal{G}}(A,B)$ is the same as the move 
  ${\wp}_n \uberTo{} {\wp}_{n+1}$ and the invariant \ref{invariant-sim} is maintained.
\end{caseinproof}

\ucomment{
\begin{caseinproof}
If ${\wp}_{n}=\EloiseMM{ [{\theta}](X_i) <{u}}$, then in this case
the move $\wp_n \uberTo{} \wp_{n+1}$ results from the  derivations 
\begin{align*}
\AbelardM{ [\theta](X_i) <{u}} \uberTo{\texttt{E-L}_{\mu}} \AbelardM{ [{\theta}](S_i) <{u}} 
 \uberTo{\Eu{S}^*} \AbelardM{ NF_{\mathcal{S}}([{\theta}](S_i))  <{u}}=\wp_{n+1}
\end{align*} 
 and its  related derivations in  $\overline{\mycal{G}}(A,B)$  are
\begin{align*}
\AbelardM{ [\bar{\theta}](X_i) <\bar{u}} \uberTo{\texttt{E-L}_{\mu}} \AbelardM{ [\bar{\theta}](S_i) <\bar{u}}
\uberTo{\Eu{S}^*}    \AbelardM{NF_{\mathcal{S}}([\bar{\theta}](S_i)) <\bar{u}}=\bar{\wp}_{n+1}
\end{align*} 

From the induction hypothesis we have that $\bar{\theta}\synch \theta$ and  $\bar{u} \synch u$.
Therefore $\bar{\wp}_{n+1} \synch \wp$. 
\end{caseinproof}


\begin{caseinproof}
The case  when ${\wp}_{n}=\EloiseM{ {t} < [{\theta}](X_i)}{a}$ is  the same as  the previous 
one apart that  the rule \ttt{E-R}$_{\mu}$ is applied instead of  \ttt{E-L}$_{\mu}$ .
\end{caseinproof}
}



\begin{caseinproof}
If ${\wp}_{n}=\EloiseM{ {t} < (\beta;u)}{! {\alpha}}$, then recall that $\alpha$ is a constant, and 
  in this case  the  move  $\wp_{n}\uberTo{} \wp_{n+1}$ in 
 $\mycal{G}(A,B)$  results from the derivations:
\begin{align*}
\wp_{n}=\EloiseM{{t} <({\beta};{u})}{! {\alpha}} \uberTo{\ttt{E!}} \AbelardM{(t)<{[\sigma]}({u})} \uberTo{\Eu{S}^*} 
  \AbelardM{{t}<{NF_{\Eu{S}}([\sigma]({u}))}}=\wp_{n+1}, \;\;
\textrm{ where } \sigma = \match{\beta}{\gamma(\alpha)}
\end{align*}
From the induction hypothesis we have that $\bar{\wp}_{n} \synch \wp_{n}$, therefore
 $\bar{\wp}_{n}= \EloiseM{\bar{t} <(\bar{\beta};\bar{u})} {! \bar{\alpha}}$
such that $(!\bar{\alpha};\bar{t}) \synch (!\alpha;t) $ and $(\bar{\beta};\bar{u}) \synch (\beta;u)$.
Hence $\bar{\alpha} \synch \alpha$, $\bar{\beta} \synch  \beta$, $\bar{t} \synch t$ and $\bar{u} \synch  u$.
We now argue that the following   derivations  
\begin{align*}
  \bar{\wp}_{n}=\EloiseM{\bar{t} <(\bar{\beta};\bar{u})}{! \bar{\alpha}} \uberTo{\ttt{E!}} 
  \AbelardM{\bar{t}<[\bar{\sigma}](\bar{u})}
  \uberTo{\Eu{S}^*} \AbelardM{\bar{t}<{NF_{\Eu{S}}([\bar{\sigma}]({\bar{u}}))}}=\bar{\wp}_{n+1}, \\ 
\textrm{ where } \bar{\sigma}= \match{\bar{\beta}}{\bar{\alpha}}
\end{align*}
are possible in  $\overline{\mycal{G}}(A,B)$ and that the invariant \ref{invariant-sim} is maintained.
That is,  we must show that the matching
 problem $\matchq{\bar{\beta}}{\bar{\alpha}}$ has a (possibly trivial) solution and that 
$[\bar{\sigma}](\bar{u})  \synch  [{\sigma}](u)$. Notice that   maintaining   the invariant 
 does only  make sense when $\beta$ and  $\bar{\beta}$ are variables. We distinguish 
 two  cases according to the nature of $\beta$:
 \begin{itemize}  
   \item If $\beta$ is a variable $x$, then $\bar{\beta}=\beta$ since $\bar{\beta} \synch \beta$. 
      Let  $u=NF_{\Eu{S}}([\sigma_u](u_0))$,  $\bar{u}=NF_{\Eu{S}}([\bar{\sigma}_u]({u}_0))$, 
        $t=NF_{\Eu{S}}([\sigma_t](t_0))$ and $\bar{t}=NF_{\Eu{S}}([\bar{\sigma}_t]({t}_0))$.
     Notice that $x \notin  dom(\sigma_u) \cup dom(\bar{\sigma}_u)$. We must show 
     now that $[\set{ x \mapsto \bar{\alpha}} \uplus \bar{\sigma}_u ]  \synch [\set{ x \mapsto {\alpha}} \uplus {\sigma}_u]$
     and $[\set{ x \mapsto \bar{\alpha}} \uplus \bar{\sigma}_u \uplus \bar{\sigma}_t ] 
       \synch [\set{ x \mapsto {\alpha}} \uplus {\sigma}_u \uplus \sigma_t]$.
     This depends on $\alpha$: 
     \begin{itemize}
     \item If $\alpha$ is constant in $\Sigma_0(A)\cup \Sigma_0(B)$, then 
      $\bar{\alpha}= \alpha$  since $\bar{\alpha}\synch \alpha$, and  we are done. 
     \item  If $\alpha$ is a constant that came from a reduction of  $[y \mapsto \alpha](y)$, for some variable $y$.
      Then, $\bar{\alpha}$ is also a constant that came from the reduction of  $[y \mapsto \bar{\alpha}](y)$, and in this 
     case  $[y \mapsto \bar{\alpha}] \in \bar{\sigma}_t$ and $[y \mapsto \alpha] \in \sigma_t$.
This shows that  
$[\set{ x \mapsto \bar{\alpha}} \uplus \bar{\sigma}_t ] 
       \synch [\set{ x \mapsto {\alpha}}  \uplus \sigma_t]$. 
       %   appear in $(\alpha;t)$ (resp. in $(\bar{\alpha};\bar{t})$). 
       If there is another $[z \mapsto \alpha]$ in $\sigma_u$, then there must be $[z \mapsto \bar{\alpha}]$ in $\bar{\sigma}_u$ 
       since $[ \bar{\sigma}_u \uplus \bar{\sigma}_t ] \synch [ {\sigma}_u \uplus \sigma_t]$.
       Hence, $[\set{ x \mapsto \bar{\alpha}} \uplus \bar{\sigma}_u ]  \synch [\set{ x \mapsto {\alpha}} \uplus {\sigma}_u]$, 
       and $[\set{ x \mapsto \bar{\alpha}} \uplus \bar{\sigma}_u \uplus \bar{\sigma}_t ] 
       \synch [\set{ x \mapsto {\alpha}} \uplus {\sigma}_u \uplus \sigma_t]$.
     \end{itemize} 
   \item If $\beta$ is a constant,  then  $\beta = \alpha$. 
     We distinguish two cases depending on $\alpha$: 
     \begin{itemize}
     \item If $\alpha$ is constant in $\Sigma_0(A)\cup \Sigma_0(B)$ and so $\beta$, then on the one hand, $\bar{\alpha}=\alpha$, 
       since $\bar{\alpha}\synch \alpha$, and on the other hand,
       $\bar{\beta}=\beta$ since $\bar{\beta} \synch \beta$.
       Therefore $\bar{\alpha}=\bar{\beta}$, and we are done. 
        \item  If $\alpha$ is a constant that came from a reduction $[y \mapsto \alpha](y)$, for some variable 
           $y$ where $\alpha \notin \Sigma_0(A)\cup \Sigma_0(B)$, then  in this case $\beta$  came also from 
            a reduction $[z \mapsto \alpha](z)$, for some variable  $z$, since $\beta=\alpha$. 
             Notice that, on the one hand,  $\set{y \mapsto \alpha, z \mapsto \alpha}$ appears in the 
             position $\wp_{n}$.  On the other hand, $\bar{\beta}=[z\mapsto \bar{\beta}](z)$ and $\bar{\alpha}=[y\mapsto \bar{\alpha}](y)$, 
              since $\bar{\beta} \synch \beta$ and $\bar{\alpha} \synch \alpha$.
              Therefore, $\set{y \mapsto \bar{\beta}, z \mapsto \bar{\alpha}}$ appears in the position $\bar{\wp}_{n}$, and hence
                $\bar{\beta}=\bar{\alpha}$, since $\bar{\wp_n} \synch \wp_n$.
     \end{itemize}
     
 \end{itemize}
\end{caseinproof}

\begin{caseinproof}
If ${\wp}_{n}=\EloiseM{ {t} <{\beta};{u}}{? {\alpha}}$, then in this case we have the  move  $\wp_{n}\uberTo{} \wp_{n+1}$ in 
$\mycal{G}(A,B)$ that results from the derivations:
\begin{align*}
  \wp_{n}=\EloiseM{({t} <{\beta};{u})}{? {\alpha}} \uberTo{\ttt{E?}} \AbelardM{[\sigma](t)<{[\gamma]}({u})} \uberTo{\Eu{S}^*} 
\AbelardM{NF_{\Eu{S}}([\sigma]{t})<{NF_{\Eu{S}}([\gamma]({u}))}}=\wp_{n+1},  \\
\textrm{ where } \sigma = \match{\beta}{\gamma(\alpha)}
\end{align*}
From the induction hypothesis we have that $\bar{\wp}_{n} \synch \wp_{n}$, therefore
 $\bar{\wp}_{n}= \EloiseM{\bar{t} <(\bar{\beta};\bar{u})} {? \bar{\alpha}}$
such that $(?\bar{\alpha};\bar{t}) \synch (?\alpha;t) $ and $(\bar{\beta};\bar{u}) \synch (\beta;u)$.
Hence $\bar{\alpha} \synch \alpha$, $\bar{\beta} \synch  \beta$, $\bar{t} \synch t$ and $\bar{u} \synch  u$.
We now argue that the following   derivations:  
\begin{align*}
  \bar{\wp}_{n}=\EloiseM{(\bar{t} <\bar{\beta};\bar{u})}{? \bar{\alpha}} \uberTo{\ttt{E?}} 
 \AbelardM{[\bar{\sigma}](\bar{t})<[\bar{\gamma}](\bar{u})}
    \uberTo{\Eu{S}^*} \AbelardM{NF_{\Eu{S}}[\bar{\sigma}](\bar{t})<{NF_{\Eu{S}}([\bar{\gamma}]({\bar{u}}))}}=\bar{\wp}_{n+1}
\end{align*}

are possible in  $\overline{\mycal{G}}(A,B)$, 
where  $ \bar{\sigma}= \match{\bar{\beta}}{\bar{\gamma}(\bar{\alpha})}$, 
and  the choice of $\overline{\gamma}$ depends on $\alpha$. Besides, we show that the invariant (\ref{invariant-sim}) is 
  maintained. Maintaining this invariant does make sense only when $\alpha$ or $\beta$ is a variable. 
\begin{itemize}
\item If $\alpha$ is a constant that came from a reduction of $[y \mapsto \alpha](y)$, for some variable $y$,  where 
    $\alpha \notin \Sigma_{0}(A) \cup \Sigma_0(B)$. The case when $\alpha \in \Sigma_{0}(A) \cup \Sigma_0(B)$ 
  is trivial. We distinguish two cases. 
  \begin{itemize}
  \item If $\beta$ is a constant then in this case   
    $\beta=\alpha$, and  hence $\gamma=\sigma=\emptyset$. We take 
    $\bar{\gamma}=\bar{\sigma}=\emptyset$.
    On the one hand, $\beta$ came from a reduction  $[x\mapsto \alpha](x)$, and  
     $\bar{\beta}$ came from a reduction  $[x\mapsto \bar{\beta}](x)$, for some variable $x$, since
      $\bar{\beta} \synch \beta$. 
    On the one hand, $\alpha$ came from a reduction  $[y \mapsto \alpha](y)$, and  
     $\bar{\alpha}$ came from a reduction  $[y \mapsto \bar{\alpha}](y)$, for some variable $y$, since
      $\bar{\alpha} \synch \alpha$. Therefore, $\set{x\mapsto \alpha, y\mapsto \alpha}$ 
    (resp. $\set{x\mapsto \bar{\beta}, y\mapsto \bar{\alpha}}$) appears 
    in the position $\wp_n$ (resp. $\bar{\wp}_n$), hence $\beta=\alpha$, since $\bar{\wp}_n \synch \wp_n$.
  \item If $\beta$ is a variable $x$ then, $\bar{\beta}=\beta$, since $\bar{\beta} \synch \beta$. 
 In this case   we have $\gamma=\set{x \mapsto \alpha}$ and $\sigma=\emptyset$.
   Thus we take $\bar{\gamma}=\set{x \mapsto \bar{\alpha} }$.  
  And the invariant (\ref{invariant-sim}) is maintained.
  \end{itemize}
\item If $\alpha$ is a variable $x$ then $\bar{\alpha}=\alpha$.   We distinguish two cases  
  depending on the nature of $\beta$. 
  \begin{itemize}
  \item If $\beta$ is a constant  then $\bar{\beta}$ is a constant as well since $\bar{\beta} \synch \beta$. 
  In this case  $\gamma=\emptyset$     and $\sigma=\set{x \mapsto \beta}$.  Therefore we take
    $\bar{\gamma}=\emptyset$ and $\bar{\sigma}=\set{x  \mapsto \bar{\beta} }$.
  \item  If $\beta$ is a variable $y$ then   $\beta=\bar{\beta}$ since $\bar{\beta} \synch \beta$.
   Assume that ${\gamma}=\set{y \mapsto y_0}$, where $y_0$ is a constant. In this case 
     $\bar{\gamma}=\set{y \mapsto \bar{y}_0}$, and the choice   of the constant 
  $\bar{y}_0$  depends on $y_0$.
  \begin{itemize}
  \item If $y_0  \in \Sigma_0(t)\cup \Sigma_0(u)$  then we let $\bar{y}_0:=y_0$.
  \item If $y_0 \in \cons{\wp_n}  \setminus \big(\Sigma_0(t)\cup \Sigma_0(u)\big)$ then  
    there must exist a variable $z$ and a constant $z_0$ such that $(z \mapsto y_0) \in \wp_n$ and 
      $(z \mapsto z_0) \in \bar{\wp}_n$. 
      We  let  $ \bar{y}_0:=z_0$.
 \item Otherwise, i.e. $y_0$ is a fresh constant that does not appear in $\wp_n$, 
  then  $\bar{y}_0$  must be a fresh constant  as well. 
Since $|\cons{\bar{\wp}_n}| \le (|var(A)|-1)+(|var(B)|-1) < |C_0|$ then 
   $\cons{\bar{\wp}_n} \subsetneq C_0$. 
   Hence we take $\bar{y}_0$ as an arbitrary  
   element of the non empty  set $C_0 \setminus \cons{\bar{\wp}_n}$.
  \end{itemize}
\end{itemize}
\end{itemize}
\end{caseinproof}
\end{proofbycases} 
The proof of the direction ''$\Leftarrow$''   is dual  w.r.t. the proof of the direction
 ''$\Rightarrow$''. That is,  it can be obtained by replacing \Eloise by \Abelard, 
  and \Abelard by \Eloise and keeping the same definition of the $\synch$-coherence.
 This ends the proof of the proposition.
\end{proof}




\begin{lemma}
\label{refresh:once:vaut:lemma}
Let $A=\model{\Sigma,\mathcal{X},Q,Q_0,\delta,F,\kappa}$ be a 
FVA. There exists a  FVA 
$B=\model{\Sigma,\mathcal{X}',Q',Q'_0,\delta',F',\kappa'}$ that 
recognizes the same language 
such that the variables of $B$ are refreshed at most at one state,
that is, for all $x \in \mathcal{X}'$ we have that  $|\kappa'(x)|\le 1$.
\end{lemma}
This lemma can be shown by renaming bound variables (bound w.r.t. $\nu$) thanks  
 to the mechanism of  $\alpha$-conversion 
 in the equational system of $A$, like in the $\lambda$-calculus
 where the operator "$\nu$" behaves like the "$\lambda$".  
\red{\textsc{Attention: il faut tenir  en compte la recursion.} }



\begin{example}
  Consider the FVA $\mycal{A}$ of Ex. ~\ref{semantics:var:example}  depicted in
  Fig.~\ref{vautomata:fig:1}.  \\ 
The word $!a\, !f(a,a)\, ?g(a)  \, !f(c,d)$ is recognized by $A$.
\end{example}


\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=2cm, bend angle=60,
   on grid,auto, initial text=, >=stealth] 
   \node[state,initial,accepting] (r_0)   {$p_0$}; 
   \node[state] (r_1) [right =of r_0] {$p_1$}; 
    \path[->] 
    (r_0) [bend left] edge   node [above] {$x$} (r_1)
    (r_1) [bend left] edge  node  [below] {$x$} (r_0);
\end{tikzpicture}
\end{center}


%% \begin{example}
%% Here is a more subtle example .... 
%% \begin{center}
%% \begin{tikzpicture}[shorten >=1pt,node distance=2cm, bend angle=30,
%%    on grid,auto, initial text=, >=stealth] 
%%    \node[state,initial,accepting] (p_0)   {$p_0$}; 
%%    \node[state] (p_1) [below left =of p_0] {$p_1$}; 
%%    \node[state] (p_2) [below right =of p_0] {$p_2$}; 
%%    \node[state,accepting] (p_3) [below right =of p_1] {$p_3$}; 

%%     \path[->] 
%%     (p_0)  edge   node [above] {y} (p_1)
%%     (p_0)  edge  node  [above] {y} (p_2)
%%     -- (1,-2) node {$A$};

%%   \begin{scope}[xshift=4cm, yshift=0cm,node distance=2cm]
%%    \node[state,initial,accepting] (q_0)   {$q_0$}; 
%%     \path[->] 
%%     (q_0) [loop above] edge   node [left] {y} ()
%%     -- (0,-2.3) node {$B$};
%%   \end{scope}

%%   \begin{scope}[xshift=6cm, yshift=0cm,node distance=2cm]
%%    \node[state,initial,accepting] (r_0)   {$r_{0,0}$}; 
%%    \node[state] (r_1) [right =of r_0] {$r_{1,0}$}; 

%%     \path[->] 
%%     (r_0) [bend left] edge   node [above] {$a$} (r_1)
%%     (r_1)  edge  node  [below] {$xy$} (r_0)
%%     -- (1,-2) node {$A \cap B$};
%%  \end{scope}

%% \end{tikzpicture}
%% \end{center}
%% \end{example}



Let $A$ be the following  BFVA, where 
$\kappa(x)=\set{p_0,p_1}$ and $\kappa(y)=\emptyset$.
%\begin{figure}[h*]
\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=2cm, bend angle=60,
   on grid,auto, initial text=, >=stealth] 
   \node[state,initial] (p_0)   {$p_0$}; 
   \node[state] (p_1) [right =of p_0] {$p_1$}; 
   \node[state,accepting](p_2) [right =of p_1] {$p_2$};

    \path[->] 
    (p_0) edge [loop above]  node [above] {x} ()
    (p_0) edge  node   {y} (p_1)
    (p_1) edge  [loop above] node [above] {x}  ()
    (p_1) edge  node [above] {y} (p_2);
\end{tikzpicture}
\end{center}
\caption{A BFVA not closed under complementation.}
\label{non-comlement:example:fig}
\end{figure}

\begin{definition}
\label{sim:def}
Let  $A$ and $B$ be  two FVAs and let $\psi_A(A)$ and $\psi_B(B)$ 
be their respective unfolding. A relation $R\subseteq Q(\psi_A(A)) \times Q(\psi_B(B))$ 
is a \gsim{simulation} if whenever $pRq$ then 
\begin{itemize}
\item If $p  \stackrel{!\alpha}{\rTo} p'$ then   for all  ground substitutions $\gamma$,  
$\exists q' : q \stackrel{?\beta}{\rTo} q'$ such that  $\matchq{\beta}{\gamma(\alpha)}$ 
 and $\gamma(p') R \sigma(q')$ where   $\sigma= \match{\beta}{\gamma(\alpha)}$.
\item If $p  \stackrel{?\alpha}{\rTo} p'$ then   there is  a ground substitution $\gamma$ and  
$\exists q' : q \stackrel{!\beta}{\rTo} q'$ such that  $\matchq{\alpha}{\gamma(\beta)}$ 
 and $\sigma(p') R \beta(q')$ where   $\sigma= \match{\alpha}{\gamma(\beta)}$.
\end{itemize}
where  $\sigma(p)$  stands for the application of $\sigma$ to 
 the subtree (of $\psi_{A}(A)$  or $\psi_B(B)$) rooted at $p$. 
\end{definition}


We define the relation of \gsim{simulation} in two equivalent ways. The first one
 is formulated in terms  of the infinite   unfolding of the  
FVAs. From this formulation it is not easy to study the  
 decidability of  the \gsim{simulation}. 

\begin{definition}
A strategy for \Eloise in $\mycal{G}(A,B)$ is  $\mycal{I}$-finite, if 
she instantiates the variables from a finite set of constants. 
That is, there is a finite set $C_0$ of constant symbols  such that 
 the co-domain of the substitution $\gamma$ in the  rules \ttt{E!} 
and \ttt{E?} is a subset of $C_0$.
\end{definition}

\subsection{Delayed communication}
\label{asynch:comm:sec}
Unlike the synchronous communication, we consider here the possibility
that the services   can communicate with each others and letting 
 the client to wait.  The only requirement that  must be fulfilled is that the client has not to 
 wait for ever.  
In other words, the simulation should be able to suitably
schedule   the available services and  provide the target service to the client.



In the following, $u_i$ are  behavior expressions, 
 the derivation rules that appear in the conditions  
correspond to the rules of the   \gsim{simulation} (see Figure \ref{sim:game:rule:fig}).
In the first rule the arrow "$\uberTo{\star}{}$" stands for an iteration  of the rules  
\ttt{A-L}$_{\mu}$, \ttt{A-L}$_{\nu}$ and \ttt{A}-$\lor$. 
And in the second rule, it stands for an iteration of \ttt{E-L}$_{\mu}$, \ttt{E-L}$_{\nu}$ and \ttt{E}-$\lor$. 


\begin{align*}
& \frac{\EloiseM{ u_0 \oplus \cdots \ u'_i  \cdots u'_j \cdots \oplus u_n}{(\alpha,i)}}
     {\AbelardM{ u_0 \oplus \cdots u_i \cdots u_j \cdots \oplus u_n}}
\tif \exists i,j\neq 1 \;\; \AbelardM{u_i < u_j } \uberTo{\star, \ttt{A!?-comp}} \EloiseM{u'_i< u'_j}{\alpha},   \\
& \\
& \frac{\AbelardM{ u_0 \oplus \cdots  u'_i \cdots u'_j \cdots  \oplus u_n}}
       {\EloiseM{u_0 \oplus \cdots u_i \cdots u_j \oplus u_n}{(\alpha,k)}}
\tif \exists i,j \;\; \EloiseM{u_i<u_j}{\alpha} \uberTo{\star,\ttt{E-!?}} \AbelardM{u'_i<u'_j}, \textrm{ where } j \neq 1\\
\end{align*}
 
 These rules  define a B\"uchi   game: its starting position is $\AbelardM{u_0 \oplus \ldots \oplus u_n}$,
and the set of accepting states $\mathcal{F}$ is the set of states containing 
 the pair $(\alpha,1)$, where  $\alpha$ is an arbitrary term. 
This condition ensures that  any infinite communication involves the client.

The definition of the $\synch$-coherence between terms as follows.
\begin{definition}
\label{coherence:terms:def}
 Let $C \subseteq \Sigma_0$ be a  finite set of constant symbols. 
 We define the coherence relation $\synch_{C} \subseteq \mterms \times \mterms$ between 
 terms with  respect  to $C$  by: 
 $\bar{\alpha} \synch_C \alpha$ iff there exist two ground substitutions 
   $\bar{\sigma}$ and $\sigma$, and a term $\alpha_0 \in \mterms$ such that  
      $\bar{\sigma} \synch_C \sigma$ and $\bar{\sigma}(\alpha_0)= \bar{\alpha}$ 
      and  $\sigma(\alpha_0)=\alpha$.
\end{definition}

    \begin{align}
      \begin{cases}
         (\set{ x \mapsto \bar{\sigma}_3(\alpha)} \uplus \bar{\sigma}_2)   \synch        (\set{ x \mapsto {\sigma_3(\alpha)}} \uplus \sigma_2), \tand \\
         (\bar{\sigma}_1 \uplus \set{ x \mapsto \bar{\sigma}_3(\alpha)} \uplus \bar{\sigma}_2) (y) 
         =  (\bar{\sigma}_1 \uplus \set{ x \mapsto \bar{\sigma}_3(\alpha)} \uplus \bar{\sigma}_2) (z) 
        \textrm{ iff } \\ 
       \;\;         ({\sigma}_1 \uplus \set{ x \mapsto {\sigma}_3(\alpha)} \uplus {\sigma}_2) (y) 
         =  ({\sigma}_1 \uplus \set{ x \mapsto {\sigma}_3(\alpha)} \uplus {\sigma}_2) (z) 
      \end{cases}
    \end{align}


\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{60pt}
  \begin{center}
\begin{tikzpicture}[shorten >=1pt,bend angle=30, node distance=3cm,on grid,auto, initial text=,
  bend angle=45] 
   \node[state,initial above,accepting] (p_0)   {$p_0$}; 
   \node[state,accepting](p_1) [left =of p_0] {$p_1$};
   \node[state,accepting](p_2) [right =of p_0] {$p_2$};
    \path[->] 
    (p_0) edge  [bend left]  node   {$?x$} (p_1)
    (p_1) edge  [bend left] node  {$!x$}  (p_0)
    (p_0) edge  [bend left]  node  {$!y$} (p_2)
    (p_2) edge  [bend left]  node  {$?y$}  (p_0);
\end{tikzpicture}
  \end{center}
  \vspace{-20pt}
  \caption{A gull}
  \vspace{-10pt}
\end{wrapfigure}

\newpage
\begin{proof}
For the intersection, we refine  the proof 
 that v-automata are closed under intersection \cite{GKS10}. 
    First, we recall that, given two finite automata
$A_i=(\Sigma,Q_i,\delta_i,q_i^0,Q^f_i)$, $i=1,2$, 
the state space of the intersection of $A_1$ and $A_2$  is $Q_1\times Q_2$, 
and $(q'_1,q'_2) \in \delta((q_1,q_2),a)$ iff $q'_1 \in \delta_1(q_1,a)$
 and   $q'_2 \in \delta_2(q_2,a)$. If $A_1$ and $A_2$ are BFVAs then
the letter $a$ may be a variable as well. Hence, on the one hand, 
there are many cases to consider when one intersects two different labeled transitions:   
 when the two labels are both variables, and when one of them is a variable and 
 the other is a constant. In the former case we should consider whether 
the two variables are bound or free. 
On the other hand, bound variables can be refreshed when passing some states, 
giving rise  to  new variables that must be considered. 

Summing up,  given two BFVAs $\mathcal{A}_1=\model{\Sigma_1,X_1,Q_1,Q_0^1,\delta_1,F_1,\kappa_1}$,
and $\mathcal{A}_2=\model{\Sigma_2,X_2,Q_2,Q_0^2,\delta_2,F_2,\kappa_2}$, where  $X_1 \cap X_2 = \emptyset$, 
 we would like to define $\delta$ such that 
for $\alpha \in (\Sigma_1\cup \Sigma_2) \cup \mycal{X}$ we have 
$(q'_1,q'_2) \in \delta((q_1,q_2),\alpha)$ iff there exist
$\alpha_1 \in \Sigma_1 \cup \mycal{X}$ and $\alpha_2 \in \Sigma_2 \cup \mycal{X}$
such that $q'_1 \in \delta_1(q_1,\alpha_1)$  and $q'_2 \in \delta_2(q_2,\alpha_2)$ 
and such that $\alpha_1$ and $\alpha_2$ can match in the sense explained above.

To define $\delta$, we define a relation $H$ for the correspondence 
 between the \emph{occurrences} of variables and constants of $A$ and the 
 \emph{occurrences}  of the variables and constants of $B$.
We define $H=H_{V} \cup H_{AB}$ where 
\begin{align*}
H_{V} &\subseteq ((Q_1 \times X_1 \times Q_1) \times (Q_2 \times X_2 \times Q_2)),   \tand \\
H_{AB} & \subseteq (\Sigma_1 \times (Q_2 \times X_2 \times Q_2)) \cup ((Q_1 \times X_1 \times Q_1) \times \Sigma_2)
\end{align*}

Furthermore,   we should consider the \emph{coherence} of  $H_V \cup H_{AB}$. That is, we allow 
for instance that two fresh occurrences of the  same  variable to match two distinct constants, 
 but we do not allow  that  two  non-fresh  occurrences of the  same  variable to match two distinct constants. 
Formally, out of the BFVA $\mathcal{A}_i$, $i=1,2$, we built the \emph{dependency graph} 
  $G_i$ of  the non fresh occurrences of the variables of $\mathcal{A}_i$.   
 Intuitively, an  occurrence of a  variable $x$ 
 depends on another occurrence of $x$  if there is a path in $\mathcal{A}_i$ from the latter occurrence 
 to the former  
 that does not pass through a third  occurrence of $x$ and $x$ is not 
 refreshed throughout this path. 

Formally, the graph $G_1=(V_1,E_1)$ is defined as follows. The set of its vertices is  $V(G_1)=Q_1 \times X_1 \times Q_1$, 
and there is an edge $(p_0,x,p_1) \uberTo{} (q_0,x,q_1) \in E(G_1)$ iff  there exists a path in $\mathcal{A}_1$ of the form 
 \begin{align*}
 p_0 \uberTo{x} p_1 \uberTo{\alpha_1} p_2 \uberTo{\alpha_2}  \cdots p_{n-1} \uberTo{x} p_n
 \end{align*}

such that $p_{n-1}=q_0$, $p_n=q_1$, and for all $ i \in \set{2,\cdots,n-1}$, $x\neq \alpha_i$ and
  $p_i \notin \kappa(x)$. 
The definition of $G_2$ is similar.
 The relation  $H$ is called coherent iff  the two following conditions hold:

\begin{align*}
\begin{cases}
((p_1,x,p_2),\alpha)) \in H,  \tand  \\
((q_1,x,q_2), \beta)) \in H \tand  \\ 
(p_1,x,p_2) \uberTo{} (q_1,x,q_2) \in E(G_1) 
\end{cases}
 \implies  \alpha \equiv \beta,
\end{align*}

and 

\begin{align*}
\begin{cases}
(\alpha,(p_1,x,p_2)) \in H,  \tand  \\
(\beta,(q_1,x,q_2))) \in H \tand  \\ 
(p_1,x,p_2) \uberTo{} (q_1,x,q_2) \in E(G_2) 
\end{cases}
 \implies  \alpha \equiv \beta
\end{align*}
 
  For a fixed coherent  $H$, we define 
\begin{align*}
  C_{H}=\model{\Sigma_1\cup \Sigma_2, X_1 \times X_2, Q_1\times Q_2, Q_0^1 \times Q_0^2,\delta, F_1 \times F_2,\kappa},
\end{align*}
where  
 \begin{align*}
     (q_1,q_2) \in \kappa((x,y))    \textrm{ iff }   q_1 \in \kappa_1(x) \tand  q_2 \in \kappa_2(y),
 \end{align*}

and  $(q'_1,q'_2) \in \delta((q_1,q_2),\alpha)$ if one of the following cases holds:
\begin{itemize} 
\item $\alpha \in \Sigma_1 \cap \Sigma_2$ and $q'_i \in \delta_1(q_i,\alpha)$ for $i=1,2$, 

\item $\alpha \in \Sigma_2$ and there is a variable $x_1\in X_1$ such that $((q_1,x_1,q'_1),\alpha)\in H_{AB}$, 
   $q'_1 \in \delta_1(q_1,x_1)$ and    $q'_2 \in \delta_2(q_2,\alpha)$.

\item $\alpha \in \Sigma_1$ and there is a variable $x_2\in X_2$ such that $(\alpha,(q_2,x_2,q'_2))\in H_{AB}$, 
   $q'_1 \in \delta_1(q_1,\alpha)$ and    $q'_2 \in \delta_2(q_2,x_2)$. 
\item $\alpha=(x_1,x_2)$, if $((q_1,x_1,q'_1),(q_2,x_2,q'_2))\in H_V$ and $q'_i \in \delta'_i(q_i,x_i)$, $i=1,2$.
\end{itemize}

Finally, we define 
\begin{align*} 
  C=\cup_{H} C_{H} \tst H  \textrm{ is coherent  }  
\end{align*}
\qed 
\end{proof}

\subsection{Canonical form of BFVAs}

\begin{definition}
A BFVA  $A=\model{\Sigma,\mathcal{X},Q,q_0,\delta,F,\kappa}$ is in canonical form iff
every variable is refreshed  at most at one state, i.e. $|\kappa(x)|\le 1$ for all $x\in \mycal{X}$, 
and for each transition $q_1\uberTo{x}q_2$, where $x\in \mycal{X}$ and $x\notin \kappa(q_1)$,
every $(q_0,q_1)$-path  passes through the state  in which the variable $x$ is refreshed.  
\end{definition}
\begin{lemma}
For every BFVA there exists an equivalent BFVA in the canonical form.
\end{lemma}


\begin{proof}
The second  step consists in splitting each state of $\mycal{A}_1\times \mycal{A}_2$ so that in each new state 
we memorize the variables being identical.
Formally, out of $\mycal{A}_1\times \mycal{A}_2$ we construct the BFVA 
$(\mycal{A}_1\times \mycal{A}_2)^{M}=\model{\Sigma^M,\mycal{X}^M,Q^M,q_0^M,\delta^M,F^M,\kappa^M}$
as follows.
Let $\xi$ be the set  of all the \emph{coherent equivalence} relations  over $(\mycal{X}_1\cup \Sigma_1) \times (\mycal{X}_2\cup \Sigma_2)$, i.e. 
\begin{align*}
    \xi=\{E &\tst E \subseteq (\mycal{X}_1\cup \Sigma_1) \times (\mycal{X}_2\cup \Sigma_2), \\
            & \tand E \textrm{ is an equivalence relation},  \\
            & \tand  (a,b) \notin  E, \textrm{ where } a,b\in \Sigma_1\cup\Sigma_2 \tand a\neq b \},
 \end{align*}
 Then
\begin{description} 
\item[$\bullet$] $\Sigma^M=(\Sigma_1 \times \Sigma_2)\cup (\Sigma_1 \times \mycal{X}_2) \cup (\mycal{X}_1 \times \Sigma_2)$.
\item[$\bullet$]  $\mycal{X}^M=\mycal{X}_1 \times \mycal{X}_2$.
\item[$\bullet$] $Q^M=(Q_1\times Q_2) \times \xi$.
\item[$\bullet$] $q_0^M=((q_0^1,q_0^2),\emptyset)$.
\item[$\bullet$] $\delta^M$ is defined by:  
\begin{align*}
 &  ((q'_1,q'_2),E') \in \delta^{M}\big(((q_1,q_2),E),  (\alpha_1,\alpha_2)\big)  \textrm{ iff } \\
 &  (q'_1,q'_2) \in \delta ((q_1,q_2),  (\alpha_1,\alpha_2)) \tand E' = (E \cup \set{(\alpha_1,\alpha_2)})_{|D} ,
\end{align*}
where $D=(\mycal{X}_1 \cup \mycal{X}_2) \setminus (\kappa_1^{-1}(q'_1)\cup \kappa_2^{-1}(q'_2) )$.
\item[$\bullet$] $F^M=(F_1\times F_2) \times \xi$.
\item[$\bullet$] $\kappa^M= \kappa \times \xi$, i.e.  $dom(\kappa^M)=dom(\kappa)$, $codom(\kappa^M)=codom(\kappa) \times \xi$ and \\  
    $\kappa^{M}(\boldsymbol{x})=\set{(\boldsymbol{q},E),  \textrm{ where } \boldsymbol{q} \in \kappa(\boldsymbol{x}) \tand E\in \xi}$.
\end{description}


The third  step consists  in constructing the variables and constants of  $(A_1\times A_2)^{{M}}$. 
Let $\mathbb{V}_{n,m}=(\set{V_1,\ldots,V_n},\set{C_1,\ldots,C_m})$ be  such that  
$V_i \subseteq \mycal{X}_1\cup \mycal{X}_2$ and $C_i \subseteq \mycal{X}_1\cup \mycal{X}_2 \cup \Sigma(\mycal{A}_1) \cup \Sigma(\mycal{A}_2)$
 for all $i$,  and  $|C_i\cap \Sigma|=1$.
For a fixed $\mathbb{V}_{n,m}$, and  out of $(A_1\times A_2)^M$ we     construct 
\begin{align*}
(A_1 \times  A_2)^{\mathbb{V}_{n,m}}=\model{\Sigma^{\mathbb{V}_{n,m}},X^{\mathbb{V}_{n,m}},Q^{\mathbb{V}_{n,m}},q^{\mathbb{V}_{n,m}},\delta^{\mathbb{V}_{n,m}},F^{\mathbb{V}_{n,m}},\kappa^{\mathbb{V}_{n,m}}}
\end{align*}
 as follows:
\begin{description} 
\item[$\bullet$] $\Sigma^{\mathbb{V}_{n,m}}=\Sigma \cup \set{c_1,c_2,\ldots,c_m}$, where $c_i \notin \Sigma$.
\item[$\bullet$] $X^{\mathbb{V}_{n,m}}=\set{z_1,z_2,\ldots,z_n}$, where $ z_i \notin (\mycal{X}_1\cap \mycal{X}_2)$.
\item[$\bullet$] $Q^{\mathbb{V}_{n,m}}=Q^{M}$.
\item[$\bullet$] $q_0^{\mathbb{V}_{n,m}}=q_0^{M}$.
\item[$\bullet$] $\delta^{\mathbb{V}_{n,m}}$ is defined by:
\begin{align*}
((q'_1,q'_2),E')  \in \delta^{\mathbb{V}_{n,m}} (((q_1,q_2),E),a) \textrm{ iff } & ((q'_1,q'_2),E')  \in \delta^{M} (((q_1,q_2),E),(a,a)) \\
&\textrm{ where } a \in \Sigma, \\
%%
((q'_1,q'_2),E')  \in \delta^{\mathbb{V}_{n,m}} (((q_1,q_2),E),c_k) \textrm{ iff } & ((q'_1,q'_2),E')  \in \delta^{M} (((q_1,q_2),E),(\alpha_1,\alpha_2))
\tst  \\
 & (\alpha_1,a) \in E \tor (\alpha_2,a) \in E, \textrm{ for } a \in \Sigma, \tand  \\
   & \quad \quad \set{\alpha_1,\alpha_2,a} \subseteq C_k \tor \\
 & \set{\alpha_1,\alpha_2,a} \subseteq C_k, \textrm{ for some } k\in[1,m]\\ 
%%
((q'_1,q'_2),E')  \in \delta^{\mathbb{V}_{n,m}} (((q_1,q_2),E),z_k) \textrm{ iff } & ((q'_1,q'_2),E')  \in \delta^{M} (((q_1,q_2),E),(w_1,w_2))\\
& \tand  \set{w_1,w_2} \subseteq V_k,  \textrm{ for some }  k\in[1,n],
\end{align*}
and $\delta^{\mathbb{V}_{n,m}}$ is subject to the two following dual conditions $(\Pi_1)$ and $(\Pi_2)$:
\begin{align*}
(\Pi_1)\begin{cases}
  \hspace{1cm} \textrm{ there is  an edge-simple  path } \\
 ((p_1,q_1),E_1)\uberTo{(x_1,y_1)}((p_2,q_2),E_2)\uberTo{-} \ldots  \uberTo{(x_1,y_n)}((p_n,q_n),E_n) \\
%\end{align*}
\textrm { in }  (A_1\times  A_2)^{M} \textrm{ where }  p_i \notin \kappa^1(x_1), \forall i\in\set{2,\ldots,n}, \\
\\
 \hspace{1cm} \textrm{ iff either there is an edge-simple  path } \\
\\
%\begin{align*}
 ((p_1,q_1),E_1)\uberTo{z_k}((p_2,q_2),E_2)\uberTo{\_} \ldots \uberTo{z_k}((p_n,q_n),E_n) \\
%\end{align*}
\textrm{in } (A_1\times A_2)^{\mathbb{V}_{n,m}} \textrm{ where }\set{x_1,y_1,y_n} \subseteq V_k,  \\
\hspace{1cm} \textrm{ or  there is an edge-simple  path } \\
%\begin{align*}
 ((p_1,q_1),E_1)\uberTo{c_k}((p_2,q_2),E_2)\uberTo{\_} \ldots \uberTo{c_k}((p_n,q_n),E_n)\\
\textrm{in } (A_1\times A_2)^{\mathbb{V}_{n,m}} \textrm{ where } \set{x_1,y_1,y_n} \subseteq C_k. 
\end{cases}
\end{align*}


\begin{align*}
(\Pi_2)\begin{cases}
  \hspace{1cm} \textrm{ there is  an edge-simple  path } \\
 ((p_1,q_1),E_1)\uberTo{(x_1,y_1)}((p_2,q_2),E_2)\uberTo{-} \ldots  \uberTo{(x_n,y_1)}((p_n,q_n),E_n) \\
%\end{align*}
\textrm { in }  (A_1\times  A_2)^{M} \textrm{ where }  q_i \notin \kappa^2(y_1), \forall i\in\set{2,\ldots,n}, \\
\\
 \hspace{1cm} \textrm{ iff either there is an edge-simple  path } \\
\\
%\begin{align*}
 ((p_1,q_1),E_1)\uberTo{z_k}((p_2,q_2),E_2)\uberTo{\_} \ldots \uberTo{z_k}((p_n,q_n),E_n) \\
%\end{align*}
\textrm{in } (A_1\times A_2)^{\mathbb{V}_{n,m}} \textrm{ where }\set{x_1,y_1,x_n} \subseteq V_k,  \\
\hspace{1cm} \textrm{ or  there is an edge-simple  path } \\
%\begin{align*}
 ((p_1,q_1),E_1)\uberTo{c_k}((p_2,q_2),E_2)\uberTo{\_} \ldots \uberTo{c_k}((p_n,q_n),E_n)\\
\textrm{in } (A_1\times A_2)^{\mathbb{V}_{n,m}} \textrm{ where } \set{x_1,y_1,x_n} \subseteq C_k. 
\end{cases}
\end{align*}



\item[$\bullet$] $F^{\mathbb{V}_{n,m}}=F^M$.
\item[$\bullet$] $\kappa^{\mathbb{V}_{n,m}}$ is defined by $\kappa^{\mathbb{V}_{n,m}}(z_i)=\set{(\boldsymbol{q},E) \tst (\boldsymbol{q},E) \in \kappa^{M}((x_1,x_2)) \tand \set{x_1,x_2}=V_i}$.
\end{description} 
Then we let $(A_1 \times A_2)^{\mathbb{V}_{n,m}^c}$ be the BVFA obtained  from  $(A_1 \times A_2)^{\mathbb{V}_{n,m}}$
by replacing each constant $c_k$ by the (unique) constant $a \in C_k$.   
Finally, we define: 
\begin{align*}
A_1 \cap A_2 = \bigcup_{\mathbb{V}_{n,m}}(A_1 \times A_2)^{\mathbb{V}_{n,m}^c}
\end{align*}
Now we must show that our construction is correct and complete, i.e. 
\begin{align*}
L(\mycal{A}_1)\cap L(\mycal{A}_2)=L(\bigcup_{\mathbb{V}_{n,m}}(A_1 \times A_2)^{\mathbb{V}_{n,m}^c}).
\end{align*}
 To this goal
we introduce a variant  of BVFA  \emph{with constraints}. That is, the transitions are pairs $(\alpha,S)$ where 
$\alpha \in \mycal{X}\cup \Sigma$ and $S$ is a finite set of equations, i.e. $S=\set{\alpha_1=\beta_1,\ldots,\alpha_n=\beta_n}$ 
where $\alpha_i,\beta_i \in \mycal{X}\cup \Sigma$.  The notion of configuration and run for BFVAs with constraints
is the same as those of BFVAs apart that a transition labeled with $(\alpha,S)$  is possible iff  $S$ has a solution\footnote{To formalize.}.
The notion of language recognized  by a BFVA with constraints can be defined similarly.
Notice that $\mycal{A}_1\times \mycal{A}_2$ defined above can be viewed as a BFVA with constraints by turning each transition labeled
with a pair $(\alpha,\beta)$ into a transition labeled with $(\alpha, \set{\alpha=\beta})$.  
Similarly, if we view $(\mycal{A}_1\times \mycal{A}_2)^{M}$  as a BFVA with constraints, 
then we get the  following immediate  Fact:
\begin{fact}
Let $\mycal{A}_1$ and $\mycal{A}_2$ be BFVAs. Then,
\begin{align*}
L(\mycal{A}_1) \cap L(\mycal{A}_2) = L(\mycal{A}_1\times \mycal{A}_2)=L((\mycal{A}_1\times \mycal{A}_2)^{M}).
\end{align*}
\end{fact}
Hence, it remains to show that 
\begin{align*}
L((\mycal{A}_1\times \mycal{A}_2)^{M})=L(\bigcup_{\mathbb{V}_{n,m}}(A_1 \times A_2)^{\mathbb{V}_{n,m}^c}).
\end{align*} 
 
For the inclusion "$\supseteq$",  we show that, for a fixed $\mathbb{V}_{n,m}$, 
 every accepting run\footnote{For readability, we put the letters of the VBA on the run.} $r_l^c=(\bs{q}_0,M_0^c)\uberTo{\alpha_1}\ldots\uberTo{\alpha_{m}}(\bs{q}_l,M_l^c)$ of $(A_1 \times A_2)^{\mathbb{V}_{n,m}^{c}}$ over a word $\boldsymbol{w}=w_1\ldots w_l\in \Sigma^{\star}$ 
 can be transformed into an accepting run  $r_l=(\bs{q}_0,M_0)\uberTo{\bs{\bs{\beta}}_1}\ldots \uberTo{\bs{\bs{\beta}}_l}(\bs{q}_l,M_l)$ of $(\mycal{A}_1\times \mycal{A}_2)^{M}$ over $\boldsymbol{w}$.
The proof is by induction on $l$. The base case $l=0$ follows trivially from the  definition of $\bs{q}_0$.
For the induction step, let $\bs{q}_l=((q_l^1,q_l^2),E_l)$ and a transition 
$(\bs{q}_l,E_l)\uberTo{\alpha_{l+1}}(\bs{q}_{l+1},E_{l+1})$ in $(A_1 \times A_2)^{\mathbb{V}_{n,m}^c}$ and a transition 
$(\bs{q}_l,E_l)\uberTo{\bs{\beta}_{l+1}}(\bs{q}_{l+1},E_{l+1})$ 
in $(\mycal{A}_1\times \mycal{A}_2)^{M}$. 
\begin{itemize}
\item If $\bs{\alpha}_{l+1}$ is a constant, say $a \in \Sigma$,  then we distinguish  many cases depending on $\bs{\beta}_{l+1}$:
 \begin{itemize}
  \item  If $\bs{\beta}_{l+1}=(a,a)$ or $\bs{\beta}_{l+1}=(x,a)$ or  $\bs{\beta}_{l+1}=(a,y)$,  then  we are done.
  \item  If $\bs{\beta}_{l+1}=(x,y)$, then in this case $\alpha_{l+1}$ must be a constant coming from  $c_k$, i.e.
   $\set{x,y} \subseteq C_k$ for some $k$. 
 \end{itemize}
\item Otherwise, if  $\alpha_{l+1}$ is a variable $z_k \in \mycal{X}^{\mathbb{V}_{n,m}}$. 
Then in this case 
$\bs{\beta}_{l+1}=(x_{l+1},y_{l+1})$    for some variables  
$x_{l+1},y_{l+1}$ and  so that $\set{x_{l+1},y_{l+1}} \subseteq V_k$, for some $k$. Then in this case 
 we must show that $z_k \in dom(M^c_{l})$  iff $x_{l+1},y_{l+1} \in dom(M_{l})$ and if $z_k \in dom(M^c_{l})$ then 
$M_l^c(z_k)=M_l(x_{l+1})=M_l(y_{l+1})$.
If $z_k \in dom(M^c_l)$ then there must exist $m'<m$ such  that $z_k \in dom(M^c_{l'})$ and $z_k$ was not refreshed between $\bs{q}_{l'}$ and 
$\bs{q}_{l}$, i.e.
 for all $j \in ]m',m]$, $\bs{q}_j \notin \kappa(z_k)$. Hence there must be $x_{l'},y_{l'} \in dom(M_{l'})$ such that 
  $x_{l'},y_{l'} \in V_k$ and $M_{l'}(x_{l'})=M_{l'}(y_{l'})=M^c_{l'}(z_k)$. From the path condition $(\Pi)$ above, it follows
  that for all $j \in ]m',m]$ there exists $x_j \in V_k$ such that $M_{j}(x_j)=M_{l'}(x_{l'})=M_{l'}(y_{l'})=M^c_{l'}(z_k)=M^c_{l}(z_k)=M_{l}(x_{l+1})$.
\end{itemize}

For the inclusion "$\subseteq$",  we show that, 
 every accepting run  
\begin{align*}
r_l=(\bs{q}_0,M_0)\uberTo{\bs{\bs{\beta}}_1}\ldots \uberTo{\bs{\bs{\beta}}_l}(\bs{q}_l,M_l) \textrm { of }  
(\mycal{A}_1\times \mycal{A}_2)^{M}
\end{align*}
    over a word $\boldsymbol{w}=w_1\ldots w_l\in \Sigma^{\star}$ 
yields a unique $\mathbb{V}_{n,m}^{l}$
 and can be transformed into an accepting run 
\begin{align*}
r_l^c=(\bs{q}_0,M_0^c)\uberTo{\alpha_1}\ldots\uberTo{\alpha_{l}}(\bs{q}_l,M_l^c) \textrm{ of } 
(A_1 \times A_2)^{\mathbb{V}_{n,m}^{c}}
\end{align*}
 over $\boldsymbol{w}$. We describe how  to construct $\mathbb{V}_{n,m}^{l}$ from the run $r_l$. More, precisely 
we construct $\mathbb{V}_{n,m}^l$ from the path $\pi_l=\bs{q}_0 \uberTo{\bs{\beta}_1}\ldots \uberTo{\bs{\beta}_l}\bs{q}_l$.
If $l=0$ then we take $\mathbb{V}_{n,m}^0=(\emptyset,\emptyset)$. Assume that 
$\mathbb{V}_{n,m}^l=(\set{V_1,\ldots,V_n},\set{C_1,\ldots,C_m})$ is constructed from $\pi_l$, 
then the construction of $\mathbb{V}_{n,m}^{l+1}$  depends on    $\bs{\beta}_{l+1}$: 
\begin{itemize}
\item If $\bs{\beta}_{l+1}=(a,a)$, where $a \in \Sigma$, then $\mathbb{V}^{l+1}_{n,m}:=\mathbb{V}^{l}_{n,m}$. 
\item If $\bs{\beta}_{l+1}=(x,b)$, where $x \in \mycal{X}_1$ and $b  \in \Sigma$  then we distinguish two cases. If there
    exists $i\in[0,l]$ such that  $x \in \bs{\beta}_{i}$ and $x$ is not refreshed in the states $q_{i},q_{i+1},\ldots, q_l$, then
    $\alpha_i=a$ and  $\bs{\beta}_i\cup \set{x,a} \subseteq C_k$, for some $k\in[1,m]$. In this case we let $\mathbb{V}^{l+1}_{n,m}:=\mathbb{V}^{l}_{n,m}$.
  Otherwise, we let $\mathbb{V}_{n,m}^{l+1}=(\set{V_1,\ldots,V_n},\set{C_1,\ldots,C_m,\set{a,x}})$.
\item If $\bs{\beta}_{l+1}=(a,y)$,  where $a  \in \Sigma$ and $x \in \mycal{X}_1$, then this case is similar to the previous one.
\item If $\bs{\beta}_{l+1}=(x,y)$, where $x \in \mycal{X}_1$ and $y \in \mycal{X}_2$. We distinguish two cases. 
If  there exists $i\in[0,l]$ such that  $x \in \bs{\beta}_{i}$ and $x$ is not refreshed in the states $q_{i},q_{i+1},\ldots, q_l$, or 
  $y \in \bs{\beta}_{i}$ and $y$ is not refreshed in the states $q_{i},q_{i+1},\ldots, q_l$ then $\alpha_i=z_k$ for some $k=[1,n]$,
  thus $\set{x,y}\subseteq V_k$. In this case we let $\mathbb{V}^{l+1}_{n,m}:=\mathbb{V}^{l}_{n,m}$. 
  Otherwise, we let $\mathbb{V}_{n,m}^{l+1}=(\set{V_1,\ldots,V_n,\set{x,y}},\set{C_1,\ldots,C_m})$.
\end{itemize}
%% \begin{align*}
%%  L((\mycal{A}_1\times \mycal{A}_2)^{M^c}) \subseteq L((A_1 \cap A_2)^{\mathbb{V}_{n,m}})
%% \end{align*} 
\qed 
\end{proof}

\newpage

\paragraph{Second step.} The second  step consists in  transforming the $2$-letters of 
$\mycal{\what{A}}$ into $1$-letters, by introducing new variable and constant symbols. 
Let $\mathbb{V}_{n,m}=(\set{V_1,\ldots,V_n},\set{C_1,\ldots,C_m})$ be  such that for all $1\leq i \leq n$, 
$V_i \subseteq \mycal{X}$ and for all $1\leq j \leq m$, $C_j \subseteq \mycal{X}  \cup \Sigma(\mycal{A})$ 
and  $|C_j\cap \Sigma|=1$.
For a fixed $\mathbb{V}_{n,m}$, and  out of $\mycal{\what{A}}$ we     construct the BFVA $\what{\mycal{A}}^{\mathbb{V}_{n,m}}$: 
\begin{align*}
 \what{\mycal{A}}^{\mathbb{V}_{n,m}}=\model{\what{\Sigma}^{\mathbb{V}_{n,m}},\what{\mycal{X}}^{\mathbb{V}_{n,m}},
   \what{Q}^{\mathbb{V}_{n,m}},\what{q}^{\mathbb{V}_{n,m}},\what{\delta}^{\mathbb{V}_{n,m}},\what{F}^{\mathbb{V}_{n,m}},\what{\kappa}^{\mathbb{V}_{n,m}}}
\end{align*}
 as follows:
\begin{description} 
\item[$\bullet$] $\what{\Sigma}^{\mathbb{V}_{n,m}}=\Sigma \cup \set{c_1,c_2,\ldots,c_m}$, where $c_i \notin \what{\Sigma}$.
\item[$\bullet$] $\what{\mycal{X}}^{\mathbb{V}_{n,m}}=\set{z_1,z_2,\ldots,z_n}$, where $ z_i \notin \mycal{X}$.
\item[$\bullet$] $\what{Q}^{\mathbb{V}_{n,m}}=\what{Q}$.
\item[$\bullet$] $\what{q}_0^{\mathbb{V}_{n,m}}=\what{q}_0$.
\item[$\bullet$] $\what{\delta}^{\mathbb{V}_{n,m}}$ is defined by:
\begin{align*}
(q',E')  \in \what{\delta}^{\mathbb{V}_{n,m}} ((q,E),a) \textrm{ iff } & (q',E')  \in \what{\delta} ((q,E),(a,a)) \\
&\textrm{ where } a \in \Sigma, \\
%%
(q',E')  \in \what{\delta}^{\mathbb{V}_{n,m}} ((q,E),c_k) \textrm{ iff } & (q',E')  \in \what{\delta} ((q,E),(\alpha_1,\alpha_2))
\tst  \\
 & (\alpha_1,a) \in E \tor (\alpha_2,a) \in E, \textrm{ for } a \in \Sigma, \tand  \\
   & \quad \quad \set{\alpha_1,\alpha_2,a} \subseteq C_k \tor \\ 
 & \set{\alpha_1,\alpha_2,a} \subseteq C_k, \textrm{ for some } k\in[1,m]\\ 
%%
(q',E')  \in \what{\delta}^{\mathbb{V}_{n,m}} ((q,E),z_k) \textrm{ iff } & (q',E')  \in \what{\delta} ((q,E),(w_1,w_2))\\
& \tand  \set{w_1,w_2} \subseteq V_k,  \textrm{ for some }  k\in[1,n],
\end{align*}
and $\what{\delta}^{\mathbb{V}_{n,m}}$ is subject to the following  condition $(\Pi)$: 
\begin{align*}
(\Pi)\begin{cases}
  \hspace{1cm} \textrm{ there is  an edge-simple  path } \\
 (q_1,E_1)\uberTo{\set{x_1,y_1}}(q_2,E_2)\uberTo{-} \ldots  \uberTo{\set{x_1,y_n}}(q_n,E_n) \\
%\end{align*}
\textrm { in }  \what{\mycal{A}}  \textrm{ where }  q_i \notin \kappa(x_1), \forall i\in\set{2,\ldots,n}, \\
\\
 \hspace{1cm} \textrm{ iff either there is an edge-simple  path } \\
\\
%\begin{align*}
 (q_1,E_1)\uberTo{z_k}(q_2,E_2)\uberTo{\_} \ldots \uberTo{z_k}(q_n,E_n) \\
%\end{align*}
\textrm{in } \what{\mycal{A}}^{\mathbb{V}_{n,m}} \textrm{ where }\set{x_1,y_1,y_n} \subseteq V_k,  \\
\hspace{1cm} \textrm{ or  there is an edge-simple  path } \\
%\begin{align*}
 (q_1,E_1)\uberTo{c_k}(q_2,E_2)\uberTo{\_} \ldots \uberTo{c_k}(q_n,E_n)\\
\textrm{in } \what{\mycal{A}}^{\mathbb{V}_{n,m}} \textrm{ where } \set{x_1,y_1,y_n} \subseteq C_k. 
\end{cases}
\end{align*}
\item[$\bullet$] $F^{\mathbb{V}_{n,m}}=F^M$.
\item[$\bullet$] $\what{\kappa}^{\mathbb{V}_{n,m}}$ is defined by $\what{\kappa}^{\mathbb{V}_{n,m}}(z_i)=\set{(q,E) \tst 
 (q,E) \in \what{\kappa}(x_1) \cap \what{\kappa}(x_2) \tand \set{x_1,x_2}=V_i}$.
\end{description} 
Then we let $\what{\mycal{A}}^{\mathbb{V}_{n,m}^c}$ be the BVFA obtained  from  $\what{\mycal{A}}^{\mathbb{V}_{n,m}}$
by replacing each constant $c_k$ by the (unique) constant $a \in C_k$.   


\begin{claim}
The $2$-BFVA $\what{\mycal{A}}$ and the BFVA $\bigcup_{\mathbb{V}_{n,m}}\what{\mycal{A}}^{\mathbb{V}_{n,m}^c}$
are equivalent.\marginpar{c est pas la meme notion d'quivalence: cf renomage constantes. Si: on remplace les 
 les cons. intermediaires $c_k$ par les $a \in C_k$.}
\end{claim}
\begin{proof}
We shall show that 
\begin{align*}
L(\what{\mycal{A}})=L(\bigcup_{\mathbb{V}_{n,m}}\what{\mycal{A}}^{\mathbb{V}_{n,m}^c}).
\end{align*}
For the inclusion "$\supseteq$",  we show that, for a fixed $\mathbb{V}_{n,m}$, 
 every accepting run\footnote{For readability, we put the letters of the BVFA on the run.} $r_l^c=(\bs{q}_0,M_0^c)\uberTo{\alpha_1}\ldots\uberTo{\alpha_{m}}(\bs{q}_l,M_l^c)$ of $\what{\mycal{A}}^{\mathbb{V}_{n,m}^{c}}$ over a word $\boldsymbol{w}=w_1\ldots w_l\in \Sigma^{\star}$ 
 can be transformed into an accepting run  $r_l=(\bs{q}_0,M_0)\uberTo{\bs{\bs{\beta}}_1}\ldots \uberTo{\bs{\bs{\beta}}_l}(\bs{q}_l,M_l)$ of 
$\what{\mycal{A}}$ over $\boldsymbol{w}$.
The proof is by induction on $l$. The base case $l=0$ follows trivially from the  definition of $\bs{q}_0$.
For the induction step, let $\bs{q}_l=(q_l,E_l)$ and a transition 
$(q_l,E_l)\uberTo{\alpha_{l+1}}(q_{l+1},E_{l+1})$ in $\what{\mycal{A}}^{\mathbb{V}_{n,m}^c}$ and a transition 
$(q_l,E_l)\uberTo{\beta_{l+1}}(q_{l+1},E_{l+1})$ \marginpar{d'ou vient cette transition avec beta? comment sait on qu'elle existe? unique? }
in $\what{\mycal{A}}$. 
\begin{itemize}
\item If $\bs{\alpha}_{l+1}$ is a constant, say $a \in \Sigma$,  then we distinguish  many cases depending on $\bs{\beta}_{l+1}$:
 \begin{itemize}
  \item  If $\bs{\beta}_{l+1}=(a,a)$ or $\bs{\beta}_{l+1}=(x,a)$ or  $\bs{\beta}_{l+1}=(a,y)$,  then  we are done.
  \item  If $\bs{\beta}_{l+1}=(x,y)$, then in this case $\alpha_{l+1}$ must be a constant coming from  $c_k$, i.e.
   $\set{x,y} \subseteq C_k$ for some $k$. 
 \end{itemize}
\item Otherwise, if  $\alpha_{l+1}$ is a variable $z_k \in \what{\mycal{X}}^{\mathbb{V}_{n,m}}$. 
Then in this case 
$\bs{\beta}_{l+1}=(x_{l+1},y_{l+1})$    for some variables  
$x_{l+1},y_{l+1}$ and  so that $\set{x_{l+1},y_{l+1}} \subseteq V_k$, for some $k$. Then in this case 
 we must show that $z_k \in dom(M^c_{l})$  iff $x_{l+1},y_{l+1} \in dom(M_{l})$ and if $z_k \in dom(M^c_{l})$ then 
$M_l^c(z_k)=M_l(x_{l+1})=M_l(y_{l+1})$.
If $z_k \in dom(M^c_l)$ then there must exist $m'<m$ such  that $z_k \in dom(M^c_{l'})$ and $z_k$ was not refreshed between $\bs{q}_{l'}$ and 
$\bs{q}_{l}$, i.e.
 for all $j \in ]m',m]$, $\bs{q}_j \notin \kappa(z_k)$. Hence there must be $x_{l'},y_{l'} \in dom(M_{l'})$ such that 
  $x_{l'},y_{l'} \in V_k$ and $M_{l'}(x_{l'})=M_{l'}(y_{l'})=M^c_{l'}(z_k)$. From the path condition $(\Pi)$ above, it follows
  that for all $j \in ]m',m]$ there exists $x_j \in V_k$ such that $M_{j}(x_j)=M_{l'}(x_{l'})=M_{l'}(y_{l'})=M^c_{l'}(z_k)=M^c_{l}(z_k)=M_{l}(x_{l+1})$.
\end{itemize}

\noindent For the inclusion "$\subseteq$",  we show that, 
 every accepting run  
\begin{align*}
r_l=(\bs{q}_0,M_0)\uberTo{\bs{\bs{\beta}}_1}\ldots \uberTo{\bs{\bs{\beta}}_l}(\bs{q}_l,M_l) \textrm { of }  
 \what{\mycal{A}}
\end{align*}
    over a word $\boldsymbol{w}=w_1\ldots w_l\in \Sigma^{\star}$ 
yields a unique $\mathbb{V}_{n,m}^{l}$
 and can be transformed into an accepting run 
\begin{align*}
r_l^c=(\bs{q}_0,M_0^c)\uberTo{\alpha_1}\ldots\uberTo{\alpha_{l}}(\bs{q}_l,M_l^c) \textrm{ of } 
\what{\mycal{A}}^{\mathbb{V}_{n,m}^{c}}
\end{align*}
 over $\boldsymbol{w}$. We describe how  to construct $\mathbb{V}_{n,m}^{l}$ from the run $r_l$. More, precisely 
we construct $\mathbb{V}_{n,m}^l$ from the path $\pi_l=\bs{q}_0 \uberTo{\bs{\beta}_1}\ldots \uberTo{\bs{\beta}_l}\bs{q}_l$.
If $l=0$ then we take $\mathbb{V}_{n,m}^0=(\emptyset,\emptyset)$. Assume that 
$\mathbb{V}_{n,m}^l=(\set{V_1,\ldots,V_n},\set{C_1,\ldots,C_m})$ is constructed from $\pi_l$, 
then the construction of $\mathbb{V}_{n,m}^{l+1}$  depends on    $\bs{\beta}_{l+1}$: 
\begin{itemize}
\item If $\bs{\beta}_{l+1}=(a,a)$, where $a \in \Sigma$, then $\mathbb{V}^{l+1}_{n,m}:=\mathbb{V}^{l}_{n,m}$. 
\item If $\bs{\beta}_{l+1}=(x,b)$, where $x \in \mycal{X}$ and $b  \in \Sigma$  then we distinguish two cases. If there
    exists $i\in[0,l]$ such that  $x \in \bs{\beta}_{i}$ and $x$ is not refreshed in the states $q_{i},q_{i+1},\ldots, q_l$, then
    $\alpha_i=a$ and  $\bs{\beta}_i\cup \set{x,a} \subseteq C_k$, for some $k\in[1,m]$. In this case we let $\mathbb{V}^{l+1}_{n,m}:=\mathbb{V}^{l}_{n,m}$.
  Otherwise, we let $\mathbb{V}_{n,m}^{l+1}=(\set{V_1,\ldots,V_n},\set{C_1,\ldots,C_m,\set{a,x}})$.
\item If $\bs{\beta}_{l+1}=(a,y)$,  where $a  \in \Sigma$ and $x \in \mycal{X}_1$, then this case is similar to the previous one.
\item If $\bs{\beta}_{l+1}=(x,y)$, where $x \in \mycal{X}_1$ and $y \in \mycal{X}_2$. We distinguish two cases. 
If  there exists $i\in[0,l]$ such that  $x \in \bs{\beta}_{i}$ and $x$ is not refreshed in the states $q_{i},q_{i+1},\ldots, q_l$, or 
  $y \in \bs{\beta}_{i}$ and $y$ is not refreshed in the states $q_{i},q_{i+1},\ldots, q_l$ then $\alpha_i=z_k$ for some $k=[1,n]$,
  thus $\set{x,y}\subseteq V_k$. In this case we let $\mathbb{V}^{l+1}_{n,m}:=\mathbb{V}^{l}_{n,m}$. 
  Otherwise, we let $\mathbb{V}_{n,m}^{l+1}=(\set{V_1,\ldots,V_n,\set{x,y}},\set{C_1,\ldots,C_m})$.
\end{itemize}
This ends the proof of the Claim. \qed
\end{proof}
This ends the proof of Lemma \ref{2BFVA:BFVA:lem}.\qed
\end{proof}

\newpage
\begin{proof}
\begin{proof}
For one direction we note that any  BFVA $\mycal{B}$ can be transformed into an equivalent 
  $2$-BFVA by replacing each transition of $\mycal{B}$ labeled with  $\alpha$ 
by  a transition labeled with the pair $(z,\alpha)$, where $z$ is a new variable that is refreshed in each state. 
For the other direction, let $\mycal{A}=\model{\Sigma,\mathcal{X},Q,Q_0,\delta,F,\kappa}$  
be a $2$-BFVA. Out of $\mycal{A}$,  we shall construct a BFVA  $\mycal{B}$ such that  $L(\mycal{A})= L(\mycal{B})$. 
The proof relies on three transformations starting from  $\mycal{A}$, each of them  preserving the language recognized  by $\mycal{A}$. 
%These transformations are grounded in two  steps. 

\paragraph{First step.} The first step consists in splitting each state of $\mycal{A}$ so that  each new state 
 memorizes the variables that are constrained to be equal.
Formally, out of $\mycal{A}$ we construct the $2$-BFVA $\what{\mycal{A}}$: 
\begin{align*}
\what{\mycal{A}}=\model{\what{\Sigma},\what{\mycal{X}},\what{Q},\what{q}_0,\what{\delta},\what{F},\what{\kappa}}
\end{align*}
as follows. We say that an  equivalence relation $E$  on $\mycal{X}\cup \Sigma $ is \emph{coherent} iff the following holds: 
 for all $a,b \in \Sigma$, if $a \ne b$ then $(a,b) \not \in E$. 
Let $\xi$ be the set  of all  \emph{coherent equivalence} relations  over $\mycal{X} \cup  \Sigma$.


% Let $\xi$ be the set  of all the \emph{coherent equivalence} relations  over $(\mycal{X} \cup  \Sigma) \times (\mycal{X} \cup \Sigma)$, i.e. 
% \begin{align*}
%     \xi=\{E &\tst E \subseteq (\mycal{X}\cup \Sigma) \times (\mycal{X}\cup \Sigma), \\
%             & \tand E \textrm{ is an equivalence relation},  \\
%             & \tand  (a,b) \notin  E, \textrm{ where } a,b\in \Sigma  \tand a\neq b \},
%  \end{align*}
 Then
\begin{description} 
\item[$\bullet$] $\what{\Sigma}=\Sigma$.
\item[$\bullet$]  $\what{\mycal{X}}=\mycal{X}$.
\item[$\bullet$] $\what{Q}=Q \times \xi$.
\item[$\bullet$] $\what{q}_0=\set{(q_0,E) \;|\; E \in \xi}$.
\item[$\bullet$] $\what{\delta}$ is defined by:  
\begin{align*}
   (q',E') \in \what{\delta} \big((q,E),  (\alpha_1,\alpha_2)\big) \quad \textrm{ iff } \quad
     & q' \in \delta (q,  (\alpha_1,\alpha_2)),  \\
     &E' = \big( ((E \cup \set{(\alpha_1,\alpha_2)})^{\star})_{|D'}\big)^{\star}, \tand  \\
     &E = \big( ((E' \cup \set{(\alpha_1,\alpha_2)})^{\star})_{|D}\big)^{\star} ,
\end{align*}
where $D=\mycal{X} \setminus \kappa^{-1}(q)$ and 
 $D'=\mycal{X} \setminus \kappa^{-1}(q')$ and $E^{\star}$ denotes the 
 reflexive, symmetric and transitive closure of $E$. 


\item[$\bullet$] $\what{F}=F \times \xi$.
\item[$\bullet$] $\what{\kappa}$ is defined by 
%= \kappa \times \xi$, i.e.  $dom(\what{\kappa})=dom(\kappa)$, 
%  $codom(\what{\kappa})=codom(\kappa) \times \xi$ and \\  
    $\what{\kappa}(x)=\set{(q,E),  \textrm{ for all } q \in \kappa(x) \tand E\in \xi}$.
\end{description}

\begin{claim}
We have that $L(\mycal{A})=L(\mycal{\what{A}})$.
\end{claim}
\begin{proof}
For the inclusion "$\supseteq$",  we show that
 every accepting run\footnote{For readability, we put the labels of the BVFA on the run.} 
$\what{r_l}=(\what{q}_0,\what{M_0})\uberTo{\alpha_1,\alpha'_1}\ldots\uberTo{\alpha_{m},\alpha'_{m}}(\what{q}_l,\what{M_l})$ of 
$\what{\mycal{A}}$ over a word $\boldsymbol{w}=w_1\ldots w_l\in \Sigma^{\star}$ 
 can be transformed into an accepting run  $r_l=({q}_0,M_0)\uberTo{\alpha_1,\alpha'_1}\ldots \uberTo{\alpha_m,\alpha'_m}({q}_l,M_l)$ of 
$\mycal{A}$ over $\boldsymbol{w}$ such that $M_i=\what{M}_i$ for all $i=0,\ldots,l$.
The proof is by induction on $l$. The base case $l=0$ follows trivially from the  definition of $\what{q}_0$.
For the induction step, let $\what{q}_l=(q_l,E_l)$ and let 
$(q_l,E_l)\uberTo{\alpha_{l+1},\alpha'_{l+1}}(q_{l+1},E_{l+1})$ be a transition  in $\what{\mycal{A}}$. 
On the one hand, by definition, 
  there exists a  transition $q_l \uberTo{\alpha_{l+1},\alpha'_{l+1}}q_{l+1}$
in $\mycal{A}$. On the other hand, from the induction hypothesis it follows that $M_l=\what{M}_l$.
Thus, $M_{l+1}=\what{M}_{l+1}$.

For the inclusion "$\subseteq$",  we show that
 every accepting run  $r_l=({q}_0,M_0)\uberTo{\alpha_1,\alpha'_1}\ldots \uberTo{\alpha_m,\alpha'_m}({q}_l,M_l)$ of 
$\mycal{A}$
over a word $\boldsymbol{w}=w_1\ldots w_l\in \Sigma^{\star}$ 
 can be transformed into an accepting run 
$\what{r_l}=(\what{q}_0,\what{M_0})\uberTo{\alpha_1,\alpha'_1}\ldots\uberTo{\alpha_{m},\alpha'_{m}}(\what{q}_l,\what{M_l})$ of 
$\what{\mycal{A}}$   over $\boldsymbol{w}$ 
such that for all $i=0,\ldots,l$, $M_i=\what{M}_i$ and $\what{q}_i=(q_i,E_i)$ where $E_i \in \xi$. 
The proof is by induction on $l$. The base case $l=0$ follows trivially from the  definition of $\what{q}_0$.
For the induction step, 
let $q_l \uberTo{\alpha_{l+1},\alpha'_{l+1}} q_{l+1}$ be a transition  in $\mycal{A}$. 
We  show next that there is a unique transition 
 $(q_l,E_l)\uberTo{\alpha_{l+1},\alpha'_{l+1}}(q_{l+1},E_{l+1})$   in $\what{\mycal{A}}$  so that
$M_{l+1}=\what{M}_{l+1}$.
This ends the proof of the Claim. \qed
\end{proof}

\paragraph{Second step.} The second  step consists in  transforming some of the $2$-labels\footnote{Notice that this transformation 
 yields a BFVA in which some transitions are labeled with a 
 $1$-label and the other transitions are labeled with  a $2$-labels. More generally, 
 a BFVA in which the transitions are labeled with at most $n$-labels is still called an $n$-BFVA since 
 each  transition labeled with $n'$-label where $n' <n$ can be (equivalently) transformed into a transition
  labeled with $n$-labels.} of 
$\mycal{\what{A}}$ into ($1$-labels) constant letters. 
Out of $\mycal{\what{A}}$ we   define  the BFVA $\what{\mycal{A}}^c$: 
\begin{align*}
 \what{\mycal{A}}^c=\model{\what{\Sigma}^c,\what{\mycal{X}}^c,
   \what{Q}^c,\what{q}^c,\what{\delta}^c,\what{F}^c,\what{\kappa}^c}
\end{align*}
as $\mycal{\what{A}}$ apart that 
the transition function $\what{\delta}^c$ is defined by:
\begin{align*}
(q',E')  \in \what{\delta}^c ((q,E),a) \textrm{ iff } & (q',E')  \in \what{\delta} ((q,E),(a,a)), \textrm{ where } a \in \Sigma, \tor \\
%%
  &  (q',E')  \in \what{\delta} ((q,E),(\alpha_1,\alpha_2))
\tst  \\
 & (\alpha_1,a) \in E \tor (\alpha_2,a) \in E, \textrm{ for } a \in \Sigma, \tand \alpha_1,\alpha_2 \in \mycal{X}\cup \Sigma.
\end{align*}
\begin{claim}
The $2$-BVFAs $\what{\mycal{A}}$ and $\what{\mycal{A}}^c$ are equivalent \
(i.e. recognize the same language).
\end{claim}

\paragraph{Third step.} The third  step consists in  transforming the remaining $2$-labels of 
$\mycal{\what{A}}^c$ into   variables by introducing new variable symbols. 
Let $\mathbb{V}_m=\set{V_1,\ldots,V_m}$ where $V_i \subseteq \mycal{X}$ and $m$ is not greater 
than the number of transitions of $\mycal{\what{A}}^c$. 
For a fixed $\mathbb{V}_m$  and out of $\mycal{\what{A}}^c$ we     construct the BFVA $\what{\mycal{A}}^c_{\mathbb{V}_m}$ as follows: 
\begin{align*}
 \what{\mycal{A}}^c_{\mathbb{V}_m}=\model{\what{\Sigma}^c_{\mathbb{V}_m},\what{\mycal{X}}^c_{\mathbb{V}_m},
   \what{Q}^c_{\mathbb{V}_m},\what{q}^c_{\mathbb{V}_m},\what{\delta}^c_{\mathbb{V}_m},\what{F}^c_{\mathbb{V}_m},\what{\kappa}^c_{\mathbb{V}_m}}
\end{align*}
 as follows:
\begin{description} 
\item[$\bullet$] $\what{\Sigma}^c_{\mathbb{V}_m}=\Sigma^c$.
\item[$\bullet$] $\what{\mycal{X}}^c_{\mathbb{V}_m}=\set{z_1,\ldots,z_m}$, where $z_i\notin \mycal{X}$.
\item[$\bullet$] $\what{Q}^c_{\mathbb{V}_m}=\what{Q}$.
\item[$\bullet$] $\what{q_0}^c_{\mathbb{V}_m}=\what{q}_0$.
\item[$\bullet$] $\what{\delta}^c_{\mathbb{V}_m}$ is defined by:
\begin{align*}
(q',E')  \in \what{\delta}^c_{\mathbb{V}_m} ((q,E),z_k) \textrm{ iff } & (q',E')  \in \what{\delta}^c ((q,E),(w_1,w_2))
 \textrm{ and } \\
 & \set{w_1,w_2} \subseteq V_k  \textrm{ for some } k \in [1,m]. 
\end{align*}

\item[$\bullet$] $F^c_{\mathbb{V}_m}=F^M$.
\item[$\bullet$] $\what{\kappa}^c_{\mathbb{V}_m}$ is defined by $\what{\kappa}^c_{\mathbb{V}_m}(z_i)=\set{(q,E)  \tst 
  (q,E) \in \what{\kappa}(x_1) \cap \what{\kappa}(x_2) \tand \set{x_1,x_2}=V_i}$.
\end{description} 
Let $\mathbb{V}_m=\set{V_1,\ldots,V_m}$ and $\mathbb{V}'_m=\set{V'_m,\ldots,V'_m}$.
We write $\mathbb{V}_m \preceq \mathbb{V}'_m$ iff ${V}_i \subseteq {V}'_i$ for all $i$.
Finally we let  $\mycal{A}^{\varepsilon}$ to be the  BVA $\biguplus_{\mathbb{V}_m} \what{\mycal{A}}^{c}_{\mathbb{V}_m}$ in which 
an $\varepsilon$-transition is added between every state  $(q,E)$ of $\what{\mycal{A}}^{c}_{\mathbb{V}_i}$ 
 and the  state  $(q,E)$ of $\what{\mycal{A}}^{c}_{\mathbb{V}_j}$ if $\mathbb{V}_i \preceq \mathbb{V}_j$. 

Besides, $\mycal{A}^{\varepsilon}$ is  subject to the following  condition $(\Pi)$: 
\begin{align*}
(\Pi)\begin{cases}
  \hspace{1cm} \textrm{ there is  an edge-simple  path} \\
 (q_1,E_1)\uberTo{\set{x_1,y_1}}(q_2,E_2)\uberTo{-} \ldots  \uberTo{\set{x_1,y_n}}(q_n,E_n) \\
%\end{align*}
\textrm { in }  \what{\mycal{A}}^c  \textrm{ where }  q_i \notin \kappa(x_1), \forall i\in\set{2,\ldots,n}, \\
\\
 \hspace{1cm} \textrm{ iff either there is an edge-simple  path } \\
\\
%\begin{align*}
 (q_1,E_1)\uberTo{z_k}(q_2,E_2)\uberTo{\_} \ldots \uberTo{z_k}(q_n,E_n) \\
%\end{align*}
\textrm{in } \mycal{A}^{\varepsilon} \textrm{ where }\set{x_1,y_1,y_n} \subseteq V_k,  \\
\end{cases}
\end{align*}

where the label $\set{\alpha_1,\alpha_2}$ denotes $(\alpha_1,\alpha_2)$ or $(\alpha_2,\alpha_1)$, 
and $-$ denotes an arbitrary label.

\begin{remark}
\label{inter:sub:BFVA:rq}
Notice that each $\what{V}^c_{\mathbb{V}_m}$ is obtained from $\what{A}^c$
by deleting some transitions and relabeling  the other transitions by new (1-letter) variables.  
\end{remark}

\begin{claim}
The $2$-BFVA $\what{\mycal{A}}^c$ and the BFVA $\mycal{A}^{\varepsilon}$
are equivalent.
\end{claim}
\begin{proof}
We shall show that 
\begin{align*}
L(\what{\mycal{A}}^c)=L(\mycal{A}^{\varepsilon}).
\end{align*}
For the inclusion "$\supseteq$",  we show that
 every accepting run
$r_l^{\varepsilon}=(\bs{q}_0,M_0^{\varepsilon})\uberTo{\alpha_1}\ldots\uberTo{\alpha_{m}}(\bs{q}_l,M_l^{\varepsilon})$ of $\mycal{A}^{\varepsilon}$ over a word $\boldsymbol{w}=w_1\ldots w_l\in \Sigma^{\star}$ 
 can be transformed into an accepting run  $\what{r}_l=(\bs{q}_0,\what{M}_0)\uberTo{\bs{\bs{\beta}}_1}\ldots \uberTo{\bs{\bs{\beta}}_l}(\bs{q}_l,\what{M}_l)$ of  $\what{\mycal{A}}^c$ over $\boldsymbol{w}$.
% such that ${M^\varepsilon}_{i}\sim \what{M}_i$\marginpar{A Definir $\sim$} for all $i$.
The proof is by induction on $l$. The base case $l=0$ follows trivially from the  definition of $\bs{q}_0$.
For the induction step, let $\bs{q}_l=(q_l,E_l)$ and a transition 
$(q_l,E_l)\uberTo{\alpha_{l+1}}(q_{l+1},E_{l+1})$ in $\mycal{A}^{\varepsilon}$.
From the definition of $A^{\varepsilon}$ it follows that there must exist at least a 
transition $(q_l,E_l)\uberTo{\bs{\beta}_{l+1}}(q_{l+1},E_{l+1})$ 
 in $\what{\mycal{A}}^c$. The choice of the latter transition depends on $\alpha_{l+1}$: 
\begin{itemize}
\item If $\alpha_{l+1}$ is a constant letter in $\Sigma$,  then the transition above is unique and 
 $\bs{\beta}_{l+1}=\alpha_{l+1}$ since the construction 
 of $\mycal{A}^{\varepsilon}$ out of $\what{\mycal{A}}^c$ keeps the transitions labeled with constant letters unchanged.  
\item If  $\alpha_{l+1}$ is a variable $z_k \in \mycal{X}^{\varepsilon}$. 
Then in this case 
$\bs{\beta}_{l+1}=(x_{l+1},y_{l+1})$    for some variables  
$x_{l+1},y_{l+1}$ so that $\set{x_{l+1},y_{l+1}} \subseteq V_k$. 
Thus, the  transition above is unique, remark \ref{inter:sub:BFVA:rq}.
Let us show that it is possible, i.e. 

\begin{align*}
\begin{cases}
\tif z_k \notin dom(M^{\eps}_{l})   \textrm{ then } x_{l},y_{l} \notin  dom(\what{M}_{l}), \tand \\
\tif x_{l} \in  dom(\what{M}_{l}) \textrm{ then }  M^{\eps}_{l}(z_k)=\what{M}_l(x_{l}), \tand \\ 
\tif y_{l} \in  dom(\what{M}_{l}) \textrm{ then }  M^{\eps}_{l}(z_k)=\what{M}_l(y_{l}).
\end{cases}
\end{align*}
\begin{itemize}
\item If $z_k \notin dom(M^{\eps}_l)$ then either \emph{(i.)}  the variable $z_k$ 
 never occurred in the run $r^{\eps}_l$ and in this case it follows from the path condition ($\Pi$) that $x_{l},y_{l} \notin  dom(\what{M}_{l})$. 
Or, \emph{(ii.)} the variable  $z_k$ 
   occurred   in the run $r^{\eps}_l$, say at some label $\bs{\beta}_{l'}$, and it was refreshed at some 
  state $\bs{q}_{l''}$ where $l' < l'' \le l$. In this case $V_k=\set{x_l,y_l}$ and from the item  \ref{} 
 it follows that both $x_l$ and $y_l$ are refreshed in $\bs{q}_{l''}$. Hence, $x_{l},y_{l} \notin  dom(\what{M}_{l})$.
 
 
\item If $x_{l}  \in  dom(\what{M}_{l})$ then the variable $x_l$  occurred in the run $\what{r}_l$, 
 say at some label $\alpha_{l'}$ and it was never refreshed. From the path condition $(\Pi)$
it follows that the variable $z_k$ occurred at the  label $\bs{\beta}_{l'}$.
Hence  $\what{M}_{l'}(x_l)=M^{\eps}_{l'}(z_k)=\what{M}_{l}(x_l)=M^{\eps}_{l}(z_k)$.
\item The case when $y_{l}  \in  dom(\what{M}_{l})$ is similar to the previous one.
\end{itemize}
\end{itemize}

\noindent For the inclusion "$\subseteq$",  we show that, 
 every accepting run  
\begin{align*}
r_l=(\bs{q}_0,\what{M}_0)\uberTo{\bs{\beta}_1}\ldots \uberTo{\bs{\beta}_l}(\bs{q}_l,\what{M}_l) \textrm { of }  
 \what{\mycal{A}}^c
\end{align*}
    over a word $\boldsymbol{w}=w_1\ldots w_l\in \Sigma^{\star}$ 
yields  an accepting run 
\begin{align*}
r_l^\eps=(\bs{q}_0,M_0^\eps)\uberTo{\alpha_1}\ldots\uberTo{\alpha_{l}}(\bs{q}_l,M_l^\eps) \textrm{ of } 
\mycal{A}^{\eps}
\end{align*}
 over $\boldsymbol{w}$. 
Remind that  $\mycal{A}^{\varepsilon}$ is  the  BVA $\biguplus_{\mathbb{V}_m} \what{\mycal{A}}^{c}_{\mathbb{V}_m}$ in which 
an $\varepsilon$-transition is added between every state  $(q,E)$ of $\what{\mycal{A}}^{c}_{\mathbb{V}_i}$ 
 and the  state  $(q,E)$ of $\what{\mycal{A}}^{c}_{\mathbb{V}_j}$ if $\mathbb{V}_i \preceq \mathbb{V}_j$. 
We describe how the run $r_l$  gives rise to the series  $\mathbb{V}_{m_1}, \ldots, \mathbb{V}_{m_k}$ such that 
  $\mathbb{V}_{m_1} \preceq \ldots \preceq  \mathbb{V}_{m_k} $ 
and  run $r^{\eps}_l$ can be decomposed into $r^{\eps}_{l_1}\uberTo{\eps}r^{\eps}_{l_2} \ldots \uberTo{\eps} r^{\eps}_{l_k}$ where 
each run $r^{\eps}_{l_i}$ occurs in the BFVA $A_{\mathbb{V}_{m_i}}$. 
  More precisely 
we construct the series  $\mathbb{V}_{m_1}, \ldots, \mathbb{V}_{m_k}$  from the path 
$\what{\pi}_l=\bs{q}_0 \uberTo{\bs{\beta}_1}\ldots \uberTo{\bs{\beta}_l}\bs{q}_l$. The idea is that we move?  in the BFVA $\what{A}_{\mathbb{V}_{m_1}}^c$ where ${\mathbb{V}_{m_1}}$ is minimal w.r.t. 
 the preorder "$\preceq$" until no transition is possible, then  we move to the next BFVA $\what{A}_{\mathbb{V}_{m_2}}^c$ via an $\eps$-transition etc.
Formally we proceed by induction on $l$. 
If $l=0$ then we take the minimal $\mathbb{V}_{m_1}$ w.r.t. $\preceq$ and we are done. 
For the induction step, assume that  $\mathbb{V}_{m_i}=\set{V_1,\ldots,V_m}$ is constructed from $\what{\pi}_l$, 
and let $(q_l,E_l)\uberTo{\bs{\beta}_{l+1}}(q_{l+1},E_{l+1})$  be a transition in $\what{\mycal{A}}^c$.
We argue next that there exists at least a possible transition 
$(q_l,E_l)\uberTo{\alpha_{l+1}}(q_{l+1},E_{l+1})$ in $\mycal{A}^{\varepsilon}$.
%hen the construction of $\mathbb{V}_{m_{i+1}}$  depends on    $\bs{\beta}_{l+1}$: 
This depends on     $\bs{\beta}_{l+1}$: 
\begin{itemize}
\item If $\bs{\beta}_{l+1}=a$, where $a \in \Sigma$, then it follows from the construction 
 of $\mycal{A}^{\varepsilon}$ from $\what{\mycal{A}}^c$ that $\alpha_{l+1}=a$ since the transitions 
 of $\what{\mycal{A}}^c$ labeled with constant letters are kept unchanged.

 % $\mathbb{V}^{l+1}_{n,m}:=\mathbb{V}^{l}_{n,m}$. 

\item If $\bs{\beta}_{l+1}=(x,y)$, where $x$ and $y$ are variables.
Then   there is a transition $(q_l,E_l)\uberTo{\alpha_{l+1}}(q_{l+1},E_{l+1})$ in $\what{\mycal{A}}^{c}_{\mathbb{V}_{m_i}}$
  such that $\alpha_{l+1}$ is a variable, say $z_k$, where $\set{x_{l+1},y_{l+1}} \subseteq V_k \in \mathbb{V}_{m_i}$,
and in this case we must show that this transition is possible i.e. 
\begin{align*}
\begin{cases}
\tif x_{l+1},y_{l+1} \notin  dom(\what{M}_{l})   \textrm{ then } z_k \notin dom(M^{\eps}_{l})   \tand \\
\tif x_{l+1} \in  dom(\what{M}_{l}) \textrm{ then }  M^{\eps}_{l}(z_k)=\what{M}_l(x_{l+1}), \tand \\ 
\tif y_{l+1} \in  dom(\what{M}_{l}) \textrm{ then }  M^{\eps}_{l}(z_k)=\what{M}_l(y_{l+1}).
\end{cases}
\end{align*}
\begin{itemize}
\item If $x_{l+1},y_{l+1} \notin  dom(\what{M}_{l})$ then there exist two transitions  labeled respectively with 
$\bs{\beta}_i$ and $\bs{\beta}_j$ in the path 
$\what{\pi}_l=\bs{q}_0 \uberTo{\bs{\beta}_1}\ldots \uberTo{\bs{\beta}_l}\bs{q}_l$ 
where $1\le i \le j \le l$ and $x_{l+1} \in \bs{\beta}_i$ and\footnote{We abuse of notation 
 and write $x \in (\beta_1,\beta_2)$ if $x \in \set{\beta_1,\beta_2}$}   $y_{l+1} \in \bs{\beta}_j$ and 
$x_{l+1}$ (resp. $y_{l+1}$) is refreshed in at least a  state $\bs{q}_s \in \set{\bs{q}_i,\ldots, \bs{q}_l}$ 
(resp. a  state $\bs{q}_{s'} \in \set{\bs{q}_j,\ldots, \bs{q}_l}$). 
If $i=j$ (i.e. $\bs{\beta}_i=(x_{l+1},y_{l+1})$)  then if follows from the construction of $A^{\eps}$
 that the variable $z_k$ (hence $V_k=\set{x_{l+1},y_{l+1}}$) is refreshed in the state $\bs{q}_i$ of $\mycal{A}^{\eps}$ as well, hence 
$z_k \notin M_l^{\eps}$. If  $i \neq j$ then it follows from the path condition ($\Pi$) that 
 $z_k\neq \alpha_r$ for all $r=1,\ldots,l$ (i.e. it is the first occurrence of $z_k$), hence $z_k \notin M_l^{\eps}$.  


\item If $x_{l+1} \in  dom(\what{M}_{l})$ then 
 there exists a transition  labeled  with 
$\bs{\beta}_i$  in the path 
$\what{\pi}_l=\bs{q}_0 \uberTo{\bs{\beta}_1}\ldots \uberTo{\bs{\beta}_l}\bs{q}_l$ 
where $1\le i  \le l$ and $x_{l+1} \in \bs{\beta}_i$  and 
$x_{l+1}$ is not refreshed the   states $\bs{q}_i,\ldots, \bs{q}_l$. 
It follows from the path condition ($\Pi$) that $\alpha_i=z_k$ and $z_k$ was not refreshed 
in the states $\bs{q}_i,\ldots, \bs{q}_l$ of $\mycal{A}^{\eps}$ as well. Hence 
$M^{\eps}_{l}(z_k)=\what{M}_l(x_{l+1})$.

\item The case when $y_{l} \in  dom(\what{M}_{l})$ is similar to the previous one.
\end{itemize}


\end{itemize}
This ends the proof of the Claim. \qed
\end{proof}


we  proceed again in two steps. 

\paragraph{First step.} We split again the states of $\mycal{A}=\model{{\Sigma},{\mycal{X}},{Q},{q}_0,{\delta},{F},{\kappa}}$ as in the proof 
 of Lemma \ref{2BFVA:BFVA:lem}: the construction  of  $\what{\mycal{A}}=\model{\what{\Sigma},\what{\mycal{X}},\what{Q},\what{q}_0,\what{\delta},\what{F},\what{\kappa}}$
is similar apart that $\what{\delta}$ is defined by 
\begin{align*}
   (q',E') \in \what{\delta} \big((q,E),  (\alpha_1,\alpha_2,\ldots,\alpha_{n+1})\big) \quad \textrm{ iff } \quad
     & q' \in \delta (q,  (\alpha_1,\alpha_2,\ldots,\alpha_{n+1})), \\
     &E' = (((E \cup \set{(\alpha_1,\alpha_2)})^{\star})_{|D'})^{\star},  \tand   \\
     &E = (((E' \cup \set{(\alpha_1,\alpha_2)})^{\star})_{|D})^{\star},   \\
\end{align*}
where $D=\mycal{X} \setminus \kappa^{-1}(q)$ and $D'=\mycal{X} \setminus \kappa^{-1}(q')$.

\begin{claim}
The $(n+1)$-BFVAs $\mycal{A}$ and $\what{\mycal{A}}$ are equivalent.
\end{claim}

\paragraph{Second Step.} The second  step consists in  transforming some of the  $(n+1)$-labels of 
$\mycal{\what{A}}$ into $n$-labels  by compacting the first and the second components 
 of (some of) the $(n+1)$-labels  into constant letters  as in the second step of the proof of 
Lemma \ref{2BFVA:BFVA:lem}. 
Out of the  $(n+1)$-BFVA  $\mycal{\what{A}}$ we     construct the 
 $(n+1)$-BFVA $\what{\mycal{A}}^c$ which is defined like $\mycal{\what{A}}$ apart that its transition function 
 $\what{\delta}^c$ is given by:
\begin{align*}
(q',E')  \in \what{\delta}^c ((q,E),(a,\alpha_3,\ldots,\alpha_n)) \textrm{ iff } & (q',E')  \in \what{\delta} ((q,E),(a,a,\alpha_3\ldots,\alpha_n)) \\
&\textrm{ where } a \in \Sigma, \tor \\
%%
 & (q',E')  \in \what{\delta} ((q,E),(\alpha_1,\alpha_2,\ldots,\alpha_n))
\tst  \\
 & (\alpha_1,a) \in E \tor (\alpha_2,a) \in E, \textrm{ for } a \in \Sigma.
\end{align*}

\begin{claim}
The $(n+1)$-BFVAs $\what{\mycal{A}}$ and $\what{\mycal{A}}^c$ are equivalent.
\end{claim}




%% Third Step
\paragraph{Third step.} The third  step consists in  transforming the remaining $2$-labels of 
$\mycal{\what{A}}^c$ into   variables by introducing new variable symbols. 
Let $\mathbb{V}_m=\set{V_1,\ldots,V_m}$ where $V_i \subseteq \mycal{X}$. 
For a fixed $\mathbb{V}_m$  and out of $\mycal{\what{A}}^c$ we     construct the BFVA $\what{\mycal{A}}^c_{\mathbb{V}_m}$ as follows: 
\begin{align*}
 \what{\mycal{A}}^c_{\mathbb{V}_m}=\model{\what{\Sigma}^c_{\mathbb{V}_m},\what{\mycal{X}}^c_{\mathbb{V}_m},
   \what{Q}^c_{\mathbb{V}_m},\what{q}^c_{\mathbb{V}_m},\what{\delta}^c_{\mathbb{V}_m},\what{F}^c_{\mathbb{V}_m},\what{\kappa}^c_{\mathbb{V}_m}}
\end{align*}
 as follows:
\begin{description} 
\item[$\bullet$] $\what{\Sigma}^c_{\mathbb{V}_m}=\Sigma^c$.
\item[$\bullet$] $\what{\mycal{X}}^c_{\mathbb{V}_m}=\set{z_1,\ldots,z_m}$, where $z_i\notin \mycal{X}$.
\item[$\bullet$] $\what{Q}^c_{\mathbb{V}_m}=\what{Q}$.
\item[$\bullet$] $\what{q_0}^c_{\mathbb{V}_m}=\what{q}_0$.
\item[$\bullet$] $\what{\delta}^c_{\mathbb{V}_m}$ is defined by:
\begin{align*}
(q',E')  \in \what{\delta}^c_{\mathbb{V}_m} ((q,E),(z_k,\alpha_3,\ldots,\alpha_n)) \textrm{ iff } & 
   (q',E')  \in \what{\delta}^c ((q,E),(\alpha_1,\alpha_2,\ldots,\alpha_n))
 \textrm{ and } \\
 & \set{\alpha_1,\alpha_2} \subseteq V_k  \textrm{ for some } k \in [1,m]. 
\end{align*}

\item[$\bullet$] $F^c_{\mathbb{V}_m}=F^M$.
\item[$\bullet$] $\what{\kappa}^c_{\mathbb{V}_m}$ is defined by $\what{\kappa}^c_{\mathbb{V}_m}(z_i)=\set{(q,E)  \tst 
  (q,E) \in \what{\kappa}(x_1) \cap \what{\kappa}(x_2) \tand \set{x_1,x_2}=V_i}$.
\end{description} 
Finally we let  $\mycal{A}^{\varepsilon}$ to be the  BVA $\biguplus_{\mathbb{V}_m} \what{\mycal{A}}^{c}_{\mathbb{V}_m}$ in which 
an $\varepsilon$-transition is added between every state  $(q,E)$ of $\what{\mycal{A}}^{c}_{\mathbb{V}_i}$ 
 and the  state  $(q,E)$ of $\what{\mycal{A}}^{c}_{\mathbb{V}_j}$ if $\mathbb{V}_i \preceq \mathbb{V}_j$. 

Besides, $\mycal{A}^{\varepsilon}$ is  subject to the following  condition $(\Pi)$: 
\begin{align*}
(\Pi)\begin{cases}
  \hspace{1cm} \textrm{ there is  an edge-simple  path } \\
 (q_1,E_1)\uberTo{(x_1,y_1,\ldots)}(q_2,E_2)\uberTo{-} \ldots  \uberTo{(x_1,y_n,\ldots)}(q_n,E_n) \\
%\end{align*}
\textrm { in }  \what{\mycal{A}}^c  \textrm{ where }  q_i \notin \kappa(x_1), \forall i\in\set{2,\ldots,n}, \\
\\
 \hspace{1cm} \textrm{ iff either there is an edge-simple  path } \\
\\
%\begin{align*}
 (q_1,E_1)\uberTo{(z_k,\ldots)}(q_2,E_2)\uberTo{\_} \ldots \uberTo{(z_k,\ldots)}(q_n,E_n) \\
%\end{align*}
\textrm{in } \what{\mycal{A}}^{\eps}\textrm{ where }\set{x_1,y_1,y_n} \subseteq V_k, 
\end{cases}
\end{align*}
\begin{claim}
The $(n+1)$-BFVA $\what{\mycal{A}}^c$ and the $n$-BFVA $\mycal{A}^{\varepsilon}$
are equivalent.
\end{claim}

%%
\paragraph{Basic fresh variable automata.}
In order to compare 
FVAs with existing models and to study the    properties of FVAs,
 it is simpler to neglect  the communication  symbols "!" and "?" in the FVAs, i.e. 
 to consider that alphabet consists of constants and variables.
This gives rise to the class of \emph{basic fresh variable automata}, or
 BFVAs for short. In other words, the definition 
 of BFVAs is the same as that of  FVAs 
 apart that the transition function becomes $\delta =Q\times \mcons \rightarrow 2^{Q}$. 
The definition of  run and language recognized 
by BFVAs is  the same as the one  of FVAs given in Def. \ref{run:lang:def}
apart that we have $\Sigma$ instead of $\overline{\Sigma}$, $\Sigma\cup \mycal{X}$ 
instead of $\mcons$, and $u$ instead of $\dual{u}$. 
 The simulation problem  is studied for both  FVAs and BFVAs.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 


==> choreography.tex <==
\subsection{Choreography}
\label{asynch:comm:sec}

We consider here the possibility
that the services  can collaborate by exchanging messages while the client is still waiting. 
In this setting the objective is similar: the simulation should be able to suitably
schedule   the available services and  provide the target service to the client.
More precisely,  a  sort of  \emph{fairness condition} 
 w.r.t. the client must be satisfied:   the client has not to 
 got stuck.
\begin{wrapfigure}{r}{0.17\textwidth}
  \vspace{-20pt}
  \begin{center}
\begin{tikzpicture}[shorten >=1pt,bend angle=30, node distance=2.6cm,on grid,auto, initial text=,
  bend angle=45] 
   \node[state,accepting](p_1)  {$p_1$};
   \node[state,initial left,accepting](p_0) [below =of p_1]    {$p_0$}; 
   \node[state,accepting](p_2) [below =of p_0] {$p_2$};
    \path[->] 
    (p_0) edge  [bend left]  node   {$?x$} (p_1)
    (p_1) edge  [bend left] node  {$!x$}  (p_0)
    (p_0) edge  [bend left]  node  {$!x$} (p_2)
    (p_2) edge  [bend left]  node  {$?x$}  (p_0);
\end{tikzpicture}
  \end{center}
  \vspace{-20pt}
  \caption{CFVA $\mycal{M}$.}
  \vspace{-10pt}
\end{wrapfigure}
This can be achieved in two steps. Firstly, we construct the game 
$\widehat{\mycal{G}}(\mycal{M},\mycal{C}\otimes \mathcal{A}_1 \otimes \cdots \otimes \mathcal{A}_n)$,
where $\mycal{C}$ is the client CFVA,  $\mycal{A}_i$'s are the services CFVAs, and $\mycal{M}$ is the CFVA
depicted below with $\kappa(x)=\set{p_0}$, where  the game 
$\widehat{\mycal{G}}$ is defined  like the game $\mycal{G}$ apart that the winning conditions are as follows: 
 an  infinite play is winning for \Eloise iff it contains at  least a move made by the client $\mycal{C}$.

Notice that the game $\widehat{\mycal{G}}$ defined so far
 ensures that in presence of a branching in the 
client behaviour, one of the branches is satistied by the services but not all of them, hence we need
to change $\widehat{\mycal{G}}$ as follows.
Secondly, all the moves of the form $p_{E}\uberTo{c_i} p_i$ where $p_E$ is an \Eloise position, and $c_i$s are 
client moves, are transformed into $p_{E}\uberTo{} p_{A} \uberTo{c_i} p_i$ where $p_A$ is a new \Abelard position.
Notice that the other moves  outgoing from $p_E$ and made by the services  are kept unchanged.
Summing up, $\widehat{\mycal{G}}$ is a $2$-players game with  \emph{B\"uchi   winning conditions}.
It  can be solved in polynomial time. 


==> long-ex-inter.tex <==
\section*{Examples(to remove)?}

\begin{example}
 We consider a more complex example of the intersection of BFVAs. 
Let  $\mycal{A}$ and $\mycal{B}$ be  the BFVAs depicted below, where 
$\kappa(y)=\kappa(w)=\set{p_1}$ and $\kappa(x)=\set{q_0}$. In the resulting 
BFVA $(\mycal{A} \times \mycal{B})^{\mathbb{V}_{2,1}^c}$ we have that 
$\kappa(z_1)=\kappa(z_3)=\emptyset$, where 
$\mathbb{V}_{2,1}=(\set{V_1,V_2},\set{C_1})$,  $V_1=\set{y,x}$, 
 $V_2=\set{w,y,x}$ and $C_1=\set{w,y,x,a}$.
And in the 
BFVA $(\mycal{A} \times \mycal{B})^{\mathbb{V'}_{2,1}^c}$ we have that 
$\kappa(z_1)=\emptyset$,  $ \kappa(z_3)=((1,0),\emptyset)$, where 
$\mathbb{V'}_{2,1}=(\set{V_1,V_2},\set{C_1})$,  $V_1=\set{y,x}$, 
 $V_2=\set{w,x}$ and $C_1=\set{w,y,x,a}$.
\end{example}
\pagestyle{empty}
\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=2cm, bend angle=50,
   on grid,auto, initial text=, >=stealth,semithick, inner sep=2pt,shorten >=1pt] 
   \node[state,initial] (p_0)   {$p_0$}; 
   \node[state,accepting] (p_1) [right =of p_0] {$p_1$};
   \node[state] (p_2) [right =of p_1] {$p_2$}; 
   \node[state] (p_3) [below =of p_1] {$p_3$}; 
   \node[state] (p_4) [below =of p_0] {$p_4$}; 

    \path[->] 
    (p_0)  edge   node [above] {a} (p_1)
    
    (p_1)  edge  node   {$w$} (p_3)
    (p_3)   edge  node   {$w$} (p_4)
    (p_4)   edge  node   {$w$} (p_1)
 
    (p_1) [bend left] edge  node  [above] {$y$} (p_2)
    (p_2) [bend left] edge  node  [below] {$y$} (p_1)
 
   -- (1,-3) node {$\mycal{A}$};

  \begin{scope}[xshift=8cm, yshift=0cm,node distance=2cm]
   \node[state,initial,accepting] (q_0)   {$q_0$}; 
   \node[state] (q_1) [right =of q_0] {$q_1$}; 

    \path[->] 
    (q_0) [bend left] edge   node [above] {$x$} (q_1)
    (q_1)  edge  node  [below] {$x$} (q_0)
    -- (1,-2.5) node {$\mycal{B}$};
 \end{scope}
  
  \begin{scope}[xshift=0cm, yshift=-7cm,node distance=2.5cm, bend angle=45]
   \node[state,initial] (r_{00})   {$_{0,0}$ }; 
   \node[state] (r_{11}) [right=of r_{00}] {$_{1,1}$ }; 
   \node[state] (r_{20}) [above=of r_{11}] {$_{2,0}$ }; 

   \node[state] (r_{30}) [right=of r_{11}] {$_{3,0}$ }; 
   \node[state] (r_{41}) [right=of r_{30}] {$_{4,1}$ }; 
   \node[state,accepting] (r_{10}) [right=of r_{41}] {$_{1,0}$ }; 
   \node[state] (r_{21}) [above=of r_{10}] {$_{2,1}$ }; 

   \node[state] (r_{31}) [below=of r_{10}] {$_{3,1}$ }; 
   \node[state] (r_{40}) [left=of r_{31}] {$_{4,0}$ }; 

    \path[->] 

    (r_{00})  edge   node  {$(a,x)$} (r_{11})

    (r_{11})  edge   node  {$(w,x)$} (r_{30})
    (r_{30})  edge  node   {$(w,x)$} (r_{41})
    (r_{41})  edge  node   {$(w,x)$} (r_{10})

    (r_{10})  edge  node   {$(w,x)$} (r_{31})
    (r_{31})  edge  node   {$(w,x)$} (r_{40})
    (r_{40})  edge  node   {$(w,x)$} (r_{11})

    (r_{11}) [bend left] edge   node [left] {$(y,x)$} (r_{20})
    (r_{20})  edge  node  [right] {$(y,x)$} (r_{11})

    (r_{10}) [bend left] edge   node [left] {$(y,x)$} (r_{21})
    (r_{21})  edge  node  [right] {$(y,x)$} (r_{10})

    -- (1,-2) node {$\mycal{A} \times \mycal{B}$};
 \end{scope}

\begin{scope}[xshift=0cm, yshift=-14cm,node distance=2.5cm, bend angle=45]
\tikzstyle{state}=[state with output]
   \node[state,initial] (r_{00})   {$_{0,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 
   \node[state] (r_{11}) [right=of r_{00}] {$_{1,1}$ \nodepart{lower} \begin{small}$a=x$\end{small}}; 
   \node[state] (r_{20}) [above=of r_{11}] {$_{2,0}$ \nodepart{lower} \begin{small}$y=a$\end{small}}; 

   \node[state] (r_{30}) [right=of r_{11}] {$_{3,0}$ \nodepart{lower} \begin{small}$w=a$\end{small}}; 
   \node[state] (r_{41}) [right=of r_{30}] {$_{4,1}$ \nodepart{lower} \begin{tiny}$x,w,a$\end{tiny}}; 
   \node[state,accepting] (r_{10}) [right=of r_{41}] {$_{1,0}$  \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 
   \node[state] (r_{21}) [above=of r_{10}] {$_{2,1}$ \nodepart{lower} \begin{small}$y=x$\end{small}}; 

   \node[state] (r_{31}) [below=of r_{10}] {$_{3,1}$ \nodepart{lower} \begin{small}$w=x$\end{small}}; 
   \node[state] (r_{40}) [below=of r_{31}] {$_{4,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{11e}) [left=of r_{40}] {$_{1,1}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{30e}) [left=of r_{11e}] {$_{3,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{20e}) [above=of r_{11e}] {$_{2,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{41e}) [above=of r_{30e}] {$_{4,1}$ \nodepart{lower} \begin{small}$w=x$\end{small}}; 
    \path[->] 

    (r_{00})  edge   node  {$(a,x)$} (r_{11})

    (r_{11})  edge   node  {$(w,x)$} (r_{30})
    (r_{30})  edge  node   {$(w,x)$} (r_{41})
    (r_{41})  edge  node   {$(w,x)$} (r_{10})

    (r_{10})  edge  node   {$(w,x)$} (r_{31})
    (r_{31})  edge  node   {$(w,x)$} (r_{40})
    (r_{40})  edge  node   {$(w,x)$} (r_{11e})

    (r_{11e})  edge  node   {$(w,x)$} (r_{30e})
    (r_{30e})  edge  node   {$(w,x)$} (r_{41e})

    (r_{41e})  edge  node  [left] {$(w,x)$}  (r_{10})

    (r_{11}) [bend left] edge   node [left] {$(y,x)$} (r_{20})
    (r_{20})  edge  node  [right] {$(y,x)$} (r_{11})

    (r_{10}) [bend left] edge   node [left] {$(y,x)$} (r_{21})
    (r_{21})  edge  node  [right] {$(y,x)$} (r_{10})


    (r_{11e}) [bend left] edge   node [left] {$(y,x)$} (r_{20e})
    (r_{20e})  edge  node  [right] {$(y,x)$} (r_{11e})

    -- (1,-2) node {$(\mycal{A} \times \mycal{B})^{M}$};
 \end{scope}
\end{tikzpicture}
\end{center}


\pagestyle{empty}
\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=2cm, bend angle=50,
   on grid,auto, initial text=, >=stealth,semithick, inner sep=2pt,shorten >=1pt] 

\begin{scope}[xshift=0cm, yshift=-14cm,node distance=2.5cm, bend angle=45]
\tikzstyle{state}=[state with output]
   \node[state,initial] (r_{00})   {$_{0,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 
   \node[state] (r_{11}) [right=of r_{00}] {$_{1,1}$ \nodepart{lower} \begin{small}$a=x$\end{small}}; 
   \node[state] (r_{20}) [above=of r_{11}] {$_{2,0}$ \nodepart{lower} \begin{small}$y=a$\end{small}}; 

   \node[state] (r_{30}) [right=of r_{11}] {$_{3,0}$ \nodepart{lower} \begin{small}$w=a$\end{small}}; 
   \node[state] (r_{41}) [right=of r_{30}] {$_{4,1}$ \nodepart{lower} \begin{tiny}$x,w,a$\end{tiny}}; 
   \node[state,accepting] (r_{10}) [right=of r_{41}] {$_{1,0}$  \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 
   \node[state] (r_{21}) [above=of r_{10}] {$_{2,1}$ \nodepart{lower} \begin{small}$y=x$\end{small}}; 

   \node[state] (r_{31}) [below=of r_{10}] {$_{3,1}$ \nodepart{lower} \begin{small}$w=x$\end{small}}; 
   \node[state] (r_{40}) [below=of r_{31}] {$_{4,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{11e}) [left=of r_{40}] {$_{1,1}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{30e}) [left=of r_{11e}] {$_{3,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{20e}) [above=of r_{11e}] {$_{2,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{41e}) [above=of r_{30e}] {$_{4,1}$ \nodepart{lower} \begin{small}$w=x$\end{small}}; 
    \path[->] 

    (r_{00})  edge   node  {$a$} (r_{11})

    (r_{11})  edge   node  {$a$} (r_{30})
    (r_{30})  edge  node   {$a$} (r_{41})
    (r_{41})  edge  node   {$a$} (r_{10})

    (r_{10})  edge  node   {$z_3$} (r_{31})
    (r_{31})  edge  node   {$z_3$} (r_{40})
    (r_{40})  edge  node   {$z_3$} (r_{11e})

    (r_{11e})  edge  node   {$z_3$} (r_{30e})
    (r_{30e})  edge  node   {$z_3$} (r_{41e})

    (r_{41e})  edge  node  [above] {$z_3$}  (r_{10})

    (r_{11}) [bend left] edge   node [left] {$a$} (r_{20})
    (r_{20})  edge  node  [right] {$a$} (r_{11})

    (r_{10}) [bend left] edge   node [left] {$z_1$} (r_{21})
    (r_{21})  edge  node  [right] {$z_1$} (r_{10})


    (r_{11e}) [bend left] edge   node [left] {$z_3$} (r_{20e})
    (r_{20e})  edge  node  [right] {$z_3$} (r_{11e})

    -- (1,-2) node {$(\mycal{A} \times \mycal{B})^{\mathbb{V}_{2,1}^c}$};
 \end{scope}
\end{tikzpicture}
\end{center}
%%%%%
\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=2cm, bend angle=50,
   on grid,auto, initial text=, >=stealth,semithick, inner sep=2pt,shorten >=1pt] 

\begin{scope}[xshift=0cm, yshift=-14cm,node distance=2.5cm, bend angle=45]
\tikzstyle{state}=[state with output]
   \node[state,initial] (r_{00})   {$_{0,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 
   \node[state] (r_{11}) [right=of r_{00}] {$_{1,1}$ \nodepart{lower} \begin{small}$a=x$\end{small}}; 
   \node[state] (r_{20}) [above=of r_{11}] {$_{2,0}$ \nodepart{lower} \begin{small}$y=a$\end{small}}; 

   \node[state] (r_{30}) [right=of r_{11}] {$_{3,0}$ \nodepart{lower} \begin{small}$w=a$\end{small}}; 
   \node[state] (r_{41}) [right=of r_{30}] {$_{4,1}$ \nodepart{lower} \begin{tiny}$x,w,a$\end{tiny}}; 
   \node[state,accepting] (r_{10}) [right=of r_{41}] {$_{1,0}$  \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 
   \node[state] (r_{21}) [above=of r_{10}] {$_{2,1}$ \nodepart{lower} \begin{small}$y=x$\end{small}}; 

   \node[state] (r_{31}) [below=of r_{10}] {$_{3,1}$ \nodepart{lower} \begin{small}$w=x$\end{small}}; 
   \node[state] (r_{40}) [below=of r_{31}] {$_{4,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{11e}) [left=of r_{40}] {$_{1,1}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{30e}) [left=of r_{11e}] {$_{3,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

 %  \node[state] (r_{20e}) [above=of r_{11e}] {$_{2,0}$ \nodepart{lower} \begin{small}$\emptyset$\end{small}}; 

   \node[state] (r_{41e}) [above=of r_{30e}] {$_{4,1}$ \nodepart{lower} \begin{small}$w=x$\end{small}}; 
    \path[->] 

    (r_{00})  edge   node  {$a$} (r_{11})

    (r_{11})  edge   node  {$a$} (r_{30})
    (r_{30})  edge  node   {$a$} (r_{41})
    (r_{41})  edge  node   {$a$} (r_{10})

    (r_{10})  edge  node   {$z_2$} (r_{31})
    (r_{31})  edge  node   {$z_2$} (r_{40})
    (r_{40})  edge  node   {$z_2$} (r_{11e})

    (r_{11e})  edge  node   {$z_2$} (r_{30e})
    (r_{30e})  edge  node   {$z_2$} (r_{41e})

    (r_{41e})  edge  node  [above] {$z_2$}  (r_{10})

    (r_{11}) [bend left] edge   node [left] {$a$} (r_{20})
    (r_{20})  edge  node  [right] {$a$} (r_{11})

    (r_{10}) [bend left] edge   node [left] {$z_1$} (r_{21})
    (r_{21})  edge  node  [right] {$z_1$} (r_{10})


%    (r_{11e}) [bend left] edge   node [left] {$z_2$} (r_{20e})
 %   (r_{20e})  edge  node  [right] {$z_2$} (r_{11e})

    -- (1,-2) node {$(\mycal{A} \times \mycal{B})^{\mathbb{V'}_{2,1}^c}$};
 \end{scope}
\end{tikzpicture}
\end{center}


==> preliminaries.tex <==
\section{Preliminaries}
\label{prelim:sec}

Familiarity with the standard  notions of first-order  signature, (ground) term,
arity, position and substitution is assumed. Let $\mathcal{X}$ be a countable set
of variables, $\Sigma$ a countable set of function symbols.  
Let $\mathcal{T}(\Sigma,\mathcal{X})$
denote the set of terms built out of the symbols in $\Sigma$ and the
variables in $\mathcal{X}$. We shall denote by $\mterms$ the set 
$\set{!,?}\times \terms$, where $\set{!,?}\cap (\Sigma \cup \mathcal{X})=\emptyset$.
If $t\in \terms$ then $!t$ (resp. $?t$) denotes sending (receiving) the message
$t$. 
 
A substitution is a mapping
$\{x_1\mapsto t_1,\ldots,x_n\mapsto t_n\}$ with variables $x_1, \ldots, x_n$ in
$\mathcal{X}$ and terms $t_1, \ldots, t_n$ in $\terms$.
If all the $t_i,i=1\ldots n$ are ground then we say that $\sigma$ is ground. 
 If $t$ is a term
and $\sigma$ is a
 substitution then $\sigma(t)$ denotes the term that results from the application
 of $\sigma$ to $t$. Given a finite set $M \subset \mathcal{X}$, a renaming  of the elements of  $M$ is 
a bijection $\eta: M \rTo \mathcal{X}$. For a function  
 $F: A \rTo B$, and $A'\subseteq A$, the restriction 
of $F$ on $A'$ is denoted by $F_{|A'}$.

If $G=(V_G,E_G)$ is a graph, then a path in $G$ is a sequence of the form $\pi =
g_{0}g_{1}\ldots g_{n}$ such that $(g_{i},g_{i+1}) \in E_{G}$ for
$0\leq i < n$. A path is \emph{simple} if $g_{i} \neq g_{j}$ for $i,j
\in \set{0,\ldots ,n}$ and $i \neq j$. The integer $n$ is the length
of $\pi$, $g_{0}$ is the source of $\pi$, noted $\source \pi = g_{0}$,
and $g_{n} $ is the target of $\pi$, noted $\target \pi = g_{n}$.  We
denote by 
$\Pip(G)$ the set of simple non empty (i.e. of length greater than
$0$) paths in $G$.
A matching problem of a term $t$ by a term $u$, denoted by $\matchq{t}{u}$, 
is solvable iff there is  a substitution $\sigma$ such that $\sigma(t)=u$.
The set of solutions of $\matchq{t}{u}$ is denoted by $\match{t}{u}$.

\mycomment{TODO}{Short introduction to $2$-player reachability games.}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 


==> semi-decidability.tex <==
\section{A semi decision procedure for  \vaut{automata} simulation}

In this section we  show that the problem of  \gsim{simulation} of 
\vaut{automata} is semi-decidable. Then we show that it is 
 decidable under some assumptions.
\mycomment{Revise the following when the results are stable}{We proceed in two steps. Firstly, we show  in Section \ref{contruct:monotonic:sec}  
how to construct a particular strategy for \Abelard  so that 
the game-graph is might be finite. Then we show that such strategy is correct and complete. 
 Secondly,  we show in Section \ref{termination:sec} 
that the game graph induced by such strategy is actually finite.  
Therefore, a standard reachability algorithm can be used to solve this $2$-player 
 game.}


%Summing up, from  the Lemma  \ref{equiv:sim:lem:1} 
%and the Proposition \ref{posi:monotonic:strat:lemma}  we get the following conclusion.  

\mycomment{WB}{The following Th. can be turned into a definition, there is no need
 to prove the correctness and soundness of the game theoretic formulation, 
as in the literature.}
\begin{theorem}
\label{equiv:sim:th}
Let $A$ and $B$ be two \vaut{automata}. 
 There is a \gsim{simulation} of $A$ by $B$ (in the sense of Definition \ref{sim:def}) 
iff \Eloise has a   winning strategy  in the game $\mathcal{G}(A,B)$. 
\end{theorem}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 


==> yc-vautomata.tex <==
\section{Fresh variable automata}
\label{vaut:sec}
In this section we introduce the formalism of FVAs and
explain the idea behind it through simple examples.  This formalism is
similar to the classical automata except for two features. Firstly,
the actions no longer belong to a finite alphabet but to an infinite
set of terms. Secondly, at each state some of the variables are
replaced with fresh ones.
% depending on the their scope.

\input example.tex

\begin{definition}%{(Variable automaton)}
  A \emph{FVA} is a tuple
  $A=\model{\Sigma,\mathcal{X},Q,Q_0,\delta,F,\kappa}$ where $\Sigma$
  is a denumerable set of functional symbols,
  $\mathcal{X}$ is a finite set of variables,
  $Q$ is a (possibly infinite) set of states, $Q_0\subseteq Q$ is a
  set of initial states, $\delta=Q \times \mterms \to 2^{Q}$ is a
  transition function, $F\subseteq Q$ is a set of accepting states,
  and $\kappa: \mycal{X} \rightarrow  2^Q$ is the refreshing function that associates 
  to every  variable the (possibly empty) set of states where it is refreshed.
\end{definition}

FVAs recognize \emph{words} which are 
sequences of actions. The \emph{mirror} of a word $\omega=
\frac ?! t_1\cdot \frac ?! t_n\cdot \ldots$ is the word
$\overline\omega = \frac !? t_1\cdot \frac !? t_n\cdot \ldots$.  

%% Not Needed 
%% Given
%% a FVAs
%% $A=\model{\Sigma,\mathcal{X},Q,Q_0,\delta,F,\kappa}$, the
%% \emph{underlying} rooted multi-graph of $A$ denoted by $\mycal{G}_A$,
%% is defined by $v^{\star}(\mycal{G}_A)=Q_0$, $V(\mycal{G}_A)=Q$, and
%% $E(\mycal{G}_A)=\set{(q_1,q_2) \;|\; \exists t \in \mterms \tst q_2
%%   \in \delta(q_1,t)}$.\footnote{yc: need to keep multiplicity of edges
%%   ?}


\begin{example}
  \label{semantics:var:example}
  The left-hand side of Figure \ref{vautomata:fig:1} depicts a
  FVA where 
  % the back-vertices are $p_0$ and $p_1$ since
  % they are pointed by a back-edge, with
  $\kappa(x)=\set{p_1}$ and $\kappa(y)=\set{p_0}$.  That is, the variable $x$
  (resp. $y$) is refreshed when passing through $p_1$ (resp. $p_0$),
  and the variable $z$ is never refreshed (refreshment is defined
  below).  
\end{example}

\begin{figure}
\label{vautomata:fig:1}
\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=2cm, bend angle=45,
   on grid,auto, initial text=, >=stealth] 
   \node[state,initial,accepting] (p_0)   {$p_0$}; 
   \node[state] (p_1) [below =of p_0] {$p_1$}; 
   \node[state,accepting](p_2) [below =of p_1] {$p_2$};
    \path[->] 
    (p_0) edge  node {$?x$} (p_1)
    (p_1) edge  node  {$?y$} (p_2)
    (p_2) edge  [bend left] node  {$?x$}  (p_1)
    (p_2) edge [bend right] node [right] {$?z$} (p_0);

  \begin{scope}[xshift=7.8cm, yshift=0cm,node distance=2cm]
   \node[state,initial,accepting] (q_0)   {$q_0$}; 
   \node[state] (q_1) [below =of q_0] {$q_1$}; 
   \node[state,accepting] (q_2) [below =of q_1] {$q_2$}; 
   \node[state] (q_{11}) [below left=of q_2] {$q_1^1$}; 
   \node[state,accepting] (q_{21}) [below left=of q_{11}] {$q_{2}^1$}; 
   \node[state] (q_{14}) [below left=of q_{21}] {$q_{1}^4$}; 
   \node[state,accepting] (q_{24}) [below left=of q_{14}] {$q_{2}^4$}; 

   \node[state,accepting] (q_{06}) [below right=of q_{21}] {$q_0^6$}; 
   \node[state] (q_{16}) [below =of q_{06}] {$q_{1}^6$}; 

   \node[state,accepting] (q_{03}) [below right =of q_2] {$q_0^3$}; 

   \node[state] (q_{13})   [below =of q_{03}] {$q_{1}^3$};
   \node[state,accepting] (q_{23}) [below =of q_{13}] {$q_{2}^3$};

   \node[state,accepting] (q_{05}) [below right=of q_{23}] {$q_{0}^5$};
   \node[state]           (q_{15}) [below left=of q_{23}] {$q_{1}^5$};


   \node[state] (q_{17}) [below left=of q_{24}] {$q_{1}^7$};
   \node[state,accepting] (q_{07}) [below right=of q_{24}] {$q_{0}^7$};
   \node[state] (q_{18}) [below =of q_{07}] {$q_{1}^8$};

    \path[->] 
    (q_0) edge  node  {$?x$} (q_1) 
    (q_1) edge  node  {$?y$} (q_2) 
    (q_2) edge  node  {$?z$} (q_{03}) 
    (q_2) edge  node [above left] {$?x$} (q_{11}) 

    (q_{11}) edge  node  [above left] {$?y$} (q_{21}) 
    (q_{21}) edge  node  [above left] {$?x^1$} (q_{14}) 
    (q_{14}) edge  node  [above left] {$?y$} (q_{24}) 

    (q_{21}) edge  node  {$?z$} (q_{06}) 
    (q_{06}) edge  node  {$?x$} (q_{16}) 

    (q_{03}) edge  node  {$?x$} (q_{13}) 
    (q_{13}) edge  node  {$?y^1$} (q_{23}) 

    (q_{23}) edge  node  [above left] {$?x^2$} (q_{15}) 
    (q_{23}) edge  node  {$?z$} (q_{05}) 

    (q_{24}) edge  node [above left] {$?x^2$} (q_{17})
    (q_{24}) edge  node  {$?z$} (q_{07}) 
    (q_{07}) edge  node  {$?x^1$} (q_{18}) 

;
\end{scope}
\end{tikzpicture}
\end{center}
\caption{A FVA and its related infinite
  unfolding. Different possible values of a given variable are denoted
with a superscript}
\end{figure}
 We formulate the notions of run, simulation, etc. on the \emph{unfolding}
of a FVA, i.e. in the construction of an infinite tree
in which each path is a sequence of transitions in the automaton. A
grammar for this tree is specified by an \emph{equational system}
built from the initial states and the transition relation in the
original FVA.
%as formalized in the following definition. The equational system are
%close to regular expressions.  \mycomment{TODO}{More precise, ref?}
%\newpage
\begin{definition}%{(Equational systems)}
\label{equational:sys:def}
Let $\mathcal{F}$ be a set of non-terminals and $\mycal{X}$ a
set of (first order) variables.  An \emph{equational system} is a
couple $\langle X_0, \big\{X_i=S_i \big\}_{i\in I}\rangle$,
where % $\kappa: \mycal{X} \to \mycal{F}$ is the scope function,
$X_0 \in \mycal{F}$ is the axiom, for all $i,j \in I$ $X_i \in \mycal{F}$
and $i\neq j$ implies $X_i\neq X_j$, and $S_i$ is a \emph{behavior
  expression} as defined by the following grammar:%% \footnote{YC:
  %% addition of $\nu x$ to have explicite variable refreshment in the
  %% run}
\begin{align*}
S ::=  (t,q) \gvert (t,q) ; S   \gvert \nu x.\, S \gvert Z \gvert  S  \lor S 
\end{align*} 
where $t \in \mterms$, $q\in Q$, and $Z\in \mycal{F}$.
\end{definition}
%% We note that the size of an equational system (i.e. the total size of
%% equations) is linear in the size of the transition relation.
%% \observe{Make explicit the correspondence between the subset of
%%   feed-back vertices (i.e. states) of $Q$ and the fixed point
%%   variables $\mycal{F}$? \textbf{yc}: done ?}

For instance an equational system for the FVA of
Example \ref{semantics:var:example} is composed of three equations:
\begin{align*}
\begin{cases} 
X_0 & = \; \nu y . (?x,q_1); X_1  \\
 X_1 &= \; \nu x . (?y,q_2) ; X_2 \\
X_2 &= (?x,q_1);X_1 \; \lor \;  (?z,q_0); X_0 \\
\end{cases}
\end{align*} 
given that in the original automaton $\kappa(x)= X_1$ and $ \kappa(y)=
X_0$, and $X_0$ is the axiom.  
%% \observe{Relate this
%%   choice of $\kappa$ to Example 3 after the link between the states
%%   and the fixed-point variables being established.}

%\textsc{Manque la construction explicite d'un systeme equationnel a
%  partir d'un automate}

The \emph{(infinite) unfolding} of an automaton $\mycal{A} = \langle
X_0, \big\{X_i=S_i \big\}_{i\in I}\rangle$ is the (infinite) tree
obtained by the iterated application of the production rules $X_i\to
S_i$ on $X_0$. Each application is called an \emph{unfolding} of the
automaton. 

% The memory $\mycal{M}$ keeps the history of the  renamings that have been  applied. 
\ucomment{%
  The rule (\ref{Unfold}) reduces an expression of the form $ [\theta]
  (X_i)$ to $[\rho^i \circ \theta](S_i)$ where $\rho^i$ is a renaming
  of all the variables of $\kappa^{-1}(X_i)$.  The first condition of
  this rule states that the co-domains of the fresh renamings must be
  pairwise disjoint. The second condition states that the very first
  fresh renaming w.r.t. to each non-terminal must be the
  identity.  A renaming that enjoys these properties is called a
  \emph{fresh renaming}.  The rule (\ref{Simplify}) states that the
  earlier fresh renaming $\rho^i$ of the variables under the scope of
  $X_i$ has not to be considered because the variables of $X_i$ will
  be refreshed next by another fresh renaming by the rule
  \ref{Unfold}.  The rule (\ref{Eval}) applies the renamings from
  right to left to the atomic term, that is, $\ttt{eval}([\rho_1 \circ
  \cdots \circ \rho_n](t)) = \ttt{eval}([\rho_1 \circ \cdots \circ
  \rho_{n-1}](\rho_n (t)))$.}

\ucomment{The application of a substitution $\sigma$ to a behavioral expression, denoted by 
  $\sigma(S)$ is defined inductively by $\sigma(S_1 \oplus S_2)=\sigma(S_1) \oplus \sigma(S_2)$, 
  $\oplus \in \set{;, \lor}$  and $\sigma(X)=X$ if $X$ is a non-terminal.   }


%% \mycomment{TODO}{More precise on the definition of the infinite FVAs which 
%% corresponds to the unfolding of an equational system, since the unfolding is only defined 
%% on equational systems. }

\begin{example}
\label{vaut:ex}
Consider again the FVA of Ex.~\ref{semantics:var:example}
and its equational system. 
% \begin{align*}
% \begin{cases} 
% X_0 & = \; \nu y. (?x,q_1); X_1  \\
%  X_1 &= \; \nu x. (?y,q_2) ; X_2 \\
% X_2 &= (?x,q_1);X_1 \; \lor \;  (?z,q_0); X_0 \\
% \end{cases}
% \end{align*} 
The unfolding of this
equational system is obtained through the following derivations by
applying the reduction rules given earlier.  The related infinite
FVA is depicted on the right side of Figure
\ref{vautomata:fig:1}.  

%The names \ref{Unfold}, \ref{Simplify} and \ref{Distribute} and
%\ref{Eval} of the rules of $\mathcal{R}$ are abbreviated by
%\ttt{U,S,D} and \ttt{E}, respectively.  We do not make explicit the
%memory $\mycal{M}$ since it can be understood.

$$
\begin{array}{rl}
  X_0 =&  ( \nu y ; (?x,q_1); X_1 ) \\
  =& ( \nu y . (?x,q_1); ( \nu x . (?y,q_2) ; X_2 ) ) \\
  =& ( \nu y . (?x,q_1); ( \nu x . (?y,q_2) ; ( (?x,q_1);X_1 \; \lor \;  (?z,q_0); X_0 ) ) ) \\
  =& ( \nu y . (?x,q_1); ( \nu x . (?y,q_2) ; ( (?x,q_1);( \nu x .
  (?y,q_2) ; X_2 ) \; \\
  &\lor \;  (?z,q_0); ( \nu y . (?x,q_1); X_1 ) ) ) ) \\
  =& ( \nu y . (?x,q_1); ( \nu x . (?y,q_2) ; ( (?x,q_1);( \nu x .
  (?y,q_2) ; ( (?x,q_1);X_1 \;\\
  &\lor \;  (?z,q_0); X_0 ) ) \; \lor \;  (?z,q_0); ( \nu y . (?x,q_1); ( \nu x . (?y,q_2) ; X_2 ) ) ) ) ) \\

\end{array}
$$
%\ucomment{\begin{align}
%X_0 &\uberTo{\ttt{U}} [\rho^{0}_{1}](x;X_1) \;\; \textrm{ where } \rho^{0}_{1}=y\mapsto y  \label{st:1} \\
%& \uberTo{\ttt{D,E}} x;[\rho^{0}_{1}](X_1) \label{st:2} \\
%&  \uberTo{\ttt{U}} x; [\rho^{1}_{1}\rho^{0}_{1}](y; (x;X_1 \; \lor \;  z; X_0))\;\; \textrm{ where } \rho^{1}_{1}=x\mapsto x \notag\\
%&  \uberTo{\ttt{D,E}} x; (y; (x;[\rho^{1}_{1}\rho^{0}_{1}](X_1) \; \lor \;  z; [\rho^{1}_{1}\rho^{0}_{1}](X_0))) \notag\\
%& \uberTo{\ttt{S}} x; (y; (x;[\rho^{0}_{1}](X_1) \; \lor \;  z; [\rho^{1}_{1}](X_0))), \textrm{ since } [\rho^{1}_{1}\rho^0_1](X_1)\to \rho^0_1(X_1) \tand 
%                [\rho^{1}_{1}\rho^0_1](X_0) \to [\rho^1_1](X_0) \label{st:3}\\
%& \uberTo{\ttt{U}} x; (y; (x; [\textcolor{red}{\rho^{1}_{2}} \rho^{0}_{1}](y; (x;X_1 \; \lor \;  z; X_0 )) 
%     \; \lor \;  z; [\textcolor{red}{\rho^{0}_{2}} \rho^{1}_{1}](x;X_1))), \notag\\
%& \;\;\; \textrm{ where } \rho^{1}_{2}= x \mapsto x^1 \tand \rho^{0}_{2}= y\mapsto y^1 \notag\\
%& \uberTo{\ttt{D,E}} 
%x; (y; (x; (\textcolor{red}{y}; (\textcolor{red}{x^1}; [\textcolor{red}{\rho^{1}_{2}} \rho^{0}_{1}](X_1) \; \lor \;  z; [\rho^{1}_{2} \textcolor{red}{\rho^{0}_{1}}](X_0) )) 
%     \; \lor \;  z; (x;[\rho^{0}_{2} \textcolor{red}{\rho^{1}_{1}}](X_1)))), \notag\\
%&  \uberTo{\ttt{S}} x; (y; (x; ({y}; ({x^1};  [\rho^{0}_{1}](X_1) \; \lor \;  z; [\rho^{1}_{2}] (X_0) )) 
%     \; \lor \;  z; (x; [\textcolor{red}{\rho^{0}_{2} }](X_1)))),  \label{st:4} \\
%&  \uberTo{\ttt{U}} x; (y; (x; ({y}; ({x^1}; [\rho^{1}_{3}\rho^{0}_{1}]\big( y; (x;X_1 \; \lor \;  z; X_0 )\big) \; \lor \;  \notag \\
%& \hspace{2cm} z; [\rho^{0}_{3}\rho^{1}_{2}] (x; X_1) )) 
%     \; \lor \;  z; (x;[\rho^{1}_{3}\rho^{0}_{2}] ( y; (x;X_1 \; \lor \;  z; X_0)))), \notag\\
%& \;\;\; \textrm{ where } \rho^{1}_{3}=x\mapsto x^2 \tand \rho^{0}_{3}=y\mapsto y^3 \notag\\
%&  \uberTo{\ttt{D,E}} x; (y; (x; ({y}; ({x^1}; \big( \textcolor{red}{y}; (\textcolor{red}{x^2};[\rho^{1}_{3}\rho^{0}_{1}]X_1 \; \lor \;  z; [\rho^{1}_{3}\rho^{0}_{1}]X_0 )\big) \; \lor \;  \notag \\ 
%& \hspace{2cm} z; [\rho^{0}_{3}\rho^{1}_{2}] (x; X_1) )) 
%     \; \lor \;  z; (x; ( \textcolor{red}{y^1}; (\textcolor{red}{x^2};[\rho^{1}_{3}\rho^{0}_{2}] X_1 \; \lor \;  z; [\rho^{1}_{3}\rho^{0}_{2}] X_0)))), \label{st:5}
%   \end{align}} 
To make clear the correspondence between this series
 of derivations and the related infinite unfolding depicted at the
 right of Figure \ref{vautomata:fig:1}, we notice that the expression
 each line in the above equality sequence corresponds to unfolding of
 all leaf nodes in its predecessor.  

%\ucomment{(\ref{st:1}) above
%   corresponds to the state $q_0$, the expression (\ref{st:2}) to the
%   unfolding up to the state $q_1$, the expression (\ref{st:3}) to the
%   unfolding up to the states $q_1^1,q_0^3$, the expression
%   (\ref{st:4}) to the the unfolding up to the states
%   $q_1^4,q_0^6,q_1^3$, and the expression (\ref{st:5}) corresponds to
%   the the unfolding up to the states
%   $q_1^7,q_0^7,q_1^6,q_1^5,q_0^5$.}


\end{example}

Now we are ready to define the notions of run and language.  First we
define a transition relation $\exec{}{}$ on the subtrees of an
unfolding $T$ as follows:
\begin{center}
  \parbox[t]{0.45\linewidth}{%
    \infer[~]{T \exec{\varepsilon,q_0}{\emptyset} T}{~}  
    \infer[\ensuremath{t\in\gterms}]{S \exec{\omega,q}{\set{x\mapsto t} \cup \theta_{|\text{dom}(\theta)\setminus\set{x}}}
      S'}{S \exec{\omega,q}\theta \nu x  . S'}}
  \parbox[t]{0.45\linewidth}{%
    \infer[i\in\{1,2\}]{S \exec{\omega,q}\theta S_i}{S \exec{\omega,q}\theta S_1 \lor S_2}
    \infer[\star\in\{!,?\}]{S \exec{\omega\cdot \star u\theta,q' }\theta S'}{S \exec{\omega,q}\theta (\star u,q') ; S'}}
\end{center}

By construction if $T\exec{\omega,q}{\theta} S$ then the variable
automaton, after performing the actions $\omega$, is in the state $q$
and the current valuation of variables is given by $\theta$. The word
recognized by this run is the mirror of $\omega$.
\begin{definition}
\label{run:def}
A FVA $A=\model{\Sigma,\mathcal{X},Q,Q_0,\delta,F,\kappa}$
with an unfolding $T$ \emph{recognizes} a finite word $\omega$ if
there exists a subtree $S$ of $T$ and a run
$T\exec{\overline{\omega},q}{\theta} S$ $q_n $ such that $q_n$ is a
final state of $A$. The set of words recognized by $A$ is denoted by
$L(A)$.
\end{definition}

\begin{example}
  Consider the FVA $A$ of Ex.~\ref{vaut:ex} depicted in
  Fig.~\ref{vautomata:fig:1}.  The tree-word $!a\, !f(a,a)\, ?g(a)
  \, !f(c,d)$ is recognized by $A$.
\end{example}

The following Lemma is not hard to prove.
\begin{lemma}
Let $\mycal{A}=\model{\Sigma,\mathcal{X},Q,Q_0,\delta,F,\kappa}$ 
and $\mycal{A}'=\model{\Sigma,\mathcal{X},Q,Q_0,\delta,F,\kappa'}$ be two 
FVAs. If $\kappa \subseteq \kappa'$, then 
$L(\mycal{A}) \subseteq L(\mycal{A}')$.
\end{lemma}


% \begin{lemma}
% \label{refresh:once:vaut:lemma}
% Let $A=\model{\Sigma,\mathcal{X},Q,Q_0,\delta,F,\kappa}$ be a 
% FVA. There exists a  FVA 
% $B=\model{\Sigma,\mathcal{X}',Q',Q'_0,\delta',F',\kappa'}$ that 
% recognizes the same language 
% such that the variables of $B$ are refreshed at most at one state,
% that is, for all $x \in \mathcal{X}'$ we have that  $|\kappa'(x)|\le 1$.
% \end{lemma}
% This lemma can be shown by renaming bound variables (bound w.r.t. $\nu$) thanks  
%  to the mechanism of  $\alpha$-conversion 
%  in the equational system of $A$, like in the $\lambda$-calculus
%  where the operator "$\nu$" behaves like the "$\lambda$".  
% \red{\textsc{Attention: il faut tenir  en compte la recursion.} }

\ucomment{For the special case of an alphabet consisting of variables and constants only  we can 
give an equivalent definition of the run of  FVAs as  follows.} 
We define  the notion of run of  FVAs.
This definition    is close to the one  of register automata: the 
idea is that a fixed number of  registers is sufficient to store the variable values. 
Let   $\mycal{A}=\model{\Sigma,\mathcal{X},Q,Q_0,\delta,F,\kappa}$ be a FVA.  
Intuitively,  we need  a memory $M$ to store the values of variables.  
The transition  $ q_1 \uberTo{t} q_2 $, where $t\in \mterms$ is a term, means 
 that, if $u \in \overline{\mycal{T}}(\Sigma)$ is the input  term, then  passing from $q_1$ to $q_2$ requires 
 to  compute $\sigma$ the solution of the matching problem $\matchq{M(t)}{\dual{u}}$,
 update  the  memory $M$ to $M \uplus \sigma$, and 
  free  all the variables in  $\kappa^{-1}(q_2)$ from $M$.
The formal definition follows.
A \emph{configuration}  is a pair  $(q,M)$ where $q \in Q$ and 
$M:\mycal{X} \pfun  \Sigma$  is a partial function.
 We define a transition relation  over the  configurations 
  as follows:  $(q_1,M_1)\uberTo{u} (q_2,M_2)$, where $u\in \overline{\mycal{T}}(\Sigma)$,
   iff there exist a term $t \in \mterms$, 
  such that  $q_2\in \delta(q_1,t)$, and a substitution $\sigma=\matchq{M(t)}{\dual{u}}$
  so that $M_2= (M_1 \uplus \sigma) \setminus \kappa^{-1}(q_2)$

A finite tree-word $u=u_1u_2\ldots u_n \in {\overline{\mycal{T}}(\Sigma)}^*$ is \emph{recognized} by 
$\mycal{A}$ iff  there exists a sequence 
$(q_0,M_{0}) \uberTo{u_1}(q_1,M_1)\uberTo{u_2} \ldots \uberTo{u_n}(q_n,M_n)$, such that 
$M_{0}=\emptyset$, $q_0\in Q_0$ and $q_n \in F$.



\subsection{Comparison with other models}
FVAs (in wich the alphabet consists of  variables and  letters) are 
incomparable with v-automata \cite{GKS10}. On the one hand the language 
$L=\set{a_1a_1a_2a_2\cdots a_n a_n, n\ge 0, a_i \in \Sigma}$ can not be   
recognized by a v-automaton as shown in \cite{GKS10}. However, 
 it can be recognized by the following FVA, where 
$\kappa(x)=\set{p_0}$. 
\begin{center}
\begin{tikzpicture}[shorten >=1pt,node distance=2cm, bend angle=60,
   on grid,auto, initial text=, >=stealth] 
   \node[state,initial,accepting] (r_0)   {$p_0$}; 
   \node[state] (r_1) [right =of r_0] {$p_1$}; 
    \path[->] 
    (r_0) [bend left] edge   node [above] {$x$} (r_1)
    (r_1) [bend left] edge  node  [below] {$x$} (r_0);
\end{tikzpicture}
\end{center}
On the other hand,  the language of all the words in 
which the last letter is different from all the other letters 
can be recognized by a v-automaton but not by a FVA,
since there is no way to express that a variable  is distinct from  
other variables.  In fact, the subclass of variable automata without free variables 
  is  exactly the subclass 
 of FVAs without fresh variables.    

 
FVAs are strictly 
less expressive than register automata \cite{tcs/KaminskiF94}. 
On the one hand, the language of all words  in which some 
letter appears exactly twice can be recognized by a register automaton 
but not by a FVA. On the other hand, 

\mycomment{}{It was shown in \cite{GKS10} that a v-automaton 
 can be simulated by a \emph{non-deterministic} register automaton \cite{ijfcs/KaminskiZ10}
 but not a deterministic one. Exploit this ... }





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 

